Task-aware Privacy Preservation for Multi-dimensional Data

Local differential privacy (LDP) can be adopted to anonymize richer user data attributes that will be input to sophisticated machine learning (ML) tasks. However, today's LDP approaches are largely task-agnostic and often lead to severe performance loss -- they simply inject noise to all data attributes according to a given privacy budget, regardless of what features are most relevant for the ultimate task. In this paper, we address how to significantly improve the ultimate task performance with multi-dimensional user data by considering a task-aware privacy preservation problem. The key idea is to use an encoder-decoder framework to learn (and anonymize) a task-relevant latent representation of user data. We obtain an analytical near-optimal solution for the linear setting with mean-squared error (MSE) task loss. We also provide an approximate solution through a gradient-based learning algorithm for general nonlinear cases. Extensive experiments demonstrate that our task-aware approach significantly improves ultimate task accuracy compared to standard benchmark LDP approaches with the same level of privacy guarantee.

==> figures_latex/fig_ml_nonlinear.tex <==
\begin{figure*}[t]
\vskip 0.2in
\begin{center}
% \subfigure[]{
% {\includegraphics[width=0.4\columnwidth]{figures/valuation_test_loss_privacy.pdf}}
% \label{fig:valuation_loss_privacy}
% }
% \subfigure[]{
% {\includegraphics[width=0.4\columnwidth]{figures/cancer_test_loss_privacy.pdf}}
% \label{fig:cancer_loss_privacy}
% }
\subfigure{
\input{figures_tikz/legend}
}\\
\subfigure{
\input{figures_tikz/valuation_test_loss_privacy_nonlinear}
}
% \subfigure{
% \input{figures_tikz/cancer_test_loss_privacy}
% }

\caption{Task loss $l(\hat{y}, y)$ under different LDP budgets for real estate valuation, when a one-hidden-layer feedforward neural network is adopted for both encoder and decoder. }
\label{fig:ml_nonlinear}
\end{center}
\vskip -0.2in
\end{figure*}


==> figures_latex/fig_neural_network.tex <==
\begin{figure*}[t]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.4\columnwidth]{figures/one_layer_neural_network.pdf}

\caption{One-hidden-layer feedforward neural network.}
\label{fig:neural_network}
\end{center}
\vskip -0.2in
\end{figure*}


==> sections/iclr_old/analysis.tex <==
In this section, we solve the task-aware privacy preservation problem. Assuming a linear model and mean-squared error (MSE) task loss, we are able to find near-optimal analytical results, which shed clear insight on how to co-design an encoder and decoder. We then move to general settings and present a heuristic learning algorithm which demonstrates strong empirical performance. 

\subsection{Linear Model with MSE Task Loss} \label{subsec:linear_model}

In this subsection, we consider a linear model with MSE task loss. More specifically, encoder function $g_e$, decoder function $g_d$, and task function $f$ are assumed to be linear functions in their corresponding inputs, and the loss function is $l = \|(\hat{y} - y)\|^2_2$. The task function $f$ can then be expressed as $f(x) = K x$, where $K \in \reals^{m \times n}$ is the task matrix. 
% \cite{?}.

\phead{Practicality of the setting.} Linear transformation is a common encoding and decoding approach for many dimensionality-reduction techniques, such as PCA. And $\ell_2$ task loss is widely used in many application scenarios. 
% I do not fully follow the following example - Kevin
For example, given $N$ samples of $x$, suppose we want to estimate the mean value of these samples in a few directions, given by task matrix $K$. Then the sum of the variance of these estimates by using $\hat{x}$ instead of $x$ will be 
\JC
{
$\frac{1}{N}\E_{x,w}[\|K(\hat{x} - x)\|^2_2]$, so $\loss = \E_{x,w}[\|K(\hat{x} - x)\|^2_2] = \E_{x,w}[\|(\hat{y} - y)\|^2_2]$ is a natural objective function.
}

\phead{Contents.} We first summarize key results. For our task-aware approach, the optimal decoder is first determined in Proposition \ref{prop:opt_decoder}, and then the optimal encoder and the corresponding optimal loss is formulated in Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma} under Assumption \ref{assumption:boundary_h}. We then relax Assumption \ref{assumption:boundary_h} and provide lower and upper bounds for the optimal loss in Theorem \ref{thm:opt_loss_bound} and an approximate solution. 
% For \JC{the task-agnostic and privacy-agnostic approach, the corresponding optimal losses are determined in Corollary \ref{cor:opt_loss_task_agnostic} and \ref{cor:opt_loss_privacy_agnostic}, respectively.} 
All proofs are in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phead{Detailed analysis.} We start our analysis with a few definitions. First, without loss of generality, we assume the covariance matrix of $x-\mu_x$, i.e., $\E[(x-\mu_x)(x-\mu_x)^\top]$, is positive definite, where $\mu_x \in \reals^n$ is the mean vector of $x$. This assumption guarantees $x$ cannot be linear transformed to a low-dimensional representation without losing information. 

We then factorize $\E[(x-\mu_x)(x-\mu_x)^\top]$ into $L L^\top$ through Cholesky decomposition, where $L \in \reals^{n \times n}$ is a lower triangular matrix with positive diagonal entries. For analytical convenience, we let $h = L^{-1}(x-\mu_x)$, which can be viewed as another representation of $x$, with mean $\mu_h = \bm{0}$ and covariance matrix $\Sigma_{hh} = I$. Let $\dist_h$ denote the distribution of $h$, and $H = \{L^{-1}(x-\mu_x) | x \in X\}$ denote the compact set that contains all the possible values of $h \sim \dist_h$. Since $K (\hat{x} - x) = P (\hat{h} - h)$, where $P = K L$, working with data representation $h$ with task matrix $P$ is equivalent to using $x$ and $K$. Considering zero-centered $h$ instead of original $x$ saves us from considering the constant terms in the linear encoder and decoder functions.

Let $E \in \reals^{Z \times n}$ and $D \in \reals^{n \times Z}$  denote the encoder and decoder matrix associated with $h$, i.e., $\phi = E h$ and $\hat{h} = D(E h+w)$. Without loss of generality, we let $Z \geq n$ and allow some rows of $E$ to be zero. Equivalently, based on the relationship between $x$ and $h$, we have $\phi = E L^{-1} (x-\mu_x)$ and $\hat{x}-\mu_x = L D(E L^{-1}(x-\mu_x)+w)$. We denote the covariance matrix of $w$ by $\Sigma_{ww}$, and it can be expressed as $\Sigma_{ww} = \sigma_w^2 I$, where $\sigma_w^2$ is the variance of the noise added to each dimension of $\phi$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first determine the optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$, which is given by the following proposition.

\begin{prop}[Optimal decoder $D$ that minimizes $\loss$]\label{prop:opt_decoder}
An optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$ and $\sigma_w^2$ can be expressed as $D = E^\top (E E^\top + \sigma_w^2 I)^{-1}$, and corresponding $\loss$ is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  E^\top (EE^\top + \sigma_w^2 I)^{-1} E), \label{eq:loss_E}
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. 
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% One can obtain the resultant optimal $\loss$ for the task-agnostic approach by letting $E = L$ and using Eq.\ref{eq:loss_E} as stated in Proposition \ref{prop:opt_decoder}. It is worth noting that the associated decoder $D = L^\top (L L^\top + \sigma_w^2 I)^{-1}$ is not an identity matrix in general. 

% \begin{cor}[Optimal $\loss$ for the task-agnostic approach that preserves $\epsilon$-LDP]\label{cor:opt_loss_task_agnostic}
% For the task-agnostic approach, the optimal $\loss$ that preserves $\epsilon$-LDP is
% \begin{align}
% \loss = \tr(P^\top P) - \tr(P^\top P  L^\top (LL^\top + \sigma_w^2 I)^{-1} L), \label{eq:loss_task_agnostic}
% \end{align}
% where $\sigma_w^2 = 2 (\Delta_1 g_e)^2 / \epsilon^2$ with $g_e(x) = x$. 
% \end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The next main step is to find an encoder $E$ that minimizes Eq.\ref{eq:loss_E}. Since $\Delta_1 g_e = \max_{v, v' \in E(H)} \|v - v'\|_1$, where $E(H) = \{Eh | h \in H\}$ is the image of $H$ under linear transformation $E$, the design of encoder $E$ will affect $\Delta_1 g_e$ and therefore $\sigma_w^2$, and for different $H$'s the effect of $E$ is also different in general. So we need to carefully consider the relationship between $E$ and $H$. 

When computing $\Delta_1 g_e$ we can actually use $H$'s convex hull $S$ instead of $H$ itself, according to the following lemma. This brings some analytical convenience in the further analysis.

\begin{lem}[Convex hull preserves $\Delta_1 g_e$]\label{lem:convex_hull}
\begin{align}
\Delta_1 g_e = \max_{v, v' \in E(S)} \|v - v'\|_1.
\end{align}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For encoder $E$, consider its singular value decomposition (SVD) instead: $U \Sigma V^\top$, where $U \in \reals^{Z \times Z}$ and $V \in \reals^{n \times n}$ are orthogonal matrices and $\Sigma \in \reals^{Z \times n}$ is a rectangular diagonal matrix. And the singular values are denoted by $\sigma_1, \cdots, \sigma_n$ with $|\sigma_1| \geq \cdots \geq |\sigma_n|$. Then designing $E$ is equivalent to designing matrix $U$, $V$ and $\Sigma$. The geometric interpretation of applying transform $E = U \Sigma V^\top$ to set $S$ consists of three sub-transforms: 1) rotate $S$ by applying rotation matrix $V^\top$; 2) scale $V^\top (S)$ by applying scaling matrix $\Sigma$; 3) rotate $\Sigma V^\top (S)$ by applying rotation matrix $U$. In general, the choice of any of $U$, $\Sigma$, and $V$ will affect $\Delta_1 g_e$ and hence $\sigma_w^2$.

Our overall strategy is to first minimize the loss $\loss$ and the sensitivity value $\Delta_1 g_e$ over $U$ and $V$. The resulting $U$ and $V$ only depend on $\Sigma$ under Assumption \ref{assumption:boundary_h} (Propositions \ref{prop:opt_V}, \ref{prop:opt_U}). We then find the optimal $\Sigma$ that minimizes the $\loss$ within a given privacy budget $\epsilon$ (Proposition \ref{prop: opt_sigma}). By the end, we relax Assumption \ref{assumption:boundary_h} to discuss the quality of our solution (Theorem \ref{thm:opt_loss_bound}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We start by noting that for two points within a compact set, they must lay on the boundary to have the maximum $\ell_1$ distance. We then make the following assumption in terms of $\partial S$, which is the boundary of $S$. It decouples the relationship between the choice of $V$ and the value of $\Delta_1 g_e$.

\begin{assumption} [Boundary $\partial S$ is a centered hypersphere] \label{assumption:boundary_h}
The boundary $\partial S$ is a centered hypersphere of radius $r \geq 0$, which is expressed as $\{ h \in \reals^n | \|h\|_2^2 = r^2\}$.
\end{assumption}

This is a strong assumption, but at the end of this subsection we will give a lower and upper bound of $\loss$ for any possible $\partial S$ based on the results under this assumption. Since $\partial V(S) = \{ h \in \reals^n | \|h\|_2^2 = r^2\} = \partial S$ for any orthogonal $V$, this assumption gives us a nice property: the choice of $V$ doesn't affect $\Delta_1 g_e$ and $\sigma_w^2$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Based on the above assumption, we can safely consider the optimal design of $V$ that minimizes $\loss$ when $\Sigma$ and $\sigma_w^2$ are given, which leads to the following proposition.

\begin{prop}[Optimal rotation matrix $V$ that minimizes $\loss$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_V}
Suppose the eigen-decomposition of the Gram matrix $P^\top P$ is expressed as $P^\top P Q = Q \Lambda$, where $\Lambda = \text{diag}(\lambda_1, \cdots, \lambda_n)\in \reals^{n\times n}$ is a diagonal matrix whose diagonal elements are eigenvalues with $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$, and $Q \in \reals^{n \times n}$ is an orthogonal matrix whose columns are corresponding normalized eigenvectors. Then, when $\Sigma$ and $\sigma_w^2$ are given, $\loss$ is minimized for $V = Q$, any $Z \geq n$, and any orthogonal $U$. And the corresponding $\loss$ can be expressed as:
\begin{align}
\loss = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2}. \label{eq:loss_Sigma}
\end{align}
\end{prop}
 
It is clear that choosing a $Z > n$ brings no additional benefit. Hence we can only consider \SC{$Z = n$} for simplicity. 
% \JC{ Further, through similar analysis, one can obtain the resultant optimal $\loss$ for the privacy-agnostic approach, which has a pre-determined $Z \leq n$.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \JC{
% \begin{cor}[Optimal $\loss$ for the privacy-agnostic approach that preserves $\epsilon$-LDP]\label{cor:opt_loss_privacy_agnostic}
% For the privacy-agnostic approach with a pre-determined $Z \leq n$, the optimal $\loss$ that preserves $\epsilon$-LDP is
% \begin{align}
% \loss = \sum_{i=1}^Z \lambda_i \frac{\sigma_w^2}{\sigma_i^2+\sigma_w^2} + \sum_{i=Z+1}^n \lambda_i. \label{eq:loss_privacy_agnostic}
% \end{align}
% where $\sigma_w^2 = 2 (\Delta_1 g_e)^2 / \epsilon^2$.
% \end{cor}
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

After the first two sub-transforms $\Sigma$ and $V^\top$, the boundary $\partial S = \{ h \in \reals^n | \|h\|_2^2 = r^2\}$ becomes $\partial \Sigma V^\top (S) =  \{ v \in \reals^n | \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$, which is a hyperellipsoid. We then have the following proposition that gives the optimal $U$ which minimizes $\Delta_1 g_e$. 

\begin{prop}[Optimal rotation matrix $U$ that minimizes $\Delta_1 g_e$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_U}
For a given $\Sigma$, $U = I$ minimizes $\Delta_1 g_e$, and the corresponding minimum value is
\begin{align}
\Delta_1 g_e = 2r \sqrt{\sum_{i=1}^n \sigma_i^2}. \label{eq:opt_g_e}
\end{align}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we need to consider how to design the scaling matrix $\Sigma$, or equivalently, the values of $\sigma_1^2, \cdots, \sigma_n^2$, to minimize Eq.\ref{eq:loss_Sigma}, which is the only remaining piece. Clearly, for any given $\sigma_1^2, \cdots, \sigma_n^2$ if we increase them proportionally, $\sigma_w^2$ also needs to be increased proportionally to preserve the same $\epsilon$-LDP. So without loss of generality, we impose an additional constraint $\sum_{i=1}^n \sigma_i^2 = M$, where $M$ is a positive constant. And the following proposition gives the optimal choice of $\Sigma$ that minimizes $\loss$ and preserves $\epsilon$-LDP with the Laplace mechanism.

\begin{prop}[Optimal scaling matrix $\Sigma$ that minimizes $\loss$ and preserves $\epsilon$-LDP with Laplace mechanism under Assumption \ref{assumption:boundary_h}]\label{prop: opt_sigma}
The optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $\epsilon$-LDP with Laplace mechanism under constraint $\sum_{i=1}^n \sigma_i^2 = M$ is given by
\begin{align}
\sigma_i^2 = 
\begin{dcases*}
M \cdot (\frac{\sqrt{\lambda_i}}{\sum_{i=1}^{Z'} \sqrt{\lambda_i}}(1+Z'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2}), & $\forall i \in \{1, 2, \cdots, Z'\}$\\
0, & $\forall i \in \{Z'+1, Z'+2, \cdots, n\}$
\end{dcases*} \label{eq:opt_sigma_laplace}
\end{align}
where $Z' \leq n$ is the largest integer such that:
\begin{align}
\frac{\sqrt{\lambda_{Z'}}}{\sum_{i=1}^{Z'} \sqrt{\lambda_i}}(1+Z'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2} > 0, \label{eq:opt_T_laplace}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{8r^2/\epsilon^2}{1 + Z'\cdot8r^2/\epsilon^2} (\sum_{i=1}^{Z'}  \sqrt{\lambda_i})^2 + \sum_{i=Z'+1}^n \lambda_i. \label{eq:loss_laplace}
\end{align}
\end{prop}

For our task-aware approach, Proposition \ref{prop:opt_decoder}-\ref{prop: opt_sigma} complete the optimal encoder and decoder design that preserves $\epsilon$-LDP with the Laplace mechanism under Assumption \ref{assumption:boundary_h}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{figures_latex/fig_theory.tex}

% We now compare the performance of our task-aware approach and the benchmark approaches when $L = I$ and Assumption \ref{assumption:boundary_h} holds. 
% In this case, for the \JC{task-agnostic}
% % benchmark
%  approach, according to Eq. \ref{eq:loss_task_agnostic}, we have
% \begin{align} 
% \loss = \frac{\sigma_w^2}{1 + \sigma_w^2} \cdot \tr(P^\top P) = \frac{n \cdot 8r^2/\epsilon^2}{1 + n \cdot8r^2/\epsilon^2} \sum_{i=1}^n \lambda_i.
% \end{align}
% \JC{
% For the privacy-agnostic approach, according to Eq. \ref{eq:loss_privacy_agnostic} and Eq. \ref{eq:opt_g_e}, and assuming we have equal $\sigma_i$'s and minimum $\delta_1 g_e$, we get
% \begin{align}
% \loss = \frac{Z \cdot 8r^2/\epsilon^2}{1 + Z \cdot 8r^2/\epsilon^2} \sum_{i=1}^{Z} \lambda_i + \sum_{i=Z+1}^n \lambda_i,
% \end{align}
% where the value of $Z$ is pre-determined. 
% }

\phead{\SC{Validation of Task Loss from Theoretical Results (Fig. \ref{fig:theory}).}} We now compare the performance of our task-aware approach and the benchmark approaches when $L = I$ and Assumption \ref{assumption:boundary_h} holds.
\JC{The derivations of the benchmark approaches are in Section \ref{subsec:benchmarks}.}
We consider three different settings which have $n=4$ and $\lambda_1 = 4$ in common. And in setting 1, 2, and 3 we let $\lambda_2 = \lambda_3 = \lambda_4$ be 0, 1, 2 respectively. 
\JC{
For the privacy-agnostic approach\footnote{\label{footnote_privacy_agnostic_z} One can use another value of $Z$, under which the result may be slightly different but our task-aware approach will still outperform.}, we use a pre-determined $Z = 2$.
Our observations are: 1) Compared to the task-agnostic approach, our task-aware approach achieves the largest improvement in setting 1, because $\lambda_{2:4} = 0$ implies that $x_{2:4}$ are purely redundant. We can even expect higher gain than setting 1 when we have larger $n$ and zero $\lambda_{2:n}$'s, and the gain will be zero if all the $\lambda_i$'s are equal. 2) The privacy-agnostic approach completely missed the information carried by $x_{3:4}$, which explains the improvement of our task-aware approach for small $r/\epsilon$ in setting 2 and 3. We can expect higher gain than setting 3 when we have larger $n$ and larger $\lambda_{2:n}$'s, and the gain will be zero if all the missed $x_i$'s correspond to zero $\lambda_i$'s and all the other $\lambda_i$'s are equal.

% , our task-aware approach 
% %The corresponding result is shown in Fig. \ref{fig:theory}. 
% Our observation is that in setting 1, the improvement of our task-aware approach is larger than the other two settings because $\lambda_{2:4} = 0$ implies that $x_{2:4}$ are purely redundant. In setting 2 and 3, our task-aware approach can still outperform the benchmark approach by a small margin. We can expect higher gain than setting 1 when we have larger $n$ and zero $\lambda_{2:n}$'s, and the gain will be zero if all the $\lambda_i$'s are equal.
} 
%\SC{Our subsequent experiments on real-world datasets illustrate significant gains.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phead{Transition to general boundary $\partial S$.} Based on the results under Assumption \ref{assumption:boundary_h}, we can give a lower and upper bound of $\loss^*$ for general $\partial S$, which is not necessarily a centered hypersphere.

\begin{thm}[Lower and upper bound of $\loss^*$ for general boundary $\partial S$ when $\epsilon$-LDP is preserved with Laplace mechanism]\label{thm:opt_loss_bound}
Suppose $\partial S \subset \{ h \in \reals^n: r_\text{min}^2 \leq \|h\|_2^2 \leq r_\text{max}^2\}$. Then when $\epsilon$-LDP is preserved with the Laplace mechanism, the optimal $\loss^*$ is bounded by:
\begin{align}
\loss(r_\text{min}; \lambda_{1:n}, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_{1:n}, \epsilon)
% \loss(r_\text{min}; \lambda_1, \cdots, \lambda_n, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_1, \cdots, \lambda_n, \epsilon)
\end{align}
where $\loss(r; \lambda_{1:n}, \epsilon)$ is the value of $\loss$ determined by Eq.\ref{eq:opt_T_laplace} and \ref{eq:loss_laplace} for given radius $r$, eigenvalues $\lambda_{1:n}$ and privacy budget $\epsilon$.
\end{thm}

Therefore, to preserve $\epsilon$-LDP with the Laplace mechanism, our task-aware solution for general $\partial S$ is: 1) First, find the smallest $r_\text{max}$ and the largest $r_\text{min}$ that bound $\partial S$; 2) Then assume $\partial S$ is $\{ h \in \reals^n | \|h\|_2^2 = r_\text{max}^2\}$, and choose the encoder $E$ and decoder $D$ based on Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma}. We don't use the corresponding $\sigma_w^2$ however, because it may guarantee a higher LDP than needed. 3) Next, compute $\sigma_w^2$ for real $\partial S$ under decoder $D$ and privacy budget $\epsilon$. 

The associated loss for the task-aware approach is at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon)$. Though in general not optimal, it differs from $\loss^*$ by at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon) - \loss(r_\text{min}; \lambda_{1:n}, \epsilon)$. 
\SC{The difference is small when $\partial S$ is ``nearly'' a hypersphere, i.e., $r_\text{max} - r_\text{min} \approx 0$.} 
%(Remember we also have $\mu_h = \bm{0}$ and $\Sigma_{hh} = I$. Even though it may not provide any guarantees on $r_\text{max} - r_\text{min}$, for $h$ associated with real datasets we don't expect $r_\text{max} - r_\text{min}$ to be large, either.)}

% old
%The difference is small when $\partial S$ is ``nearly'' a hypersphere, i.e., $r_\text{max} - r_\text{min} \approx 0$. (Remember we also have $\mu_h = \bm{0}$ and $\Sigma_{hh} = I$. Even though it may not provide any guarantees on $r_\text{max} - r_\text{min}$, for $h$ associated with real datasets we don't expect $r_\text{max} - r_\text{min}$ to be large, either.)

\subsection{General Settings} \label{subsec:general_settings}

For more complex scenarios, it is challenging to give an analytical solution to the task-aware privacy preservation problem, especially when the encoder function $g_e$, decoder function $g_d$, and task function $f$ correspond to neural networks. Thus, we present a heuristic learning algorithm. \JC{(The benchmark algorithms are given in Section \ref{subsubsec:benchmark_algorithms} due to space limit.)}

% \phead{Task-aware.} 
Algorithm \ref{alg:ldp_codesign} is our proposed task-aware algorithm for general settings. First, the privacy budget $\epsilon$ and the latent dimension $Z$ are required inputs for the algorithm. \JC{In general, $Z$ should be proper, i.e., it is neither too small (we can find a better solution by choosing a larger $Z$) nor too big (which introduces unnecessary complexity). In practice a practitioner may need to determine a proper $Z$ on a case-by-case basis (See Section \ref{subsec:proper_z} of the Appendix for more details).}
% In general, $Z$ should be large so that it is not the bottleneck. In other words, we won't find a better solution by choosing a larger $Z$. $Z = n$ usually suffices.
Next, the algorithm adopts an alternating iteration approach, where in each epoch, we first update parameters $\theta_e$, $\theta_d$ by their corresponding negative gradients in line 3, and then recompute $\Delta_1 g_e$ and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$ in line 4. Note that, in terms of encoder parameter $\theta_e$, instead of considering the gradient of $\loss$, we add an $\ell_2$ regularization term $\eta \|\theta_e\|^2$ where $\eta$ is a positive constant. Therefore, we update $\theta_e$ with the negative gradient $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$. Without regularization, the $\|\theta_e\|^2$ will grow to infinity since we can always achieve a smaller $\loss$ by increasing the scale of $\phi$ proportionally. But it is not a direction we are looking for, since $\sigma_w^2$ will also increase proportionally to guarantee $\epsilon$-LDP.  

% \phead{Benchmarks.} 

% \JC{
% For the privacy-agnostic approach, we first train the encoder and decoder without considering privacy preservation by updating $\theta_e$ and $\theta_d$ with $- \nabla_{\theta_e} \loss$ and $- \nabla_{\theta_d} \loss$, respectively. Next, we fix encoder parameters $\theta_e$ and train the decoder with input $\phi + w$ (a modification of Algorithm \ref{alg:ldp_codesign} line 3-4). The task-agnostic approach trains the decoder in the same way, but fixes $g_e$ to an identity mapping function.
% }

% The algorithm used for the benchmark approach only differs from Algorithm \ref{alg:ldp_codesign} in line 3. Since $g_e$ is fixed to an identity mapping, we only need to update $\theta_d$ with $- \nabla_{\theta_d} \loss$ by one or multiple steps in line 3. In line 4, although $\Delta_1 g_e$ remains unchanged, we still re-sample $w$ to avoid overfitting. 

% \begin{wrapfigure}{L}{0.5\textwidth}
% \begin{minipage}{0.5\textwidth}

% \begin{algorithm}[H]
% \begin{algorithm}[tb]
%    \caption{Task-aware Algorithm for $\epsilon$-LDP Preservation in General Settings}
%    \label{alg:ldp_codesign}
%    \begin{algorithmic}[1]
%         \Require Privacy budget $\epsilon$ and $Z$
%         \State Initialize encoder/decoder parameters $\theta_e, \theta_d$ and noise vector $w$
%         \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
%              \State Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
%              \State Recompute $\Delta_1 g_e$, and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$
%         \EndFor
%         \State Return $\theta_e, \theta_d$ and $\Delta_1 g_e$
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]
   \caption{Task-aware Algorithm for $\epsilon$-LDP Preservation in General Settings}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \REQUIRE Privacy budget $\epsilon$ and $Z$
        \STATE Initialize encoder/decoder parameters $\theta_e, \theta_d$ and noise vector $w$
        \FOR{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \STATE Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
             \STATE Recompute $\Delta_1 g_e$, and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$
        \ENDFOR
        \STATE Return $\theta_e, \theta_d$ and $\Delta_1 g_e$
    \end{algorithmic}
\end{algorithm}

% \end{minipage}
% \end{wrapfigure}


==> sections/iclr_old/conclusion.tex <==
This paper provides a principled task-aware privacy preservation method to improve the privacy-utility trade-off for ML tasks that increasingly operate on rich, multi-dimensional user data. 
% as the dimension and complexity of rich user data grows.
%In this paper, we considered a task-aware privacy preservation problem based on an encoder-decoder framework. 
We gave an analytical near-optimal solution for a general linear encoder-decoder model and MSE task loss, and developed a heuristic learning algorithm for more general nonlinear settings. Our evaluation showed that our task-aware approach outperforms the benchmark approaches on overall task loss under various LDP budgets. 
Our future work will focus on the analysis of the task-aware privacy preservation problem for approximate LDP and other LDP mechanisms as well as multi-task learning. 


==> sections/iclr_old/evaluation.tex <==
Our evaluation compares the performance of the proposed task-aware approach and the benchmark approaches. Three applications and corresponding datasets from the standard UCI Machine Learning Repository \citep{uci} are considered: mean estimation of hourly household power consumption, real estate valuation, and breast cancer detection. Configuration and training details are provided in the appendix due to space limitations.

%\subsection{Mean Estimation of Hourly Household Power Consumption}
\phead{Mean Estimation of Hourly Household Power Consumption.}
We first consider a mean estimation problem, based on  measurements of individual household electric power consumption over four years \citep{hebrail2012individual}. Each data sample $x \in \reals^{24}$ is a time-series that contains the hourly household power consumption for one single day, and our objective is to estimate the mean of the hourly household power consumption for $N$ days. As discussed in Section \ref{subsec:linear_model}, we can define the overall task loss in the following way: 
\begin{align}
\loss = \E_{x \sim \dist_x}[\|K(\hat{x} - x)\|^2_2] = \sum_{i=1}^{24} k_i^2 \E_{x \sim \dist_x}[\|\hat{x}_i - x_i\|^2_2]
\end{align}
where $K = \text{diag}(k_1, k_2, \cdots, k_{24})$ factors the importance of the mean estimation for each hour. In our experiment we set $k_i = 2$ for $i \in \{9, 10, \cdots, 20\}$ (i.e., day-time hours) and $k_i = 1$ for other $i$'s (i.e., night-time hours). And we adopt a linear encoder and decoder model. As the considered problem is based on a linear model with MSE task loss, we adopt the solutions developed in Section \ref{subsec:linear_model} for the three approaches (we choose $Z = 3$ for the privacy-agnostic approach).

% \footref{footnote_privacy_agnostic_z}

\input{figures_latex/fig_household.tex}

Fig. \ref{fig:household} shows our experimental results. First, on the left, we compare the task loss $l(\hat{y}, y)$ for the three approaches under different LDP budgets. For each approach, the overall task loss $\loss$ decreases when a larger LDP budget $\epsilon$ is given. Besides, for a given LDP budget, our task-aware approach always outperforms the benchmark approaches on overall task loss $\loss$, 
\JC{and the maximum improvements against the task-agnostic and privacy-agnostic approach are $22.9\%$ ($\epsilon = 10$) and $11.7\%$ ($\epsilon = 5$), respectively.}
Second, on the right, we select $\epsilon = 5$ and compare the MSE of power consumption for each hour. We see that our task-aware approach achieves a lower MSE for all the day-time hours, and a similar MSE for the night-time hours. This observation can be explained by three reasons: 1) We select a higher $k_i$ for the day-time hours, so our task-aware approach gives higher priority to minimizing the loss for those dimensions in $x$; 2) Although $x$ has 24 dimensions, the variance in each dimension can be mostly explained by several common latent dimensions, so our task-aware approach still achieves a similar MSE for the night-time hours; \JC{3) Our task-aware approach is able to adopt different scales to different latent dimensions according to their task relevance while the privacy-agnostic approach cannot.} 

%\subsection{Real Estate Valuation and Breast Cancer Detection}

Next, we consider a real estate valuation problem and a breast cancer detection problem. Both the problems are not based on the linear model with MSE task loss, so we use Algorithm \ref{alg:ldp_codesign} developed in Section \ref{subsec:general_settings} to solve them \JC{(we use $Z = 3$ for both our task-aware approach and the privacy-agnostic approach for fair comparison; and the performance of the task-aware approach under different $Z$'s can be found in Section \ref{subsec:proper_z} of the Appendix)}.

\phead{Real Estate Valuation.} For this problem, we use historical real estate valuation data collected from Taiwan \citep{yeh2018building}, which contains 400+ instances. Here, $x \in \reals^6$ contains 6 attributes that are highly related to the value of a house, including transaction date, house age, geographic coordinates, etc. And $y \in \reals$ represents the valuation of a house. We first train a one-hidden-layer feedforward neural network regression model using the ground truth $x$ and $y$, to serve as our task function $f$. Then, we minimize the $\ell_2$ loss of $\hat{y}$ and $y$, based on a linear encoder and decoder model.

\phead{Breast Cancer Detection.} For this problem, we use a well-known breast cancer diagnostic dataset \citep{street1993nuclear} from Wisconsin, which contains 500+ instances. Here, $x \in \reals^{30}$ contains 30 attributes that measure 10 features of a cell nucleus. And $y$ is a binary variable that represents a diagnosis result (malignant or benign). We first train a one-hidden-layer feedforward neural network classification model using the ground truth $x$ and $y$, to serve as our task function $f$. Then we aim to minimize the cross-entropy loss of $\hat{y}$ and $y$, with encoder and decoder both being one-hidden-layer feedforward neural networks.

\input{figures_latex/fig_ml.tex}

Fig. \ref{fig:ml} shows the evaluation results. For both problems, we can see our task-aware approach nearly always outperforms the benchmark approaches on overall task loss $\loss$ under different LDP budgets, which demonstrates the effectiveness of our proposed solution. \JC{The maximum improvements against the task-agnostic and privacy-agnostic approach are $26.1\%$ ($\epsilon = 10$) and $21.2\%$ ($\epsilon = 5$) for real estate valuation, and are $70.0\%$ ($\epsilon = 100$) and $68.5\%$ ($\epsilon = 100$) for breast cancer detection.} 

% We also see the classification model used for the cancer detection problem is more vulnerable to noise, since both approaches end up with high classification loss for $\epsilon = 5$, which is a relatively large privacy budget compared to the mean estimation and real estate valuation problems.

% \phead{Limitations.} Further research is required to learn anonymized representations that are useful for \textit{multiple} tasks. Moreover, our theoretical guarantees do not apply to general deep neural networks.


==> sections/iclr_old/intro.tex <==
In recent years, there has been a tremendous growth in the volume of available data for machine learning (ML) tasks, leading to increasing emphasis on protecting user privacy. Differential privacy (DP) \citep{dwork2006calibrating,dwork2014algorithmic} is a state-of-the-art technique for data privacy, and its local variant -- local differential privacy (LDP) \citep{kasiviswanathan2011can} -- provides stronger privacy guarantees for individual users without dependence on any trusted third party. In practice, LDP has been successfully deployed in products of companies like Google \citep{erlingsson2014rappor}, Apple \citep{apple2021dp}, and Microsoft \citep{ding2017collecting} for some basic frequency or histogram estimation tasks where raw user data is restricted to an $n$-bit discrete variable.  

In the future, LDP has the promising potential to be adopted in more complex scenarios \citep{hassan2019differential,dankar2013practicing,zhao2014achieving,cortes2016differential} (e.g., health care, power grids, Internet of Things) that feature richer user data attributes that feed into more sophisticated downstream ML tasks. In such cases, today's standard task-agnostic LDP approaches may not be ideal. For example, consider complex user data that must be anonymized before passing it into a ML task function, such as a neural network classifier for credit scores. A standard approach would be to simply perturb the data by adding artificial noise whose scale depends on the sensitivity of user data (i.e. worst-case variation among a user population) and a given privacy budget, \textit{regardless} of what ultimate task the anonymized data will be used for. However, as the dimension and variability of user data inevitably grows, today's methods would generally have to increase the scale of noise to provide the same LDP guarantee, even though many data attributes might be highly variable across a user population, but minimally \textit{relevant} for a task. As a consequence, one often adds excessive noise to all data attributes, which can severely degrade an ultimate task's performance. 
%or will require an excessive amount of data samples to achieve the same task performance. 

%\input{figures_latex/fig_architecture.tex}

To address these challenges, this paper introduces a fundamentally different \textit{task-aware} LDP approach. Our method improves the performance of ML tasks that operate on multi-dimensional user data while still guaranteeing the same levels of privacy. 
Our key technical insight is to characterize the dependence of task performance on various user data attributes, which guides how we \textit{learn} a concise, task-relevant encoding (i.e. latent representation) of user data. Then, for the same privacy budget, we can directly expose and perturb only the task-relevant encoding rather than raw user data, which often allows us to add less noise and thereby improve task accuracy (see Section 2 for a concrete example).
Crucially, user privacy is guaranteed under the same privacy budget according to the post-processing immunity of DP \citep{dwork2014algorithmic} (i.e., one cannot make the output of a privacy algorithm less differentially private without additional knowledge). As such, an adversary cannot decode the anonymized latent representation to reduce the level of privacy.
Our method allows us to learn and expose only high-valued data attributes and flexibly adjust their signal-to-noise ratio based on their importance to a task. 
Moreover, when different data attributes are inter-dependent, task-aware LDP preservation is even more promising in that we can consider the utilities of the underlying orthogonal bases through principal component analysis (PCA) \citep{dunteman1989principal}, instead of the raw data attributes.

\phead{Contributions.} In light of prior work, our contributions are three-fold. First, we propose a task-aware privacy preservation problem 
\JC{ 
in which the effect of noise perturbation to preserve LDP is effectively considered, based on an encoder-decoder framework (Section \ref{sec:problem_formulation}). 
}
% which aims at minimizing the overall task loss under a given LDP budget (Section \ref{sec:problem_formulation}).
Second, in terms of task-aware privacy preservation, we obtain an analytical near-optimal solution for a linear setting and MSE task loss, and provide a heuristic learning algorithm for more general settings (Section \ref{sec:analysis}). Third, we validate the effectiveness of our task-aware approach through three real-world experiments, which show our task-aware approach outperforms the benchmark approaches on overall task loss under various LDP budgets by as much as \JC{$70.0\%$} (Section \ref{sec:evaluation}). 
All the proofs are given in the Appendix. 

\phead{Related Work.} 
1) \underline{Utility maximization in DP/LDP}. Most theoretical DP/LDP research either provides a utility upper bound for a given privacy budget under some weak assumptions \citep{alvim2011differential,kenthapadi2012privacy,duchi2013local,makhdoumi2013privacy,hardt2010geometry,wang2019subsampled,acharya2020context}, or designs optimal privacy preservation mechanisms in some specific use cases \citep{mcsherry2007mechanism,wasserman2010statistical,friedman2010data,xiao2010differential,thakurta2013differentially,kairouz2014extremal,geng2015optimal,liu2016dependence,yiwen2018utility,joseph2019role,gondara2020differentially,wang2020empirical}. To the best of our knowledge, with respect to \textit{multi-dimensional user data}, \JC{\citet{murakami2019utility}, \citet{wang2019collecting} and \citet{chen2021perceptual} are the only three similar works to ours.}
% old 
\citet{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be \SC{privacy-sensitive}, and hence the utility improvement is mainly achieved by providing privacy guarantees \SC{for only a subset of attributes}. 
\citet{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally \SC{improves} utility.
\JC{
\citet{chen2021perceptual} preserves DP for images by adding noise to a latent representation learned through back-propagation of task loss, where the effect of noise perturbation is not considered.
}
The key differences of our work are: i) we don't make additional assumptions on the sensitivity of user data, ii) our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data, \JC{and iii) we effectively capture the effect of noise perturbation resulting from privacy requirements.}
% old 
%\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be sensitive, and hence the utility improvement is mainly achieved by providing different privacy guarantees. 
%\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally leads to a better utility. 
%The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
2) \underline{End-to-end (E2E) learning}. There has been a wide variety of works training a cascade of deep neural networks (DNNs) through E2E learning, where a task-specific output is directly predicted from the raw inputs \citep{muller2006off,wang2012end,donti2017task,zhou2018voxelnet,amos2018differentiable}. Our work also follows such a practice, but introduces an LDP guarantee while improving the task performance.
3) \underline{DP in deep learning}. The popularity of deep learning also draws great attention to DP preservation therein \citep{song2013stochastic,shokri2015privacy,abadi2016deep,phan2016differential,papernot2016semi,phan2017adaptive,mcmahan2018general,wang2018not,phan2019heterogeneous,arachchige2019local,liu2020fedsel,mireshghallah2020principled,bu2020deep}. Our work is fundamentally different. Instead of preserving LDP \textit{during the learning process}, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. \JCC{In other words, we don't perturb the gradient for back-propagation but perturb the representation to guarantee LDP. Furthermore,} we don't specifically deal with privacy preservation during the \textit{offline} training process, which requires some ground truth user data (\SC{e.g., from a small set of consenting volunteers)}. 
However, LDP of user data is guaranteed after a trained model is deployed \textit{online}.


==> sections/iclr_old/motivation.tex <==
% \subsection{Background}

\phead{$\epsilon$-LDP \citep{kasiviswanathan2011can}.} Let $x \in \reals^n$ be an individual data sample, and $X$ be the domain of $x$, which is assumed to be a compact subset of $\reals^n$. A randomized algorithm $\mathcal{M}: X \mapsto \reals^d$ is said to satisfy $\epsilon$-LDP with \SC{\textit{privacy-budget}} $\epsilon>0$, if 
\begin{align}
\Pr[\mathcal{M}(x) \in \mathcal{S}] \leq e^\epsilon \Pr[\mathcal{M}(x') \in  \mathcal{S}], \quad \forall x, x' \in X, \mathcal{S}  \subseteq \text{im} ~\mathcal{M}.  
\end{align}
Essentially, when $\epsilon$ is small, one cannot readily differentiate whether the input of $\mathcal{M}$ is an individual user $x$ or $x'$ based on $\mathcal{M}$'s outcome. 
% either rephrase or don't keep - this is is not clear
%\SC{When $\epsilon$ is small and for any two indivduals $x$ and $x'$, we have $\Pr[\mathcal{M}(x) \in \mathcal{S}] \approx e \Pr[\mathcal{M}(x') \in \mathcal{S}]$}. 
% This means that one cannot readily differentiate whether the input of $\mathcal{M}$ is $x$ or $x'$ based on its outcome. 

\phead{Laplace mechanism \citep{dwork2014algorithmic}.} To release a sensitive function $g: X \mapsto \reals^d$ under $\epsilon$-LDP, $\forall \epsilon > 0$, the Laplace mechanism is a widely used mechanism which adds Laplace noise to function $g$:
\begin{align}
\mathcal{M}_\text{Lap}(x, g, \epsilon) & = g(x) + \text{Lap}^d(\mu = 0, b = \frac{\Delta_1 g}{\epsilon}), \label{eq:lap}
\end{align}
where $\text{Lap}^d(\mu, b)$ is a $d$-dimensional vector whose elements are i.i.d. Laplace random variables with mean $\mu$ and scale $b$, which \SC{leads} its variance to be $2b^2$. 
%For concreteness, the analysis and evaluation of this paper focus on the Laplace mechanism although the central idea is applicable to other random privacy preservation algorithms as well.
\SC{For concreteness, the analysis and evaluation of this paper focus on the Laplace mechanism although the central idea of learning task-relevant data representations is applicable to other random privacy mechanisms as well.}
$\Delta_1 g = \max_{x, x' \in X} \| g(x) - g(x')\|_1$ measures the sensitivity of $g$ under the $\ell_1$ norm.


% \subsection{Motivating Example}

\input{figures_latex/fig_motivation.tex}

% \paragraph{A Motivating example.} 

\phead{A motivating example.} Consider an example shown in Fig. \ref{fig:motivation}. For simplicity, we only consider an example with two people, Alice and Bob, and two data attributes, age and wage. Suppose we need to preserve $\epsilon$-LDP for each person with $\epsilon = 1$ and our task is to estimate the mean wage as closely as possible. A straightforward task-agnostic approach will directly expose both the two data attributes, and add Laplace noise with scale $b = 20$ to each attribute. However, a task-aware approach will expose only the wage attribute and add Laplace noise with scale $b = 10$. Both the approaches guarantee LDP under the same budget ($\epsilon=1$), but the wage attribute given by the task-aware approach is less noisy, and we can expect that the corresponding estimated mean wage (i.e. the ultimate task objective) is close to the real value with a higher probability.
%\SC{By injecting less noise, a task-aware privacy-preservation approach can often improve a downstream task's performance, such as mean wage estimation, but with the same guaranteed LDP budget.}

In more complex scenarios, such as when each data attribute is not redundant but is valued differently in terms of the considered task or data attributes are dependent but not perfectly correlated, etc., the optimal solution will not be as straightforward as the given example and will be explored in the following sections.


==> sections/iclr_old/problem_formulation.tex <==
% for jiangnan, uncomment
% for sandeep intro, keep here
\input{figures_latex/fig_architecture.tex}

We now introduce the task-aware privacy preservation problem \SC{depicted in Fig. \ref{fig:architecture}}. Let $y = f(x) \in \reals^m$ denote the task output associated with each ground truth data sample $x$, where $f$ represents the task function. To guarantee $\epsilon$-LDP for each data sample $x$, its true value should never be exposed to the task function. Instead, an estimate of $x$, denoted by $\hat{x}$, is used as the input to the task function with the corresponding task output $\hat{y} = f(\hat{x})$. The objective is to minimize the overall task loss
\JC{
$\loss = \E[l(\hat{y}, y)]$ due to the difference between $\hat{x}$ and $x$, where $x$ follows distribution $\dist_x$,
}
% $\loss = \E_{x \sim \dist_x}[l(\hat{y}, y)]$ due to the difference between $\hat{x}$ and $x$, where $\dist_x$ is the distribution of $x$, 
and $l$ is a task loss function that captures the discrepancy between task output $\hat{y}$ and $y$, such as the common $\ell_2$ and cross-entropy loss.
%Common examples of this function include the $\ell_2$ loss and cross-entropy loss.

More concretely, $x$ is first mapped to a latent representation $\phi \in \reals^Z$ through an encoder function $\phi = g_e(x; \theta_e)$, where $\theta_e$ are \SC{a set of encoder parameters}. $\phi$ is then perturbed  by a Laplace noise vector $w \in \reals^Z$. That is, $g_e$ is treated as the sensitive function $g$ in Eq.\ref{eq:lap}. Next, $\hat{x}$ is reconstructed from $\phi + w$ using a decoder function $\hat{x} = g_d(\phi+w; \theta_d)$ where $\theta_d$ are \SC{a set of decoder parameters}. \JCC{Note that in reality the encoder is deployed at the end of each individual user and in general has to be lightweight (e.g., linear or one hidden-layer neural network).} 
%The overall diagram is shown in Fig \ref{fig:architecture}.

The optimal task-aware $\hat{x}$ minimizes $\loss$ while preserving $\epsilon$-LDP. In other words, the task-aware privacy preservation problem aims to co-design encoder and decoder, i.e., find proper values for $Z$, $\theta_e$ and $\theta_d$, such that $\loss$ is minimized and $\epsilon$-LDP is preserved. Formally,
\begin{align}
\min_{Z, \theta_e, \theta_d} \quad & \loss = \E_{x,w} [l(\hat{y}, y)],\label{eq:ldp_problem_begin}\\
\text{s.t.} \quad & y = f(x), \\
&\hat{y} = f(g_d(g_e(x; \theta_e)+w; \theta_d)),\\
& x \sim \dist_x, w \sim \text{Lap}^Z(0, \frac{\Delta_1 g_e}{\epsilon}). \label{eq:ldp_problem_end}
\end{align}

The difficulty of our task-aware LDP problem mainly comes from the discrepancy of the measurement of overall task loss $\loss$, which depends on $\dist_x$ and captures the \textit{average} performance, and the mechanism of preserving LDP, which depends on $X$ and focuses only on the \textit{worst-case} privacy guarantee.
% \JC{
% Moreover, two benchmark approaches -- \textbf{task-agnostic approach} and \textbf{privacy-agnostic approach} are described in \ref{subsec:benchmarks} due to space limit.
% }

\phead{Benchmarks.}
\JC{
We now describe two natural approaches to preserve $\epsilon$-LDP. First, a \textbf{task-agnostic approach} adds noise directly to the normalized $x$\footnote{We may either normalize each dimension independently when $x$ is a multi-variate random variable, or normalize all the dimensions jointly when $x$ is a uni-variate time-series.}. For convenience we assume $x$ is already normalized, and we have $Z = n$ and $g_e(x) = x$. Second, a \textbf{privacy-agnostic approach} adds noise to $\phi$ obtained by considering the problem defined in Eq.\ref{eq:ldp_problem_begin}-\ref{eq:ldp_problem_end} with a pre-determined $Z \leq n$ and $w$ being a zero vector instead. That is, the privacy-preservation part is neglected when designing the encoder, and hence a proper $Z$ needs to be pre-determined or one would always conclude a larger $Z$ (under which more information can be delivered when noise is absent) is better. Both two benchmark approaches still need to determine the optimal decoder parameters $\theta_d$ for input $\phi + w$. Note that for the task-agnostic approach even though $g_e$ is an identity function, the corresponding optimal $g_d$ is usually not an identity function, as exemplified in Section \ref{subsubsec:task_loss_task_agnostic}.
}

% A natural approach is to preserve $\epsilon$-LDP by adding noise directly to the normalized $x$\footnote{We may either normalize each dimension independently when $x$ is a multi-variate random variable, or normalize all the dimensions jointly when $x$ is a uni-variate time-series.}, which we refer to as the \textbf{task-agnostic} benchmark. Here, for convenience, we assume $x$ is already normalized, so we always have $Z = n$ and $g_e(x) = x$. The benchmark approach only needs to determine the optimal decoder parameters $\theta_d$. Note that even though $g_e$ is an identity function, the corresponding optimal $g_d$ is usually not an identity function, as exemplified in Section \ref{subsec:linear_model}.


==> sections/jiangnan/abstract.tex <==
  Local differential privacy (LDP), a state-of-the-art technique for privacy preservation, has been successfully deployed in a few real-world applications. It can be envisioned that, in the future, LDP will be adopted in more complex scenarios where richer user data attributes are available and more complicated tasks are considered, in which case a task-agnostic LDP preservation approach may not be favorable. In this paper, we focus on how to improve the task performance for multi-dimensional user data by considering a task-aware privacy preservation problem. We present a task-aware approach based on an encoder-decoder framework, which gives an analytical near-optimal solution for a linear setting with an MSE task loss, and provides an approximate solution through a heuristic learning algorithm for more general nonlinear settings. Our evaluation demonstrates that the proposed task-aware approach outperforms a standard benchmark approach on overall task loss under various LDP budgets.


==> sections/jiangnan/analysis.tex <==
In this section, we solve the task-aware privacy preservation problem. Assuming a linear model and mean-squared error (MSE) task loss, we are able to find near-optimal analytical results, which shed clear insight on how to co-design encoder and decoder. We then move to general settings and present a heuristic learning algorithm which demonstrates strong empirical performance. 

\subsection{Linear Model with MSE Task Loss} \label{subsec:linear_model}

In this subsection, we consider a linear model with MSE task loss. More specifically, encoder function $g_e$, decoder function $g_d$ and task function $f$ are assumed to be linear functions in their corresponding inputs, and the loss function is $l = \|(\hat{y} - y)\|^2_2$. The task function $f$ can then be expressed as $f(x) = K x$, where $K \in \reals^{m \times n}$ is the task matrix \cite{?}.

\paragraph{Practicality of the setting.} Linear transformation is a common encoding and decoding approach for many dimension-reduction techniques, such as PCA. And $\ell_2$ task loss is widely used in many application scenarios. 
% I do not fully follow the following example - Kevin
For example, given $N$ samples of $x$, suppose we want to estimate the mean value of these samples in a few directions, given by task matrix $K$. Then the sum of the variance of these estimations by using $\hat{x}$ instead of $x$ will be $\frac{1}{N}\E_{x \sim \dist_x}[\|K(\hat{x} - x)\|^2_2]$, so $\loss = \E_{x \sim \dist_x}[\|K(\hat{x} - x)\|^2_2] = \E_{x \sim \dist_x}[\|(\hat{y} - y)\|^2_2]$ is a natural objective function.

\paragraph{Contents.} We first summarize key key results. For our task-aware approach, the optimal decoder is first determined in Proposition \ref{prop:opt_decoder}, and then the optimal encoder and the corresponding optimal loss is formulated in Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma} under Assumption \ref{assumption:boundary_h}. We then relax Assumption \ref{assumption:boundary_h} and provide lower and upper bounds for the optimal loss in Theorem \ref{thm:opt_loss_bound} and an approximated design solution. For the benchmark approach, the corresponding optimal loss is determined in Corollary \ref{cor:opt_loss_benchmark}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Detailed analysis.} We start our analysis with a few definitions. First, without loss of generality, we assume the covariance matrix of $x-\mu_x$, i.e., $\E[(x-\mu_x)(x-\mu_x)^\top]$, is positive definite, where $\mu_x \in \reals^n$ is the mean vector of $x$. This assumption guarantees $x$ cannot be linear transformed to a low-dimensional representation without losing information. 

We then factorize $\E[(x-\mu_x)(x-\mu_x)^\top]$ into $L L^\top$ through Cholesky decomposition, where $L \in \reals^{n \times n}$ is a lower triangular matrix with positive diagonal entries. For analytical convenience, we let $h = L^{-1}(x-\mu_x)$, which can be viewed as another representation of $x$, with mean $\mu_h = \bm{0}$ and covariance matrix $\Sigma_{hh} = I$. Let $\dist_h$ to denote the distribution of $h$, and $H = \{L^{-1}x | x \in X\}$ to denote the compact set that contains all the possible values of $h \sim \dist_h$. Since $K (\hat{x} - x) = P (\hat{h} - h)$, where $P = K L$, it is equivalent to considering data representation $h$ with task matrix $P$ for our task-aware privacy preservation problem. Considering zero-centered $h$ instead of original $x$ saves us from considering the constant terms in the linear encoder and decoder functions.

Let $E \in \reals^{Z \times n}$ and $D \in \reals^{n \times Z}$  denote the encoder and decoder matrix associated with $h$, i.e., $\phi = E h$ and $\hat{h} = D(E h+w)$. Without loss of generality, we let $Z \geq n$ and allow some columns of $E$ be zero. Equivalently, based on the relationship between $x$ and $h$ we have $\phi = E L^{-1} (x-\mu_x)$ and $\hat{x}-\mu_x = L D(E L^{-1}(x-\mu_x)+w)$. We also use $\Sigma_{ww}$ to denote the covariance matrix of $w$, and it can be expressed as $\Sigma_{ww} = \sigma_w^2 I$, where $\sigma_w^2$ is the variance of the noise we will add to each dimension of $\phi$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first determine the optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$, which is given by the following proposition.

\begin{prop}[Optimal decoder $D$ that minimizes $\loss$]\label{prop:opt_decoder}
An optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$ and $\sigma_w^2$ can be expressed as $D = E^\top (E E^\top + \sigma_w^2 I)^{-1}$, and corresponding $\loss$ is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  E^\top (EE^\top + \sigma_w^2 I)^{-1} E), \label{eq:loss_E}
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. 
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We can get the resulted optimal $\loss$ for our benchmark apporach by letting $E = L$ and plug it into Eq.\ref{eq:loss_E}. The associated decoder $D = L^\top (L L^\top + \sigma_w^2 I)^{-1}$ is not an identity matrix in general.
\begin{cor}[Optimal $\loss$ for the benchmark approach that preserves $\epsilon$-LDP]\label{cor:opt_loss_benchmark}
For the benchmark approach, the optimal $\loss$ that preserves $\epsilon$-LDP is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  L^\top (LL^\top + \sigma_w^2 I)^{-1} L), \label{eq:loss_benchmark}
\end{align}
where $\sigma_w^2 = 2 (\Delta_1 g_e)^2 / \epsilon^2$ with $g_e(x) = x$. 
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For our task-aware approach, our next step is to design an encoder $E$ that minimizes Eq.\ref{eq:loss_E}. Since $\Delta_1 g_e = \max_{v, v' \in E(H)} \|v - v'\|_1$, where $E(H) = \{Eh | h \in H\}$ is the image of $H$ under linear transformation $E$, the design of encoder $E$ will affect $\Delta_1 g_e$ and further $\sigma_w^2$, and for different $H$'s the effect is also different in general. So we need to carefully consider the relationship between $E$ and $H$. 

For set $H$, when computing $\Delta_1 g_e$ we can actually use its convex hull $S$ instead, according to the following lemma. It brings us some convenience in the further analysis.

\begin{lem}[Convex hull preserves $\Delta_1 g_e$]\label{lem:convex_hull}
\begin{align}
\Delta_1 g_e = \max_{v, v' \in E(S)} \|v - v'\|_1.
\end{align}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For encoder $E$, we find it helpful to consider its singular value decomposition (SVD) instead: $U \Sigma V^\top$, where $U \in \reals^{Z \times Z}$ and $V \in \reals^{n \times n}$ are orthogonal matrices and $\Sigma \in \reals^{Z \times n}$ is a rectangular diagonal matrix. And the singular values are denoted by $\sigma_1, \cdots, \sigma_n$ with $|\sigma_1| \geq \cdots \geq |\sigma_n|$. Then designing $E$ is equivalent to designing matrix $U$, $V$ and $\Sigma$. The geometric interpretation of applying transform $E = U \Sigma V^\top$ to set $S$ consists of three sub-transforms: 1) rotate $S$ by applying rotation matrix $V^\top$; 2) scale $V^\top (S)$ by applying scaling matrix $\Sigma$; 3) rotate $\Sigma V^\top (S)$ by applying rotation matrix $U$. In general, the choice of any of $U$, $\Sigma$ and $V$ will affect $\Delta_1 g_e$ and hence $\sigma_w^2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We know that for two points within a compact set, they must lay on the boundary to have the maximum $\ell_1$ distance. So next, we make the following assumption in terms of $\partial S$, which is the boundary of $S$. It decouples the relationship between the choice of $V$ and the value of $\Delta_1 g_e$.

\begin{assumption} [Boundary $\partial S$ is a centered hypersphere] \label{assumption:boundary_h}
The boundary $\partial S$ is a centered hypersphere of radius $r \geq 0$, which is expressed as $\{ h \in \reals^n | \|h\|_2^2 = r^2\}$.
\end{assumption}

This is a strong assumption, but at the end of this subsection we will give a lower and upper bound of $\loss$ for any possible $\partial S$ based on the results under this assumption. Since $\partial V(S) = \{ h \in \reals^n | \|h\|_2^2 = r^2\} = \partial S$ for any orthogonal $V$, this assumption gives us a nice property: the choice of $V$ doesn't affect $\Delta_1 g_e$ and $\sigma_w^2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Based on the above assumption, we can safely consider the optimal design of $V$ that minimizes $\loss$ when $\Sigma$ and $\sigma_w^2$ are given, which leads to the following proposition.

\begin{prop}[Optimal rotation matrix $V$ that minimizes $\loss$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_V}
Suppose the eigen decomposition of the Gram matrix $P^\top P$ is expressed as $P^\top P Q = Q \Lambda$, where $\Lambda = \text{diag}(\lambda_1, \cdots, \lambda_n)\in \reals^{n\times n}$ is a diagonal matrix whose diagonal elements are eigen values with $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$, and $Q \in \reals^{n \times n}$ is an orthogonal matrix whose columns are corresponding normalized eigen vectors. Then when $\Sigma$ and $\sigma_w^2$ are given, $\loss$ is minimized for $V = Q$, any $Z \geq n$ and any orthogonal $U$. And the corresponding $\loss$ can be expressed as
\begin{align}
\loss = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2}. \label{eq:loss_Sigma}
\end{align}
\end{prop}
 
In the above proposition, we see choosing a $Z > n$ brings no additional benefit, so for simplicity we only consider $Z = n$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

We notice that, after the first two sub-transforms $\Sigma$ and $V^\top$, the boundary $\partial S = \{ h \in \reals^n | \|h\|_2^2 = r^2\}$ becomes $\partial \Sigma V^\top (S) =  \{ v \in \reals^n | \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$, which is a hyperellipsoid. We therefore have the following proposition that gives the optimal $U$ which minimizes $\Delta_1 g_e$. 

\begin{prop}[Optimal rotation matrix $U$ that minimizes $\Delta_1 g_e$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_U}
For given $\Sigma$, $U = I$ minimizes $\Delta_1 g_e$, and the corresponding minimum value is
\begin{align}
\Delta_1 g_e = 2r \sqrt{\sum_{i=1}^n \sigma_i^2}.
\end{align}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next we need to consider how to design the scaling matrix $\Sigma$, or equivalently the values of $\sigma_1^2, \cdots, \sigma_n^2$, to minimize Eq.\ref{eq:loss_Sigma}, which is the only remaining piece. Clearly, for any given $\sigma_1^2, \cdots, \sigma_n^2$ if we increase them proportionally, $\sigma_w^2$ also need to be increased proportionally to preserve the same $\epsilon$-LDP. So without loss of generality, we impose an additional constraint $\sum_{i=1}^n \sigma_i^2 = M$, where $M$ is a positive constant. And the following proposition gives the optimal choice of $\Sigma$ that minimizes $\loss$ and preserve $\epsilon$-LDP with Laplace mechanism.

\begin{prop}[Optimal scaling matrix $\Sigma$ that minimizes $\loss$ and preserve $\epsilon$-LDP with Laplace mechanism under Assumption \ref{assumption:boundary_h}]\label{prop: opt_sigma}
The optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $\epsilon$-LDP with Laplace mechanism under constraint $\sum_{i=1}^n \sigma_i^2 = M$ is given by
\begin{align}
\sigma_i^2 = 
\begin{dcases*}
M \cdot (\frac{\sqrt{\lambda_i}}{\sum_{i=1}^{n'} \sqrt{\lambda_i}}(1+n'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2}), & $\forall i \in \{1, 2, \cdots, n'\}$\\
0, & $\forall i \in \{n'+1, n'+2, \cdots, n\}$
\end{dcases*} \label{eq:opt_sigma_laplace}
\end{align}
where $n' \leq n$ is the largest integer such that:
\begin{align}
\frac{\sqrt{\lambda_{n'}}}{\sum_{i=1}^{n'} \sqrt{\lambda_i}}(1+n'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2} > 0, \label{eq:opt_T_laplace}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{8r^2/\epsilon^2}{1 + n'\cdot8r^2/\epsilon^2} (\sum_{i=1}^{n'}  \sqrt{\lambda_i})^2 + \sum_{i=n'+1}^n \lambda_i. \label{eq:loss_laplace}
\end{align}
\end{prop}

For our task-aware approach, Proposition \ref{prop:opt_decoder}-\ref{prop: opt_sigma} complete the optimal encoder and decoder design that preserves $\epsilon$-LDP with Laplace mechanism, under Assumption \ref{assumption:boundary_h}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{figures_latex/fig_theory.tex}

We now compare the performance of our task-aware approach and the benchmark approach when $L = I$ and Assumption \ref{assumption:boundary_h} holds. In this case, for the benchmark approach, according to Eq. \ref{eq:loss_benchmark}, we have
\begin{align} 
\loss = \frac{\sigma_w^2}{1 + \sigma_w^2} \cdot \tr(P^\top P) = \frac{n \cdot 8r^2/\epsilon^2}{1 + n \cdot8r^2/\epsilon^2} \sum_{i=1}^n \lambda_i. \label{eq:loss_laplace}
\end{align}
We consider three different settings which have $n=4$ and $\lambda_1 = 4$ in common. And in setting 1, 2 and 3 we let $\lambda_2 = \lambda_3 = \lambda_4$ be 0, 1, 2 respectively. The corresponding result is shown in Fig. \ref{fig:theory}. Our observation is, in setting 1 the improvement of our task-aware approach is larger than the other two settings in general, because $\lambda_{2:4} = 0$ implies that $x_{2:4}$ are purely redundant. In setting 2 and 3, our task-aware approach can still outperform the benchmark approach by a small margin. We can expect higher gain than setting 1 when we have larger $n$ and zero $\lambda_{2:n}$'s, and the gain will be zero if all the $\lambda_i$'s are equal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Transition to general boundary $\partial S$.} Based on the results under Assumption \ref{assumption:boundary_h}, we can give a lower and upper bound of $\loss^*$ for general $\partial S$, which is not necessarily a centered hypersphere.

\begin{thm}[Lower and upper bound of $\loss^*$ for general boundary $\partial S$ when $\epsilon$-LDP is preserved with Laplace mechanism]\label{thm:opt_loss_bound}
Suppose $\partial S \subset \{ h \in \reals^n: r_\text{min}^2 \leq \|h\|_2^2 \leq r_\text{max}^2\}$. Then when $\epsilon$-LDP is preserved with Laplace mechanism, the optimal $\loss^*$ is bounded by:
\begin{align}
\loss(r_\text{min}; \lambda_{1:n}, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_{1:n}, \epsilon)
% \loss(r_\text{min}; \lambda_1, \cdots, \lambda_n, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_1, \cdots, \lambda_n, \epsilon)
\end{align}
where $\loss(r; \lambda_{1:n}, \epsilon)$ is the value of $\loss$ determined by Eq.\ref{eq:opt_T_laplace} and \ref{eq:loss_laplace} for given radius $r$, eigen values $\lambda_{1:n}$ and privacy budget $\epsilon$.
\end{thm}

Therefore, to perserve $\epsilon$-LDP with Laplace mechanism, our task-aware solution for general $\partial S$ is: 1) First, find the smallest $r_\text{max}$ and the largest $r_\text{min}$ that bound $\partial S$; 2) Then assume $\partial S$ is $\{ h \in \reals^n | \|h\|_2^2 = r_\text{max}^2\}$, and choose the encoder $E$ and decoder $D$ based on Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma}. We don't use the corresponding $\sigma_w^2$ however, because it may guarantee a higher LDP than needed. 3) Next, compute $\sigma_w^2$ for real $\partial S$ under decoder $D$ and privacy budget $\epsilon$. 

The associated loss for the task-aware approach is at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon)$. Though in general not optimal, it differs from $\loss^*$ by at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon) - \loss(r_\text{min}; \lambda_{1:n}, \epsilon)$. The difference is small when $\partial S$ is "nearly" a hypersphere, i.e., $r_\text{max} - r_\text{min} \approx 0$. (Remember we also have $\mu_h = \bm{0}$ and $\Sigma_{hh} = I$. Even though it may not provide any guarantees on $r_\text{max} - r_\text{min}$, for $h$ associated with real datasets we don't expect $r_\text{max} - r_\text{min}$ to be large, either.)

\subsection{General Settings} \label{subsec:general_settings}

For more complex scenarios, it is challenging to give an analytical solution to the task-aware privacy preservation problem, especially when the encoder function $g_e$, decoder function $g_d$ and task function $f$ correspond to deep neural networks (DNNs). Thus, we present a heuristic learning algorithm.

\paragraph{Task-aware.} Algorithm \ref{alg:ldp_codesign} is our proposed task-aware algorithm in the general settings. First, the privacy budget $\epsilon$ and the latent dimension $Z$ is required for the algorithm. In general, $Z$ should be large so that it is not the bottleneck (in other words, we won't find a better solution by choosing a larger $Z$). $Z = n$ is usually enough. Next, the algorithm adopts an alternating iteration approach, where in each epoch, we first update parameters $\theta_e$, $\theta_d$ by their corresponding negative gradients in line 3, and then recompute $\Delta_1 g_e$ and re-sample $w$ from $\text{Lap}^Z(0, \frac{\Delta_1 g_e}{\epsilon})$in line 4. Note that, in terms of encoder parameter $\theta_e$, instead of considering the gradient of $\loss$, we add an $\ell_2$ regularization term $\eta \|\theta_e\|^2$ where $\eta$ is a positive constant. Therefore, we update $\theta_e$ with the negative gradient $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$. Without regularization, the $\|\theta_e\|^2$ will grow to infinity since we can always achieve a smaller $\loss$ by increasing the scale of $\phi$ proportionally. But it is not a direction we are looking for, since $\sigma_w^2$ will also increase proportionally to guarantee $\epsilon$-LDP.  

\paragraph{Benchmark.} The algorithm used for the benchmark approach only differs from Algorithm \ref{alg:ldp_codesign} in line 3. Since $g_e$ is fixed to an identity function, we only need to update $\theta_d$ with $- \nabla_{\theta_d} \loss$ by one or multiple steps in line 3. In line 4, though $\Delta_1 g_e$ remains unchanged, we still re-sample $w$ to avoid overfitting. 

\begin{algorithm}[tb]
   \caption{Task-aware Algorithm for $\epsilon$-LDP Preservation in General Settings}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \Require Privacy budget $\epsilon$, and $Z$
        \State Initialize encoder/decoder parameters $\theta_e, \theta_d$ and noise vector $w$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
             \State Recompute $\Delta_1 g_e$, and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$
        \EndFor
        \State Return $\theta_e, \theta_d$ and $\Delta_1 g_e$
    \end{algorithmic}
\end{algorithm}



==> sections/jiangnan/intro.tex <==
In recent years, there has been a tremendous growth in the volume of available data for machine learning (ML) tasks, leading to increasing emphasis on protecting user privacy. Differential privacy (DP) \cite{dwork2006calibrating,dwork2014algorithmic} is a state-of-the-art technique for data privacy, and its local variant -- local differential privacy (LDP) \cite{kasiviswanathan2011can} provides stronger privacy guarantees for individual users without dependence on any trusted third party. In practice, LDP has been successfully deployed in commericial products of companies including Google \cite{erlingsson2014rappor}, Apple \cite{apple2021dp}, and Microsoft \cite{ding2017collecting} for some basic frequency or histogram estimation tasks where raw user data is restricted to an $n$-bit discrete variable.  

It is natural to envision that, in the future, LDP will be adopted in more complex scenarios \cite{hassan2019differential,dankar2013practicing,zhao2014achieving,cortes2016differential}, e.g., health care, power grids, Internet of things (IoT), etc., where richer user data attributes are available and more sophisticated tasks are considered. For such cases, a task-agnostic LDP preservation approach may not be ideal, since it simply perturbs all the data attributes by adding noise with a scale depending on the given privacy budget, regardless of what ultimate task the anonymized data will be used for. And, in general, to provide the same LDP guarantee, the scale of the noise has to be increased when more data attributes are present, even though some of them may be redundant or minimally relevant to the ultimate task. As a consequence, one often adds excessive noise that severely degrades an ultimate task's performance or will require an excessive amount of data samples to achieve the same task performance. 
%The problem can become very severe for high dimensional data. 
%As a consequence, more data samples are required to achieve the same task performance.

In this paper, we focus on how to improve the performance for an ML task based on multi-dimensional user data while still preserving a given level of user privacy. We take a \textit{task-aware} LDP preservation approach. The key technical insight is that the task performance can be potentially improved by exposing and perturbing only a salient (i.e. task-relevant) latent representation of user data.
Crucially, user privacy is guaranteed under the same privacy budget, according to the post-processing immunity of DP \cite{dwork2014algorithmic} (i.e., one cannot make the output of a privacy algorithm less differentially private without additional knowledge). For example, when the raw user data consists of a non-trivial number of attributes that are less or not relevant to the task, a salient task-aware LDP preservation approach only exposes high-valued data attributes that are essential to improving task performance, in which case only a smaller noise is needed to guarantee the same level of privacy (see Section \ref{sec:motivation} for a concrete example). Even for high-valued data attributes, we can adjust the signal-to-noise ratio in a task-driven manner based on their importance. And when different data attributes are dependent on each other, task-agnostic LDP preservation is even more promising in that we can consider the utilities of the underlying orthogonal bases through principal component analysis (PCA) \cite{dunteman1989principal}, instead of the raw data attributes.

\phead{Contributions.} In light of prior work, our contributions are three-fold. First, we propose a task-aware privacy preservation problem based on an encoder-decoder framework, which aims at minimizing the overall task loss under a given LDP budget $\epsilon$ (Section \ref{sec:problem_formulation}). Second, in terms of task-aware privacy preservation, we give an analytical near-optimal solution for a linear setting and MSE task loss, and provide a heuristic learning algorithm for more general settings (Section \ref{sec:analysis}). Third, we validate the effectiveness of our task-aware approach through three real-world experiments, which show our task-aware approach outperforms the benchmark approach on overall task loss under various LDP budgets by as much as $62.5\%$ (Section \ref{sec:evaluation}). All the proofs are given in the Appendix. 

\phead{Related Work.} 
1) \underline{Utility maximization in DP/LDP}. Most theoretical DP/LDP research either provides a utility upper bound for a given privacy budget under some weak assumptions \cite{alvim2011differential,duchi2013local,makhdoumi2013privacy,hardt2010geometry,wang2019subsampled}, or design optimal privacy preservation mechanisms in some specific use cases \cite{mcsherry2007mechanism,wasserman2010statistical,friedman2010data,xiao2010differential,kairouz2014extremal,geng2015optimal,liu2016dependence,yiwen2018utility}. To the best of our knowledge, with respect to \textit{multi-dimensional user data}, \cite{murakami2019utility} and \cite{wang2019collecting} are the only two similar works to ours.
% old 
\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be \SC{privacy-sensitive}, and hence the utility improvement is mainly achieved by providing privacy guarantees \SC{for only a subset of attributes}. 
\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally \SC{improves} utility. 
The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
% old 
%\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be sensitive, and hence the utility improvement is mainly achieved by providing different privacy guarantees. 
%\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally leads to a better utility. 
%The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
2) \underline{End-to-end (E2E) learning}. There has been a wide variety of works training a cascade of complex deep neural networks (DNNs) through E2E learning, where a task-specific output is directly predicted from the raw inputs \cite{muller2006off,wang2012end,donti2017task,zhou2018voxelnet,amos2018differentiable}. Our work also follows such a practice, but introduces an LDP guarantee while improving the task performance.
3) \underline{DP/LDP in deep learning}. The popularity of deep learning also draws great attention to DP or LDP preservation therein \cite{song2013stochastic,shokri2015privacy,abadi2016deep,phan2016differential,papernot2016semi,mcmahan2018general,arachchige2019local,bu2020deep}. Our work is fundamentally different. Instead of preserving LDP \textit{during the learning process}, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with privacy preservation during the \textit{offline} training process, which requires some ground truth user data (\SC{e.g., from a small group of consenting volunteers)}. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.
 
% A few points to consider:

% 1. End-to-end model learning \cite{donti2017task}

% 2. LDP is widely used for preserving the privacy of individual users. Most of today's LDP preservations are task-agnostic, which perturbs the raw user data by adding noises with a scale depending on the given privacy budget, regardless for what task the user data is going to be used. Some existing researches, such as \cite{murakami2019utility,yiwen2018utility}, focus on developing a utility-maximized LDP framework. However, their major assumption is some users or some fields of the user data may have low or no privacy requirement, so the utility improvement is mainly achieved by providing different privacy guarantees.

% 3. In this paper, we focus on improving the task performance by choosing a salient latent representation of user data. Our key technical insight is, under a given privacy budget, when the raw user data consists of a non-trivial number of fields that are less or not relevant to the task, a task-agnostic LDP preservation approach has to adopt a large noise to mask a user's identity. Therefore, a salient task-aware LDP preservation approach should only expose high-valued data fields that are essential to improving the task performance, in which case only a smaller noise is needed to \textit{guarantee the same level of privacy}. For multi-dimensional \textit{continuous} data, task-agnostic LDP preservation is even more promising in that we can choose a low-dimensional representation consists of the high-valued principal components of raw user data, and adjust the signal-to-noise ratio saliently based on their importance.

% 4*. A natural concern of our proposed task-aware approach is whether the privacy of user is truly preserved, since we only preserve the privacy by adding noise to a salient representation, which is usually low-dimensional. We would like to point out that, the perturbed representation is computed solely at the user's end, and is the only information acquired by the downstream system. And differential privacy is immune to post processing \cite{dwork2014algorithmic}, i.e., without additional knowledge, one cannot make the output of a privacy algorithm less differentially private. So LDP is indeed preserved at the downstream side. 

% 5. Some existing researches focus on preserve LDP in deep learning. However, our paper is fundamentally different. Instead of preserving LDP \textit{during the learning process}, which is not our concern, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with the privacy preservation during the \textit{offline} training process, which requires some ground truth user data. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.

% 6. Contributions:
% 1) Propose a task-aware privacy preservation problem based on encoder-decoder framework, which aims at minimize the overall task loss under a given LDP budget $\epsilon$;
% 2) Develop a co-design approach that gives solutions to the privacy preservation problem. An analytical near-optimal solution is given under linear model and MSE task loss, and for more general settings a heuristic learning algorithm is provided;
% 3) Demonstrate the effectiveness of our co-design approach through evaluation with three experiments, which show our co-design approach outperforms the benchmark approach on overall task loss under various LDP budgets, and the improvement can be as high as $39.6\%$.  


==> sections/jiangnan/problem_formulation.tex <==
\input{figures_latex/fig_architecture.tex}

We now introduce the task-aware privacy preservation problem. Let $y = f(x) \in \reals^m$ denote the task output associated with each ground truth data sample $x$, where $f$ represents the task function. To guarantee $\epsilon$-LDP for each data sample $x$, its true value should never be exposed to the task function. Instead, an estimate of $x$, denoted by $\hat{x}$, is used as the input to the task function with the corresponding task output $\hat{y} = f(\hat{x})$. The objective is to minimize the overall task loss $\loss = \E_{x \sim \dist_x}[l(\hat{y}, y)]$ due to the difference between $\hat{x}$ and $x$, where $\dist_x$ is the distribution of $x$, and $l$ is a task loss function that captures the discrepancy between task output $\hat{y}$ and $y$. Common examples of this function include the $\ell_2$ loss and cross-entropy loss.

More concretely, $x$ is first mapped to a latent representation $\phi \in \reals^Z$ through an encoder function $\phi = g_e(x; \theta_e)$, where $\theta_e$ is the encoder parameter. $\phi$ is then perturbed  by a Laplace noise vector $w \in \reals^Z$. That is, $g_e$ is treated as the sensitive function $g$ in Eq.\ref{eq:lap}. Next, $\hat{x}$ is reconstructed from $\phi + w$ using a decoder function $\hat{x} = g_d(\phi+w; \theta_d)$ where $\theta_d$ is the decoder parameter. The overall diagram is shown in Fig \ref{fig:architecture}.

The optimal task-aware $\hat{x}$ minimizes $\loss$ while preserving $\epsilon$-LDP. In other words, the task-aware privacy preservation problem aims to co-design encoder and decoder, i.e., find proper values for $Z$, $\theta_e$ and $\theta_d$, such that $\loss$ is minimized and $\epsilon$-LDP is preserved. Formally, we have
\begin{align}
\min_{Z, \theta_e, \theta_d} \quad & \loss = \E_{x \sim \dist_x}[l(\hat{y}, y)],\\
\text{s.t.} \quad & y = f(x), \\
& \hat{y} = f(g_d(g_e(x; \theta_e)+w; \theta_d)),\\
& w \sim \text{Lap}^Z(0, \frac{\Delta_1 g_e}{\epsilon}).
\end{align}


\paragraph{Benchmark:} 
\begin{itemize}
\item The difficulty of co-design mainly comes from the discrepancy of the measurement of overall task loss $\loss$, which depends on $\dist_x$ and captures the \textit{average} performance, and the mechanism of preserving LDP, which depends on $X$ and focuses only on the \textit{worst-case} privacy guarantee.

\item a natural benchmark approach, which preserves $\epsilon$-LDP by adding noise directly to the  normalized $x$\footnote{We may either normalize each dimension independently when $x$ is a multi-variate random variable, or normalize all the dimensions jointly when $x$ is a uni-variate time-series.}. Here for convenience, we assume $x$ is already normalized, so we always have $Z = n$ and $g_e(x) = x$. The benchmark approach only needs to determine the optimal decoder parameter $\theta_d$. Note that even though $g_e$ is an identity function, the corresponding optimal $g_d$ is usually not an identity function, which can be seen in an example in Section \ref{subsec:linear_model}.
\end{itemize}


==> sections/neurips_old/analysis.tex <==
In this section, we solve the task-aware privacy preservation problem. Assuming a linear model and mean-squared error (MSE) task loss, we are able to find near-optimal analytical results, which shed clear insight on how to co-design an encoder and decoder. We then move to general settings and present a heuristic learning algorithm which demonstrates strong empirical performance. 

\subsection{Linear Model with MSE Task Loss} \label{subsec:linear_model}

In this subsection, we consider a linear model with MSE task loss. More specifically, encoder function $g_e$, decoder function $g_d$, and task function $f$ are assumed to be linear functions in their corresponding inputs, and the loss function is $l = \|(\hat{y} - y)\|^2_2$. The task function $f$ can then be expressed as $f(x) = K x$, where $K \in \reals^{m \times n}$ is the task matrix. 
% \cite{?}.

\phead{Practicality of the setting.} Linear transformation is a common encoding and decoding approach for many dimensionality-reduction techniques, such as PCA. And $\ell_2$ task loss is widely used in many application scenarios. 
% I do not fully follow the following example - Kevin
For example, given $N$ samples of $x$, suppose we want to estimate the mean value of these samples in a few directions, given by task matrix $K$. Then the sum of the variance of these estimations by using $\hat{x}$ instead of $x$ will be 
\JC
{
$\frac{1}{N}\E_{x,w}[\|K(\hat{x} - x)\|^2_2]$, so $\loss = \E_{x,w}[\|K(\hat{x} - x)\|^2_2] = \E_{x,w}[\|(\hat{y} - y)\|^2_2]$ is a natural objective function.
}

\phead{Contents.} We first summarize key results. For our task-aware approach, the optimal decoder is first determined in Proposition \ref{prop:opt_decoder}, and then the optimal encoder and the corresponding optimal loss is formulated in Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma} under Assumption \ref{assumption:boundary_h}. We then relax Assumption \ref{assumption:boundary_h} and provide lower and upper bounds for the optimal loss in Theorem \ref{thm:opt_loss_bound} and an approximate solution. For \JC{the task-agnostic and privacy-agnostic approach, the corresponding optimal losses are determined in Corollary \ref{cor:opt_loss_task_agnostic} and \ref{cor:opt_loss_privacy_agnostic}, respectively.} All proofs are in the Appendix (supplement).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phead{Detailed analysis.} We start our analysis with a few definitions. First, without loss of generality, we assume the covariance matrix of $x-\mu_x$, i.e., $\E[(x-\mu_x)(x-\mu_x)^\top]$, is positive definite, where $\mu_x \in \reals^n$ is the mean vector of $x$. This assumption guarantees $x$ cannot be linear transformed to a low-dimensional representation without losing information. 

We then factorize $\E[(x-\mu_x)(x-\mu_x)^\top]$ into $L L^\top$ through Cholesky decomposition, where $L \in \reals^{n \times n}$ is a lower triangular matrix with positive diagonal entries. For analytical convenience, we let $h = L^{-1}(x-\mu_x)$, which can be viewed as another representation of $x$, with mean $\mu_h = \bm{0}$ and covariance matrix $\Sigma_{hh} = I$. Let $\dist_h$ denote the distribution of $h$, and $H = \{L^{-1}(x-\mu_x) | x \in X\}$ denote the compact set that contains all the possible values of $h \sim \dist_h$. Since $K (\hat{x} - x) = P (\hat{h} - h)$, where $P = K L$, working with data representation $h$ with task matrix $P$ is equivalent to using $x$ and $K$. Considering zero-centered $h$ instead of original $x$ saves us from considering the constant terms in the linear encoder and decoder functions.

Let $E \in \reals^{Z \times n}$ and $D \in \reals^{n \times Z}$  denote the encoder and decoder matrix associated with $h$, i.e., $\phi = E h$ and $\hat{h} = D(E h+w)$. Without loss of generality, we let $Z \geq n$ and allow some rows of $E$ to be zero. Equivalently, based on the relationship between $x$ and $h$, we have $\phi = E L^{-1} (x-\mu_x)$ and $\hat{x}-\mu_x = L D(E L^{-1}(x-\mu_x)+w)$. We denote the covariance matrix of $w$ by $\Sigma_{ww}$, and it can be expressed as $\Sigma_{ww} = \sigma_w^2 I$, where $\sigma_w^2$ is the variance of the noise added to each dimension of $\phi$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first determine the optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$, which is given by the following proposition.

\begin{prop}[Optimal decoder $D$ that minimizes $\loss$]\label{prop:opt_decoder}
An optimal decoder $D$ that minimizes $\loss$ for a given encoder $E$ and $\sigma_w^2$ can be expressed as $D = E^\top (E E^\top + \sigma_w^2 I)^{-1}$, and corresponding $\loss$ is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  E^\top (EE^\top + \sigma_w^2 I)^{-1} E), \label{eq:loss_E}
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. 
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One can obtain the resultant optimal $\loss$ for the task-agnostic approach by letting $E = L$ and using Eq.\ref{eq:loss_E} as stated in Proposition \ref{prop:opt_decoder}. It is worth noting that the associated decoder $D = L^\top (L L^\top + \sigma_w^2 I)^{-1}$ is not an identity matrix in general. 

\begin{cor}[Optimal $\loss$ for the task-agnostic approach that preserves $\epsilon$-LDP]\label{cor:opt_loss_task_agnostic}
For the task-agnostic approach, the optimal $\loss$ that preserves $\epsilon$-LDP is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  L^\top (LL^\top + \sigma_w^2 I)^{-1} L), \label{eq:loss_task_agnostic}
\end{align}
where $\sigma_w^2 = 2 (\Delta_1 g_e)^2 / \epsilon^2$ with $g_e(x) = x$. 
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The next main step is to find an encoder $E$ that minimizes Eq.\ref{eq:loss_E}. Since $\Delta_1 g_e = \max_{v, v' \in E(H)} \|v - v'\|_1$, where $E(H) = \{Eh | h \in H\}$ is the image of $H$ under linear transformation $E$, the design of encoder $E$ will affect $\Delta_1 g_e$ and therefore $\sigma_w^2$, and for different $H$'s the effect of $E$ is also different in general. So we need to carefully consider the relationship between $E$ and $H$. 

When computing $\Delta_1 g_e$ we can actually use $H$'s convex hull $S$ instead of $H$ itself, according to the following lemma. This brings some analytical convenience in the further analysis.

\begin{lem}[Convex hull preserves $\Delta_1 g_e$]\label{lem:convex_hull}
\begin{align}
\Delta_1 g_e = \max_{v, v' \in E(S)} \|v - v'\|_1.
\end{align}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For encoder $E$, consider its singular value decomposition (SVD) instead: $U \Sigma V^\top$, where $U \in \reals^{Z \times Z}$ and $V \in \reals^{n \times n}$ are orthogonal matrices and $\Sigma \in \reals^{Z \times n}$ is a rectangular diagonal matrix. And the singular values are denoted by $\sigma_1, \cdots, \sigma_n$ with $|\sigma_1| \geq \cdots \geq |\sigma_n|$. Then designing $E$ is equivalent to designing matrix $U$, $V$ and $\Sigma$. The geometric interpretation of applying transform $E = U \Sigma V^\top$ to set $S$ consists of three sub-transforms: 1) rotate $S$ by applying rotation matrix $V^\top$; 2) scale $V^\top (S)$ by applying scaling matrix $\Sigma$; 3) rotate $\Sigma V^\top (S)$ by applying rotation matrix $U$. In general, the choice of any of $U$, $\Sigma$, and $V$ will affect $\Delta_1 g_e$ and hence $\sigma_w^2$.

Our overall strategy is to first minimize the loss $\loss$ and the sensitivity value $\Delta_1 g_e$ over $U$ and $V$. The resulting $U$ and $V$ only depend on $\Sigma$ under Assumption \ref{assumption:boundary_h} (Propositions \ref{prop:opt_V}, \ref{prop:opt_U}). We then find the optimal $\Sigma$ that minimizes the $\loss$ within a given privacy budget $\epsilon$ (Proposition \ref{prop: opt_sigma}). By the end, we relax Assumption \ref{assumption:boundary_h} to discuss the quality of our solution (Theorem \ref{thm:opt_loss_bound}) . 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We start by noting that for two points within a compact set, they must lay on the boundary to have the maximum $\ell_1$ distance. We then make the following assumption in terms of $\partial S$, which is the boundary of $S$. It decouples the relationship between the choice of $V$ and the value of $\Delta_1 g_e$.

\begin{assumption} [Boundary $\partial S$ is a centered hypersphere] \label{assumption:boundary_h}
The boundary $\partial S$ is a centered hypersphere of radius $r \geq 0$, which is expressed as $\{ h \in \reals^n | \|h\|_2^2 = r^2\}$.
\end{assumption}

This is a strong assumption, but at the end of this subsection we will give a lower and upper bound of $\loss$ for any possible $\partial S$ based on the results under this assumption. Since $\partial V(S) = \{ h \in \reals^n | \|h\|_2^2 = r^2\} = \partial S$ for any orthogonal $V$, this assumption gives us a nice property: the choice of $V$ doesn't affect $\Delta_1 g_e$ and $\sigma_w^2$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Based on the above assumption, we can safely consider the optimal design of $V$ that minimizes $\loss$ when $\Sigma$ and $\sigma_w^2$ are given, which leads to the following proposition.

\begin{prop}[Optimal rotation matrix $V$ that minimizes $\loss$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_V}
Suppose the eigen-decomposition of the Gram matrix $P^\top P$ is expressed as $P^\top P Q = Q \Lambda$, where $\Lambda = \text{diag}(\lambda_1, \cdots, \lambda_n)\in \reals^{n\times n}$ is a diagonal matrix whose diagonal elements are eigenvalues with $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$, and $Q \in \reals^{n \times n}$ is an orthogonal matrix whose columns are corresponding normalized eigenvectors. Then, when $\Sigma$ and $\sigma_w^2$ are given, $\loss$ is minimized for $V = Q$, any $Z \geq n$, and any orthogonal $U$. And the corresponding $\loss$ can be expressed as:
\begin{align}
\loss = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2}. \label{eq:loss_Sigma}
\end{align}
\end{prop}
 
It is clear that choosing a $Z > n$ brings no additional benefit. Hence we can only consider \SC{$Z = n$} for simplicity. \JC{ Besides, through similar analysis, one can obtain the resultant optimal $\loss$ for the privacy-agnostic approach, which has a pre-determined $Z \leq n$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\JC{
\begin{cor}[Optimal $\loss$ for the privacy-agnostic approach that preserves $\epsilon$-LDP]\label{cor:opt_loss_privacy_agnostic}
For the privacy-agnostic approach with a pre-determined $Z \leq n$, the optimal $\loss$ that preserves $\epsilon$-LDP is
\begin{align}
\loss = \sum_{i=1}^Z \lambda_i \frac{\sigma_w^2}{\sigma_i^2+\sigma_w^2} + \sum_{i=Z+1}^n \lambda_i. \label{eq:loss_privacy_agnostic}
\end{align}
where $\sigma_w^2 = 2 (\Delta_1 g_e)^2 / \epsilon^2$.
\end{cor}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

After the first two sub-transforms $\Sigma$ and $V^\top$, the boundary $\partial S = \{ h \in \reals^n | \|h\|_2^2 = r^2\}$ becomes $\partial \Sigma V^\top (S) =  \{ v \in \reals^n | \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$, which is a hyperellipsoid. We then have the following proposition that gives the optimal $U$ which minimizes $\Delta_1 g_e$. 

\begin{prop}[Optimal rotation matrix $U$ that minimizes $\Delta_1 g_e$ under Assumption \ref{assumption:boundary_h}] \label{prop:opt_U}
For a given $\Sigma$, $U = I$ minimizes $\Delta_1 g_e$, and the corresponding minimum value is
\begin{align}
\Delta_1 g_e = 2r \sqrt{\sum_{i=1}^n \sigma_i^2}. \label{eq:opt_g_e}
\end{align}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we need to consider how to design the scaling matrix $\Sigma$, or equivalently, the values of $\sigma_1^2, \cdots, \sigma_n^2$, to minimize Eq.\ref{eq:loss_Sigma}, which is the only remaining piece. Clearly, for any given $\sigma_1^2, \cdots, \sigma_n^2$ if we increase them proportionally, $\sigma_w^2$ also needs to be increased proportionally to preserve the same $\epsilon$-LDP. So without loss of generality, we impose an additional constraint $\sum_{i=1}^n \sigma_i^2 = M$, where $M$ is a positive constant. And the following proposition gives the optimal choice of $\Sigma$ that minimizes $\loss$ and preserves $\epsilon$-LDP with the Laplace mechanism.

\begin{prop}[Optimal scaling matrix $\Sigma$ that minimizes $\loss$ and preserves $\epsilon$-LDP with Laplace mechanism under Assumption \ref{assumption:boundary_h}]\label{prop: opt_sigma}
The optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $\epsilon$-LDP with Laplace mechanism under constraint $\sum_{i=1}^n \sigma_i^2 = M$ is given by
\begin{align}
\sigma_i^2 = 
\begin{dcases*}
M \cdot (\frac{\sqrt{\lambda_i}}{\sum_{i=1}^{Z'} \sqrt{\lambda_i}}(1+Z'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2}), & $\forall i \in \{1, 2, \cdots, Z'\}$\\
0, & $\forall i \in \{Z'+1, Z'+2, \cdots, n\}$
\end{dcases*} \label{eq:opt_sigma_laplace}
\end{align}
where $Z' \leq n$ is the largest integer such that:
\begin{align}
\frac{\sqrt{\lambda_{Z'}}}{\sum_{i=1}^{Z'} \sqrt{\lambda_i}}(1+Z'\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2} > 0, \label{eq:opt_T_laplace}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{8r^2/\epsilon^2}{1 + Z'\cdot8r^2/\epsilon^2} (\sum_{i=1}^{Z'}  \sqrt{\lambda_i})^2 + \sum_{i=Z'+1}^n \lambda_i. \label{eq:loss_laplace}
\end{align}
\end{prop}

For our task-aware approach, Proposition \ref{prop:opt_decoder}-\ref{prop: opt_sigma} complete the optimal encoder and decoder design that preserves $\epsilon$-LDP with the Laplace mechanism under Assumption \ref{assumption:boundary_h}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{figures_latex/fig_theory.tex}

We now compare the performance of our task-aware approach and the benchmark approaches when $L = I$ and Assumption \ref{assumption:boundary_h} holds. In this case, for the \JC{task-agnostic}
% benchmark
 approach, according to Eq. \ref{eq:loss_task_agnostic}, we have
\begin{align} 
\loss = \frac{\sigma_w^2}{1 + \sigma_w^2} \cdot \tr(P^\top P) = \frac{n \cdot 8r^2/\epsilon^2}{1 + n \cdot8r^2/\epsilon^2} \sum_{i=1}^n \lambda_i.
\end{align}
\JC{
For the privacy-agnostic approach, according to Eq. \ref{eq:loss_privacy_agnostic} and Eq. \ref{eq:opt_g_e}, and assuming we have equal $\sigma_i$'s and minimum $\delta_1 g_e$, we get
\begin{align}
\loss = \frac{Z \cdot 8r^2/\epsilon^2}{1 + Z \cdot 8r^2/\epsilon^2} \sum_{i=1}^{Z} \lambda_i + \sum_{i=Z+1}^n \lambda_i,
\end{align}
where the value of $Z$ is pre-determined. 
}

\phead{\SC{Validation of Task Loss from Theoretical Results (Fig. \ref{fig:theory}).}} We consider three different settings which have $n=4$ and $\lambda_1 = 4$ in common. And in setting 1, 2, and 3 we let $\lambda_2 = \lambda_3 = \lambda_4$ be 0, 1, 2 respectively. 
\JC{
For the privacy-agnostic approach, we choose $Z = 2$.
Our observations are: 1) compared to the task-agnostic approach, our task-aware approach achieves the largest improvement in setting 1, because $\lambda_{2:4} = 0$ implies that $x_{2:4}$ are purely redundant. We can even expect higher gain than setting 1 when we have larger $n$ and zero $\lambda_{2:n}$'s, and the gain will be zero if all the $\lambda_i$'s are equal. 2) the privacy-agnostic approach completely missed the information carried by $x_{3:4}$, which explains the improvement of our task-aware approach for small $r/\epsilon$ in setting 2 and 3. We can expect higher gain than setting 3 when we have larger $n$ and larger $\lambda_{2:n}$'s, and the gain will be zero if all the missed $x_i$'s correspond to zero $\lambda_i$'s and all the other $\lambda_i$'s are equal.

% , our task-aware approach 
% %The corresponding result is shown in Fig. \ref{fig:theory}. 
% Our observation is that in setting 1, the improvement of our task-aware approach is larger than the other two settings because $\lambda_{2:4} = 0$ implies that $x_{2:4}$ are purely redundant. In setting 2 and 3, our task-aware approach can still outperform the benchmark approach by a small margin. We can expect higher gain than setting 1 when we have larger $n$ and zero $\lambda_{2:n}$'s, and the gain will be zero if all the $\lambda_i$'s are equal.
} 
%\SC{Our subsequent experiments on real-world datasets illustrate significant gains.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phead{Transition to general boundary $\partial S$.} Based on the results under Assumption \ref{assumption:boundary_h}, we can give a lower and upper bound of $\loss^*$ for general $\partial S$, which is not necessarily a centered hypersphere.

\begin{thm}[Lower and upper bound of $\loss^*$ for general boundary $\partial S$ when $\epsilon$-LDP is preserved with Laplace mechanism]\label{thm:opt_loss_bound}
Suppose $\partial S \subset \{ h \in \reals^n: r_\text{min}^2 \leq \|h\|_2^2 \leq r_\text{max}^2\}$. Then when $\epsilon$-LDP is preserved with the Laplace mechanism, the optimal $\loss^*$ is bounded by:
\begin{align}
\loss(r_\text{min}; \lambda_{1:n}, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_{1:n}, \epsilon)
% \loss(r_\text{min}; \lambda_1, \cdots, \lambda_n, \epsilon) \leq \loss^* \leq \loss(r_\text{max}; \lambda_1, \cdots, \lambda_n, \epsilon)
\end{align}
where $\loss(r; \lambda_{1:n}, \epsilon)$ is the value of $\loss$ determined by Eq.\ref{eq:opt_T_laplace} and \ref{eq:loss_laplace} for given radius $r$, eigenvalues $\lambda_{1:n}$ and privacy budget $\epsilon$.
\end{thm}

Therefore, to preserve $\epsilon$-LDP with the Laplace mechanism, our task-aware solution for general $\partial S$ is: 1) First, find the smallest $r_\text{max}$ and the largest $r_\text{min}$ that bound $\partial S$; 2) Then assume $\partial S$ is $\{ h \in \reals^n | \|h\|_2^2 = r_\text{max}^2\}$, and choose the encoder $E$ and decoder $D$ based on Proposition \ref{prop:opt_V}-\ref{prop: opt_sigma}. We don't use the corresponding $\sigma_w^2$ however, because it may guarantee a higher LDP than needed. 3) Next, compute $\sigma_w^2$ for real $\partial S$ under decoder $D$ and privacy budget $\epsilon$. 

The associated loss for the task-aware approach is at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon)$. Though in general not optimal, it differs from $\loss^*$ by at most $\loss(r_\text{max}; \lambda_{1:n}, \epsilon) - \loss(r_\text{min}; \lambda_{1:n}, \epsilon)$. 
\SC{The difference is small when $\partial S$ is ``nearly'' a hypersphere, i.e., $r_\text{max} - r_\text{min} \approx 0$.} 
%(Remember we also have $\mu_h = \bm{0}$ and $\Sigma_{hh} = I$. Even though it may not provide any guarantees on $r_\text{max} - r_\text{min}$, for $h$ associated with real datasets we don't expect $r_\text{max} - r_\text{min}$ to be large, either.)}

% old
%The difference is small when $\partial S$ is ``nearly'' a hypersphere, i.e., $r_\text{max} - r_\text{min} \approx 0$. (Remember we also have $\mu_h = \bm{0}$ and $\Sigma_{hh} = I$. Even though it may not provide any guarantees on $r_\text{max} - r_\text{min}$, for $h$ associated with real datasets we don't expect $r_\text{max} - r_\text{min}$ to be large, either.)

\subsection{General Settings} \label{subsec:general_settings}

For more complex scenarios, it is challenging to give an analytical solution to the task-aware privacy preservation problem, especially when the encoder function $g_e$, decoder function $g_d$, and task function $f$ correspond to neural networks. Thus, we present a heuristic learning algorithm.

\phead{Task-aware.} Algorithm \ref{alg:ldp_codesign} is our proposed task-aware algorithm for general settings. First, the privacy budget $\epsilon$ and the latent dimension $Z$ are required inputs for the algorithm. \JC{In general, $Z$ should be proper, i.e., it is neither too small (we can find a better solution by choosing a larger $Z$) nor too big (which introduces unnecessary complexity).}
% In general, $Z$ should be large so that it is not the bottleneck. In other words, we won't find a better solution by choosing a larger $Z$. $Z = n$ usually suffices.
Next, the algorithm adopts an alternating iteration approach, where in each epoch, we first update parameters $\theta_e$, $\theta_d$ by their corresponding negative gradients in line 3, and then recompute $\Delta_1 g_e$ and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$ in line 4. Note that, in terms of encoder parameter $\theta_e$, instead of considering the gradient of $\loss$, we add an $\ell_2$ regularization term $\eta \|\theta_e\|^2$ where $\eta$ is a positive constant. Therefore, we update $\theta_e$ with the negative gradient $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$. Without regularization, the $\|\theta_e\|^2$ will grow to infinity since we can always achieve a smaller $\loss$ by increasing the scale of $\phi$ proportionally. But it is not a direction we are looking for, since $\sigma_w^2$ will also increase proportionally to guarantee $\epsilon$-LDP.  

\phead{Benchmarks.} \JC{
For the privacy-agnostic approach, we first train encoder and decoder without considering the privacy preservation part by updating $\theta_e$ and $\theta_d$ with $- \nabla_{\theta_e} \loss$ and $- \nabla_{\theta_d} \loss$, respectively. Next, we fix encoder parameters $\theta_e$ and train decoder with input $\phi + w$ (a modification of Algorithm \ref{alg:ldp_codesign} line 3-4). The task-agnostic approach trains the decoder in the same way, but fix $g_e$ to an identity mapping function.
}

% The algorithm used for the benchmark approach only differs from Algorithm \ref{alg:ldp_codesign} in line 3. Since $g_e$ is fixed to an identity mapping, we only need to update $\theta_d$ with $- \nabla_{\theta_d} \loss$ by one or multiple steps in line 3. In line 4, although $\Delta_1 g_e$ remains unchanged, we still re-sample $w$ to avoid overfitting. 

\begin{algorithm}[tb]
   \caption{Task-aware Algorithm for $\epsilon$-LDP Preservation in General Settings}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \Require Privacy budget $\epsilon$ and $Z$
        \State Initialize encoder/decoder parameters $\theta_e, \theta_d$ and noise vector $w$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
             \State Recompute $\Delta_1 g_e$, and re-sample $w$ from $\text{Lap}^Z(0, \Delta_1 g_e / \epsilon)$
        \EndFor
        \State Return $\theta_e, \theta_d$ and $\Delta_1 g_e$
    \end{algorithmic}
\end{algorithm}



==> sections/neurips_old/basics.tex <==
Local differential privacy (LDP) \cite{dwork2014algorithmic} is the state-of-the-art technique to preserve the privacy of each individual. Let $x \in \reals^n$ be an individual data sample, and $X$ be the domain of $x$, which is a compact subset of $\reals^n$. A randomized algorithm $\mathcal{M}: X \mapsto \reals^d$ is said to satisfy $\epsilon$-LDP, if 
\begin{align}
\Pr[\mathcal{M}(x) \in \mathcal{S}] \leq e^\epsilon \Pr[\mathcal{M}(x') \in  \mathcal{S}], \quad \forall x, x' \in X, \mathcal{S}  \subseteq \text{im} \mathcal{M}  
\end{align}

To release a sensitive function $g: x \rightarrow \reals^d$ under $\epsilon$-LDP, Laplace mechanism is widely used by adding Laplace noise to function $g$:
\begin{align}
\mathcal{M}_\text{Lap}(x, g, \epsilon) & = g(x) + \text{Lap}^d(\mu = 0, b = \frac{\Delta_1 g}{\epsilon}), \quad \forall \epsilon > 0 \label{eq:lap}
\end{align}
where $\text{Lap}^d(\mu, b)$ is $d$-dimensional vector whose elements are i.i.d. Laplace random variables with mean $\mu$ and scale $b$, and $\Delta_1 g = \max_{x, x' \in X} \| g(x) - g(x')\|_1$ is the sensitivity of $g$ under $\ell_1$ norm.

% \mathcal{M}_\text{Gauss}(x, f, \epsilon, \delta) & = f(x) + \mathcal{N}^d(\mu = 0, \sigma^2 = \frac{2 \log (1.25/\delta) \cdot (\Delta_2 f)^2}{\epsilon^2}), \quad \forall \epsilon, \delta \in (0, 1) \label{eq:gauss}


==> sections/neurips_old/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
      \answerYes{\textbf{Please see Section 1.}}
  \item Did you describe the limitations of your work?
      \answerYes{\textbf{Please see the end of the evaluation (Section 5).}}
  \item Did you discuss any potential negative societal impacts of your work?
      \answerNA{\textbf{The work guarantees privacy via LDP.}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
      \answerYes{\textbf{Please see Section 4 and Assumption 1.}}
    \item Did you include complete proofs of all theoretical results?
        \answerYes{\textbf{Please see the Appendix (supplementary information).}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
      \answerYes{\textbf{Please see Appendix Section A.7.}}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{\textbf{Please see the plots in Section 5.}}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerYes{\textbf{Please see Appendix Section A.7.}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
      \answerYes{\textbf{Please see the citations for all three publicly-available datasets in Section 5. We cited both the UCI Machine Learning Repository and the individual papers as requested on the repository website. }}
  \item Did you mention the license of the assets?
      \answerYes{\textbf{As stated in the Appendix, the licenses for the individual assets were not given online.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/neurips_old/conclusion.tex <==
This paper provides a principled task-aware privacy preservation method to improve the privacy-utility trade-off for ML tasks that increasingly operate on rich, multi-dimensional user data. 
% as the dimension and complexity of rich user data grows.
%In this paper, we considered a task-aware privacy preservation problem based on an encoder-decoder framework. 
We gave an analytical near-optimal solution for a general linear encoder-decoder model and MSE task loss, and developed a heuristic learning algorithm for more general nonlinear settings. Our evaluation showed that our task-aware approach outperforms the benchmark approaches on overall task loss under various LDP budgets. 
Our future work will focus on the analysis of the task-aware privacy preservation problem for approximate LDP and other LDP mechanisms as well as multi-task learning. 


==> sections/neurips_old/evaluation.tex <==
Our evaluation compares the performance of the proposed task-aware approach and the benchmark approaches. Three applications and corresponding datasets from the standard UCI Machine Learning Repository \cite{uci} are considered: mean estimation of hourly household power consumption, real estate valuation, and breast cancer detection. Configuration and training details are provided in the appendix due to space limitations.

%\subsection{Mean Estimation of Hourly Household Power Consumption}
\phead{Mean Estimation of Hourly Household Power Consumption.}
We first consider a mean estimation problem, based on  measurements of individual household electric power consumption over four years \cite{hebrail2012individual}. Each data sample $x \in \reals^{24}$ is a time-series that contains the hourly household power consumption for one single day, and our objective is to estimate the mean of the hourly household power consumption for $N$ days. As discussed in Section \ref{subsec:linear_model}, we can define the overall task loss in the following way: 
\begin{align}
\loss = \E_{x \sim \dist_x}[\|K(\hat{x} - x)\|^2_2] = \sum_{i=1}^{24} k_i^2 \E_{x \sim \dist_x}[\|\hat{x}_i - x_i\|^2_2]
\end{align}
where $K = \text{diag}(k_1, k_2, \cdots, k_{24})$ factors the importance of the mean estimation for each hour. In our experiment we set $k_i = 2$ for $i \in \{9, 10, \cdots, 20\}$ (i.e., day-time hours) and $k_i = 1$ for other $i$'s (i.e., night-time hours). And we adopt a linear encoder and decoder model. As the considered problem is based on a linear model with MSE task loss, we adopt the solutions developed in Section \ref{subsec:linear_model} for the three approaches \JC{(we choose $Z = 3$ for the privacy-agnostic approach)}.

\input{figures_latex/fig_household.tex}

Fig. \ref{fig:household} shows our experimental results. First, on the left, we compare the task loss $l(\hat{y}, y)$ for the three approaches under different LDP budgets. For each approach, the overall task loss $\loss$ decreases when a larger LDP budget $\epsilon$ is given. Besides, for a given LDP budget, our task-aware approach always outperforms the benchmark approaches on overall task loss $\loss$, 
\JC{and the maximum improvements against the task-agnostic and privacy-agnostic approach are $22.9\%$ ($\epsilon = 10$) and $11.7\%$ ($\epsilon = 5$), respectively.}
Second, on the right, we select $\epsilon = 5$ and compare the MSE of power consumption for each hour. We see that our task-aware approach achieves a lower MSE for all the day-time hours, and a similar MSE for the night-time hours. This observation can be explained by two reasons: 1) We select a higher $k_i$ for the day-time hours, so our task-aware approach gives higher priority to minimizing the loss for those dimensions in $x$; 2) Although $x$ has 24 dimensions, the variance in each dimension can be mostly explained by several common latent dimensions, so our task-aware approach still achieves a similar MSE for the night-time hours; \JC{3) Our task-aware approach is able to adopt different scales to different latent dimensions according to their task relevance while the privacy-agnostic approach cannot.} 

%\subsection{Real Estate Valuation and Breast Cancer Detection}

Next, we consider a real estate valuation problem and a breast cancer detection problem. Both the problems are not based on the linear model with MSE task loss, so we use Algorithm \ref{alg:ldp_codesign} developed in Section \ref{subsec:general_settings} to solve them \JC{(we choose $Z = 3$ for both our task-aware approach and the privacy-agnostic approach)}.

\phead{Real Estate Valuation.} For this problem, we use historical real estate valuation data collected from Taiwan \cite{yeh2018building}, which contains 400+ instances. Here, $x \in \reals^6$ contains 6 attributes that are highly related to the value of a house, including transaction date, house age, geographic coordinates, etc. And $y \in \reals$ represents the valuation of a house. We first train a one-hidden-layer feedforward neural network regression model using the ground truth $x$ and $y$, to serve as our task function $f$. Then, we aim to minimize the $\ell_2$ loss of $\hat{y}$ and $y$, based on a linear encoder and decoder model.

\phead{Breast Cancer Detection.} For this problem, we use a well-known breast cancer diagnostic dataset \cite{street1993nuclear} from Wisconsin, which contains 500+ instances. Here, $x \in \reals^{30}$ contains 30 attributes that measure 10 features of a cell nucleus. And $y$ is a binary variable that represents a diagnosis result (malignant or benign). We first train a one-hidden-layer feedforward neural network classification model using the ground truth $x$ and $y$, to serve as our task function $f$. Then we aim to minimize the cross-entropy loss of $\hat{y}$ and $y$, with encoder and decoder both being one-hidden-layer feedforward neural networks.

\input{figures_latex/fig_ml.tex}

Fig. \ref{fig:ml} shows the evaluation results. For both problems, we can see our task-aware approach nearly always outperforms the benchmark approaches on overall task loss $\loss$ under different LDP budgets, which demonstrates the effectiveness of our proposed solution. \JC{The maximum improvements against the task-agnostic and privacy-agnostic approach are $21.9\%$ ($\epsilon = 5$) and $13.5\%$ ($\epsilon = 5$) for real estate valuation, and are $73.0\%$ ($\epsilon = 20$) and $45.6\%$ ($\epsilon = 20$) for breast cancer detection.} 

% We also see the classification model used for the cancer detection problem is more vulnerable to noise, since both approaches end up with high classification loss for $\epsilon = 5$, which is a relatively large privacy budget compared to the mean estimation and real estate valuation problems.

\phead{Limitations.} Further research is required to learn anonymized representations that are useful for \textit{multiple} tasks. Moreover, our theoretical guarantees do not apply to general deep neural networks.


==> sections/neurips_old/intro.tex <==
In recent years, there has been a tremendous growth in the volume of available data for machine learning (ML) tasks, leading to increasing emphasis on protecting user privacy. Differential privacy (DP) \cite{dwork2006calibrating,dwork2014algorithmic} is a state-of-the-art technique for data privacy, and its local variant -- local differential privacy (LDP) \cite{kasiviswanathan2011can} provides stronger privacy guarantees for individual users without dependence on any trusted third party. In practice, LDP has been successfully deployed in commericial products of companies including Google \cite{erlingsson2014rappor}, Apple \cite{apple2021dp}, and Microsoft \cite{ding2017collecting} for some basic frequency or histogram estimation tasks where raw user data is restricted to an $n$-bit discrete variable.  

It is natural to envision that, in the future, LDP will be adopted in more complex scenarios \cite{hassan2019differential,dankar2013practicing,zhao2014achieving,cortes2016differential}, e.g., health care, power grids, Internet of things (IoT), etc., where richer user data attributes are available and more sophisticated tasks are considered. For such cases, a task-agnostic LDP preservation approach may not be ideal, since it simply perturbs all the data attributes by adding noise with a scale depending on the given privacy budget, regardless of what ultimate task the anonymized data will be used for. And, in general, to provide the same LDP guarantee, the scale of the noise has to be increased when more data attributes are present, even though some of them may be redundant or minimally relevant to the ultimate task. As a consequence, one often adds excessive noise that severely degrades an ultimate task's performance or will require an excessive amount of data samples to achieve the same task performance. 
%The problem can become very severe for high dimensional data. 
%As a consequence, more data samples are required to achieve the same task performance.

In this paper, we focus on how to improve the performance for an ML task based on multi-dimensional user data while still preserving a given level of user privacy. We take a \textit{task-aware} LDP preservation approach. The key technical insight is that the task performance can be potentially improved by exposing and perturbing only a salient (i.e. task-relevant) latent representation of user data.
Crucially, user privacy is guaranteed under the same privacy budget, according to the post-processing immunity of DP \cite{dwork2014algorithmic} (i.e., one cannot make the output of a privacy algorithm less differentially private without additional knowledge). For example, when the raw user data consists of a non-trivial number of attributes that are less or not relevant to the task, a salient task-aware LDP preservation approach only exposes high-valued data attributes that are essential to improving task performance, in which case only a smaller noise is needed to guarantee the same level of privacy (see Section \ref{sec:motivation} for a concrete example). Even for high-valued data attributes, we can adjust the signal-to-noise ratio in a task-driven manner based on their importance. And when different data attributes are dependent on each other, task-agnostic LDP preservation is even more promising in that we can consider the utilities of the underlying orthogonal bases through principal component analysis (PCA) \cite{dunteman1989principal}, instead of the raw data attributes.

\phead{Contributions.} In light of prior work, our contributions are three-fold. First, we propose a task-aware privacy preservation problem based on an encoder-decoder framework, which aims at minimizing the overall task loss under a given LDP budget $\epsilon$ (Section \ref{sec:problem_formulation}). Second, in terms of task-aware privacy preservation, we give an analytical near-optimal solution for a linear setting and MSE task loss, and provide a heuristic learning algorithm for more general settings (Section \ref{sec:analysis}). Third, we validate the effectiveness of our task-aware approach through three real-world experiments, which show our task-aware approach outperforms the benchmark approach on overall task loss under various LDP budgets by as much as $62.5\%$ (Section \ref{sec:evaluation}). All the proofs are given in the Appendix. 

\phead{Related Work.} 
1) \underline{Utility maximization in DP/LDP}. Most theoretical DP/LDP research either provides a utility upper bound for a given privacy budget under some weak assumptions \cite{alvim2011differential,duchi2013local,makhdoumi2013privacy,hardt2010geometry,wang2019subsampled}, or design optimal privacy preservation mechanisms in some specific use cases \cite{mcsherry2007mechanism,wasserman2010statistical,friedman2010data,xiao2010differential,kairouz2014extremal,geng2015optimal,liu2016dependence,yiwen2018utility}. To the best of our knowledge, with respect to \textit{multi-dimensional user data}, \cite{murakami2019utility} and \cite{wang2019collecting} are the only two similar works to ours.
% old 
\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be \SC{privacy-sensitive}, and hence the utility improvement is mainly achieved by providing privacy guarantees \SC{for only a subset of attributes}. 
\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally \SC{improves} utility. 
The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
% old 
%\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be sensitive, and hence the utility improvement is mainly achieved by providing different privacy guarantees. 
%\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally leads to a better utility. 
%The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
2) \underline{End-to-end (E2E) learning}. There has been a wide variety of works training a cascade of complex deep neural networks (DNNs) through E2E learning, where a task-specific output is directly predicted from the raw inputs \cite{muller2006off,wang2012end,donti2017task,zhou2018voxelnet,amos2018differentiable}. Our work also follows such a practice, but introduces an LDP guarantee while improving the task performance.
3) \underline{DP/LDP in deep learning}. The popularity of deep learning also draws great attention to DP or LDP preservation therein \cite{song2013stochastic,shokri2015privacy,abadi2016deep,phan2016differential,papernot2016semi,mcmahan2018general,arachchige2019local,bu2020deep}. Our work is fundamentally different. Instead of preserving LDP \textit{during the learning process}, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with privacy preservation during the \textit{offline} training process, which requires some ground truth user data (\SC{e.g., from a small group of consenting volunteers)}. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.
 
% A few points to consider:

% 1. End-to-end model learning \cite{donti2017task}

% 2. LDP is widely used for preserving the privacy of individual users. Most of today's LDP preservations are task-agnostic, which perturbs the raw user data by adding noises with a scale depending on the given privacy budget, regardless for what task the user data is going to be used. Some existing researches, such as \cite{murakami2019utility,yiwen2018utility}, focus on developing a utility-maximized LDP framework. However, their major assumption is some users or some fields of the user data may have low or no privacy requirement, so the utility improvement is mainly achieved by providing different privacy guarantees.

% 3. In this paper, we focus on improving the task performance by choosing a salient latent representation of user data. Our key technical insight is, under a given privacy budget, when the raw user data consists of a non-trivial number of fields that are less or not relevant to the task, a task-agnostic LDP preservation approach has to adopt a large noise to mask a user's identity. Therefore, a salient task-aware LDP preservation approach should only expose high-valued data fields that are essential to improving the task performance, in which case only a smaller noise is needed to \textit{guarantee the same level of privacy}. For multi-dimensional \textit{continuous} data, task-agnostic LDP preservation is even more promising in that we can choose a low-dimensional representation consists of the high-valued principal components of raw user data, and adjust the signal-to-noise ratio saliently based on their importance.

% 4*. A natural concern of our proposed task-aware approach is whether the privacy of user is truly preserved, since we only preserve the privacy by adding noise to a salient representation, which is usually low-dimensional. We would like to point out that, the perturbed representation is computed solely at the user's end, and is the only information acquired by the downstream system. And differential privacy is immune to post processing \cite{dwork2014algorithmic}, i.e., without additional knowledge, one cannot make the output of a privacy algorithm less differentially private. So LDP is indeed preserved at the downstream side. 

% 5. Some existing researches focus on preserve LDP in deep learning. However, our paper is fundamentally different. Instead of preserving LDP \textit{during the learning process}, which is not our concern, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with the privacy preservation during the \textit{offline} training process, which requires some ground truth user data. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.

% 6. Contributions:
% 1) Propose a task-aware privacy preservation problem based on encoder-decoder framework, which aims at minimize the overall task loss under a given LDP budget $\epsilon$;
% 2) Develop a co-design approach that gives solutions to the privacy preservation problem. An analytical near-optimal solution is given under linear model and MSE task loss, and for more general settings a heuristic learning algorithm is provided;
% 3) Demonstrate the effectiveness of our co-design approach through evaluation with three experiments, which show our co-design approach outperforms the benchmark approach on overall task loss under various LDP budgets, and the improvement can be as high as $39.6\%$.  


==> sections/neurips_old/intro_sandeep_no_figure.tex <==
In recent years, there has been a tremendous growth in the volume of available data for machine learning (ML) tasks, leading to increasing emphasis on protecting user privacy. Differential privacy (DP) \cite{dwork2006calibrating,dwork2014algorithmic} is a state-of-the-art technique for data privacy, and its local variant -- local differential privacy (LDP) \cite{kasiviswanathan2011can} -- provides stronger privacy guarantees for individual users without dependence on any trusted third party. In practice, LDP has been successfully deployed in products of companies like Google \cite{erlingsson2014rappor}, Apple \cite{apple2021dp}, and Microsoft \cite{ding2017collecting} for some basic frequency or histogram estimation tasks where raw user data is restricted to an $n$-bit discrete variable.  

In the future, LDP has the promising potential to be adopted in more complex scenarios \cite{hassan2019differential,dankar2013practicing,zhao2014achieving,cortes2016differential} (e.g., health care, power grids, Internet of Things) that feature richer user data attributes that feed into more sophisticated downstream ML tasks. In such cases, today's standard task-agnostic LDP approaches may not be ideal. For example, consider complex user data that must be anonymized before passing it into a ML task function, such as a neural network classifier for credit scores. A standard approach would be to simply perturb the data by adding artificial noise whose scale depends on the sensitivity of user data (i.e. worst-case variation among a user population) and a given privacy budget, \textit{regardless} of what ultimate task the anonymized data will be used for. However, as the dimension and variability of user data inevitably grows, today's methods would generally have to increase the scale of noise to provide the same LDP guarantee, even though many data attributes might be highly variable across a user population, but minimally \textit{relevant} for a task. As a consequence, one often adds excessive noise to all data attributes, which can severely degrade an ultimate task's performance. 
%or will require an excessive amount of data samples to achieve the same task performance. 

%\input{figures_latex/fig_architecture.tex}

To address these challenges, this paper introduces a fundamentally different \textit{task-aware} LDP approach. Our method improves the performance of ML tasks that operate on multi-dimensional user data while still guaranteeing the same levels of privacy. 
Our key technical insight is to characterize the dependence of task performance on various user data attributes, which guides how we \textit{learn} a concise, task-relevant encoding (i.e. latent representation) of user data. Then, for the same privacy budget, we can directly expose and perturb only the task-relevant encoding rather than raw user data, which often allows us to add less noise and thereby improve task accuracy (see Section 2 for a concrete example).
Crucially, user privacy is guaranteed under the same privacy budget according to the post-processing immunity of DP \cite{dwork2014algorithmic} (i.e., one cannot make the output of a privacy algorithm less differentially private without additional knowledge). As such, an adversary cannot decode the anonymized latent representation to reduce the level of privacy.
Our method allows us to learn and expose only high-valued data attributes and flexibly adjust their signal-to-noise ratio based on their importance to a task. 
Moreover, when different data attributes are inter-dependent, task-aware LDP preservation is even more promising in that we can consider the utilities of the underlying orthogonal bases through principal component analysis (PCA) \cite{dunteman1989principal}, instead of the raw data attributes.

\phead{Contributions.} In light of prior work, our contributions are three-fold. First, we propose a task-aware privacy preservation problem 
\JC{ 
in which the effect of noise perturbation to preserve LDP is effectively considered, based on an encoder-decoder framework (Section \ref{sec:problem_formulation}). 
}
% which aims at minimizing the overall task loss under a given LDP budget (Section \ref{sec:problem_formulation}).
Second, in terms of task-aware privacy preservation, we obtain an analytical near-optimal solution for a linear setting and MSE task loss, and provide a heuristic learning algorithm for more general settings (Section \ref{sec:analysis}). Third, we validate the effectiveness of our task-aware approach through three real-world experiments, which show our task-aware approach outperforms the benchmark approaches on overall task loss under various LDP budgets by as much as \JC{$73.0\%$} (Section \ref{sec:evaluation}). All the proofs are given in the Appendix (supplement). 

\phead{Related Work.} 
1) \underline{Utility maximization in DP/LDP}. Most theoretical DP/LDP research either provides a utility upper bound for a given privacy budget under some weak assumptions \cite{alvim2011differential,duchi2013local,makhdoumi2013privacy,hardt2010geometry,wang2019subsampled,acharya2020context}, or designs optimal privacy preservation mechanisms in some specific use cases \cite{mcsherry2007mechanism,wasserman2010statistical,friedman2010data,xiao2010differential,kairouz2014extremal,geng2015optimal,liu2016dependence,yiwen2018utility,gondara2020differentially}. To the best of our knowledge, with respect to \textit{multi-dimensional user data}, \JC{\cite{murakami2019utility}, \cite{wang2019collecting} and \cite{chen2021perceptual} are the only three similar works to ours.}
% old 
\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be \SC{privacy-sensitive}, and hence the utility improvement is mainly achieved by providing privacy guarantees \SC{for only a subset of attributes}. 
\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally \SC{improves} utility.
\JC{
\cite{chen2021perceptual} preserves DP for images by adding noises to a latent representation learned through backward propagation of task loss, in which the effect of noise perturbation is not considered.
}
The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data, \JC{and we effectively capture the effect of noise perturbation resulted from the privacy requirement.}
% old 
%\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be sensitive, and hence the utility improvement is mainly achieved by providing different privacy guarantees. 
%\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally leads to a better utility. 
%The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
2) \underline{End-to-end (E2E) learning}. There has been a wide variety of works training a cascade of deep neural networks (DNNs) through E2E learning, where a task-specific output is directly predicted from the raw inputs \cite{muller2006off,wang2012end,donti2017task,zhou2018voxelnet,amos2018differentiable}. Our work also follows such a practice, but introduces an LDP guarantee while improving the task performance.
3) \underline{DP in deep learning}. The popularity of deep learning also draws great attention to DP preservation therein \cite{song2013stochastic,shokri2015privacy,abadi2016deep,phan2016differential,papernot2016semi,mcmahan2018general,arachchige2019local,bu2020deep}. Our work is fundamentally different. Instead of preserving LDP \textit{during the learning process}, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with privacy preservation during the \textit{offline} training process, which requires some ground truth user data (\SC{e.g., from a small set of consenting volunteers)}. 
However, LDP of user data is guaranteed after a trained model is deployed \textit{online}.

%However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.
 
%However, as the dimension and variability of user data $x$ grows, today's methods would generally have to increase the scale of the noise $w$ to provide the same LDP guarantee, even though many data could severely degrade ultimate task performance by adding significant levels of noise $w$ to mask highly-variable, but ultimately \textit{task-irrelevant}, user data attributes. Instead, 
%For such cases, a task-agnostic LDP preservation approach may not be ideal, since it simply perturbs all the data attributes by adding noise with a scale depending on the given privacy budget, regardless of what ultimate task the anonymized data will be used for. 
%And, in general, to provide the same LDP guarantee, the scale of the noise has to be increased when more data attributes are present, even though some of them may be redundant or minimally relevant to the ultimate task. 
%As a consequence, one often adds excessive noise that severely degrades an ultimate task's performance or will require an excessive amount of data samples to achieve the same task performance. 
%%The problem can become very severe for high dimensional data. 
%As a consequence, more data samples are required to achieve the same task performance.

% A few points to consider:

% 1. End-to-end model learning \cite{donti2017task}

% 2. LDP is widely used for preserving the privacy of individual users. Most of today's LDP preservations are task-agnostic, which perturbs the raw user data by adding noises with a scale depending on the given privacy budget, regardless for what task the user data is going to be used. Some existing researches, such as \cite{murakami2019utility,yiwen2018utility}, focus on developing a utility-maximized LDP framework. However, their major assumption is some users or some fields of the user data may have low or no privacy requirement, so the utility improvement is mainly achieved by providing different privacy guarantees.

% 3. In this paper, we focus on improving the task performance by choosing a salient latent representation of user data. Our key technical insight is, under a given privacy budget, when the raw user data consists of a non-trivial number of fields that are less or not relevant to the task, a task-agnostic LDP preservation approach has to adopt a large noise to mask a user's identity. Therefore, a salient task-aware LDP preservation approach should only expose high-valued data fields that are essential to improving the task performance, in which case only a smaller noise is needed to \textit{guarantee the same level of privacy}. For multi-dimensional \textit{continuous} data, task-agnostic LDP preservation is even more promising in that we can choose a low-dimensional representation consists of the high-valued principal components of raw user data, and adjust the signal-to-noise ratio saliently based on their importance.

% 4*. A natural concern of our proposed task-aware approach is whether the privacy of user is truly preserved, since we only preserve the privacy by adding noise to a salient representation, which is usually low-dimensional. We would like to point out that, the perturbed representation is computed solely at the user's end, and is the only information acquired by the downstream system. And differential privacy is immune to post processing \cite{dwork2014algorithmic}, i.e., without additional knowledge, one cannot make the output of a privacy algorithm less differentially private. So LDP is indeed preserved at the downstream side. 

% 5. Some existing researches focus on preserve LDP in deep learning. However, our paper is fundamentally different. Instead of preserving LDP \textit{during the learning process}, which is not our concern, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with the privacy preservation during the \textit{offline} training process, which requires some ground truth user data. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.

% 6. Contributions:
% 1) Propose a task-aware privacy preservation problem based on encoder-decoder framework, which aims at minimize the overall task loss under a given LDP budget $\epsilon$;
% 2) Develop a co-design approach that gives solutions to the privacy preservation problem. An analytical near-optimal solution is given under linear model and MSE task loss, and for more general settings a heuristic learning algorithm is provided;
% 3) Demonstrate the effectiveness of our co-design approach through evaluation with three experiments, which show our co-design approach outperforms the benchmark approach on overall task loss under various LDP budgets, and the improvement can be as high as $39.6\%$.  


==> sections/neurips_old/motivation.tex <==
\subsection{Background}

\phead{$\epsilon$-LDP \cite{kasiviswanathan2011can}.} Let $x \in \reals^n$ be an individual data sample, and $X$ be the domain of $x$, which is assumed to be a compact subset of $\reals^n$. A randomized algorithm $\mathcal{M}: X \mapsto \reals^d$ is said to satisfy $\epsilon$-LDP with \SC{\textit{privacy-budget}} $\epsilon>0$, if 
\begin{align}
\Pr[\mathcal{M}(x) \in \mathcal{S}] \leq e^\epsilon \Pr[\mathcal{M}(x') \in  \mathcal{S}], \quad \forall x, x' \in X, \mathcal{S}  \subseteq \text{im} ~\mathcal{M}.  
\end{align}
Essentially, when $\epsilon$ is small, one cannot readily differentiate whether the input of $\mathcal{M}$ is an individual user $x$ or $x'$ based on $\mathcal{M}$'s outcome. 
% either rephrase or don't keep - this is is not clear
%\SC{When $\epsilon$ is small and for any two indivduals $x$ and $x'$, we have $\Pr[\mathcal{M}(x) \in \mathcal{S}] \approx e \Pr[\mathcal{M}(x') \in \mathcal{S}]$}. 
% This means that one cannot readily differentiate whether the input of $\mathcal{M}$ is $x$ or $x'$ based on its outcome. 

\phead{Laplace mechanism \cite{dwork2014algorithmic}.} To release a sensitive function $g: X \mapsto \reals^d$ under $\epsilon$-LDP, $\forall \epsilon > 0$, the Laplace mechanism is a widely used mechanism which adds Laplace noise to function $g$:
\begin{align}
\mathcal{M}_\text{Lap}(x, g, \epsilon) & = g(x) + \text{Lap}^d(\mu = 0, b = \frac{\Delta_1 g}{\epsilon}), \label{eq:lap}
\end{align}
where $\text{Lap}^d(\mu, b)$ is a $d$-dimensional vector whose elements are i.i.d. Laplace random variables with mean $\mu$ and scale $b$, which \SC{leads} its variance to be $2b^2$. 
%For concreteness, the analysis and evaluation of this paper focus on the Laplace mechanism although the central idea is applicable to other random privacy preservation algorithms as well.
\SC{For concreteness, the analysis and evaluation of this paper focus on the Laplace mechanism although the central idea of learning task-relevant data representations is applicable to other random privacy mechanisms as well.}
$\Delta_1 g = \max_{x, x' \in X} \| g(x) - g(x')\|_1$ measures the sensitivity of $g$ under the $\ell_1$ norm.


\subsection{Motivating Example}

\input{figures_latex/fig_motivation.tex}

% \paragraph{A Motivating example.} 

Consider an example shown in Fig. \ref{fig:motivation}. For simplicity, we only consider an example with two people, Alice and Bob, and two data attributes, age and wage. Suppose we need to preserve $\epsilon$-LDP for each person with $\epsilon = 1$ and our task is to estimate the mean wage as closely as possible. A straightforward task-agnostic approach will directly expose both the two data attributes, and add Laplace noise with scale $b = 20$ to each attribute. However, a task-aware approach will expose only the wage attribute and add Laplace noise with scale $b = 10$. Both the approaches guarantee LDP under the same budget ($\epsilon=1$), but the wage attribute given by the task-aware approach is less noisy, and we can expect that the corresponding estimated mean wage (i.e. the ultimate task objective) is close to the real value with a higher probability.
%\SC{By injecting less noise, a task-aware privacy-preservation approach can often improve a downstream task's performance, such as mean wage estimation, but with the same guaranteed LDP budget.}

In more complex scenarios, such as when each data attribute is not redundant but is valued differently in terms of the considered task or data attributes are dependent but not perfectly correlated, etc., the optimal solution will not be as straightforward as the given example and will be explored in the following sections.


==> sections/neurips_old/problem_formulation.tex <==
% for jiangnan, uncomment
% for sandeep intro, keep here
\input{figures_latex/fig_architecture.tex}

We now introduce the task-aware privacy preservation problem \SC{depicted in Fig. \ref{fig:architecture}}. Let $y = f(x) \in \reals^m$ denote the task output associated with each ground truth data sample $x$, where $f$ represents the task function. To guarantee $\epsilon$-LDP for each data sample $x$, its true value should never be exposed to the task function. Instead, an estimate of $x$, denoted by $\hat{x}$, is used as the input to the task function with the corresponding task output $\hat{y} = f(\hat{x})$. The objective is to minimize the overall task loss $\loss = \E_{x \sim \dist_x}[l(\hat{y}, y)]$ due to the difference between $\hat{x}$ and $x$, where $\dist_x$ is the distribution of $x$, and $l$ is a task loss function that captures the discrepancy between task output $\hat{y}$ and $y$, such as the common $\ell_2$ and cross-entropy loss.
%Common examples of this function include the $\ell_2$ loss and cross-entropy loss.

More concretely, $x$ is first mapped to a latent representation $\phi \in \reals^Z$ through an encoder function $\phi = g_e(x; \theta_e)$, where $\theta_e$ are \SC{a set of encoder parameters}. $\phi$ is then perturbed  by a Laplace noise vector $w \in \reals^Z$. That is, $g_e$ is treated as the sensitive function $g$ in Eq.\ref{eq:lap}. Next, $\hat{x}$ is reconstructed from $\phi + w$ using a decoder function $\hat{x} = g_d(\phi+w; \theta_d)$ where $\theta_d$ are \SC{a set of decoder parameters}. 
%The overall diagram is shown in Fig \ref{fig:architecture}.

The optimal task-aware $\hat{x}$ minimizes $\loss$ while preserving $\epsilon$-LDP. In other words, the task-aware privacy preservation problem aims to co-design encoder and decoder, i.e., find proper values for $Z$, $\theta_e$ and $\theta_d$, such that $\loss$ is minimized and $\epsilon$-LDP is preserved. Formally, we have
\begin{align}
\min_{Z, \theta_e, \theta_d} \quad & \loss = \E_{x,w} [l(\hat{y}, y)],\label{eq:ldp_problem_begin}\\
\text{s.t.} \quad & y = f(x), \\
& \hat{y} = f(g_d(g_e(x; \theta_e)+w; \theta_d)),\\
& x \sim \dist_x, w \sim \text{Lap}^Z(0, \frac{\Delta_1 g_e}{\epsilon}). \label{eq:ldp_problem_end}
\end{align}

The difficulty of our task-aware LDP problem mainly comes from the discrepancy of the measurement of overall task loss $\loss$, which depends on $\dist_x$ and captures the \textit{average} performance, and the mechanism of preserving LDP, which depends on $X$ and focuses only on the \textit{worst-case} privacy guarantee.

\phead{Benchmarks.}
\JC{
Two natural approaches to preserve $\epsilon$-LDP are: 1) \textbf{Task-agnostic approach} adds noise directly to the normalized $x$\footnote{We may either normalize each dimension independently when $x$ is a multi-variate random variable, or normalize all the dimensions jointly when $x$ is a uni-variate time-series.}. For convenience we assume $x$ is already normalized, and we have $Z = n$ and $g_e(x) = x$; 2) \textbf{Privacy-agnostic approach} adds noise to $\phi$ obtained by considering the problem defined in Eq.\ref{eq:ldp_problem_begin}-\ref{eq:ldp_problem_end} with a pre-determined $Z \leq n$ and $w$ being a zero vector instead (i.e., the privacy-preservation part is neglected when designing the encoder). Both two benchmark approaches still need to determine the optimal decoder parameters $\theta_d$ for input $\phi + w$. Note that for task-agnostic approach even though $g_e$ is an identity function, the corresponding optimal $g_d$ is usually not an identity function, as exemplified in Section \ref{subsec:linear_model}.
}

% A natural approach is to preserve $\epsilon$-LDP by adding noise directly to the normalized $x$\footnote{We may either normalize each dimension independently when $x$ is a multi-variate random variable, or normalize all the dimensions jointly when $x$ is a uni-variate time-series.}, which we refer to as the \textbf{task-agnostic} benchmark. Here, for convenience, we assume $x$ is already normalized, so we always have $Z = n$ and $g_e(x) = x$. The benchmark approach only needs to determine the optimal decoder parameters $\theta_d$. Note that even though $g_e$ is an identity function, the corresponding optimal $g_d$ is usually not an identity function, as exemplified in Section \ref{subsec:linear_model}.


==> sections/neurips_old/related_work.tex <==
\paragraph{End-to-end learning.} End-to-end model learning \cite{donti2017task}

\paragraph{DP in deep learning.} Some existing researches \cite{abadi2016deep,phan2016differential,arachchige2019local} focus on preserve DP or LDP in deep learning. However, our paper is fundamentally different. Instead of preserving LDP \textit{during the learning process}, which is not our concern, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with the privacy preservation during the \textit{offline} training process, which requires some ground truth user data. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.

\paragraph{Utility-Optimized LDP.} Some existing researches, such as \cite{murakami2019utility,yiwen2018utility}, focus on developing a utility-maximized LDP framework. However, their major assumption is some users or some fields of the user data may have low or no privacy requirement, so the utility improvement is mainly achieved by providing different privacy guarantees.

==> sections/neurips_old/sandeep_intro.tex <==
In recent years, there has been a tremendous growth in the volume of available data for machine learning (ML) tasks, leading to increasing emphasis on protecting user privacy. Differential privacy (DP) \cite{dwork2006calibrating,dwork2014algorithmic} is a state-of-the-art technique for data privacy, and its local variant -- local differential privacy (LDP) \cite{kasiviswanathan2011can} -- provides stronger privacy guarantees for individual users without dependence on any trusted third party. In practice, LDP has been successfully deployed in products of companies like Google \cite{erlingsson2014rappor}, Apple \cite{apple2021dp}, and Microsoft \cite{ding2017collecting} for some basic frequency or histogram estimation tasks where raw user data is restricted to an $n$-bit discrete variable.  

In the future, LDP can conceivably be adopted in more complex scenarios \cite{hassan2019differential,dankar2013practicing,zhao2014achieving,cortes2016differential} (e.g., health care, power grids, Internet of Things), that feature richer user data attributes that feed into more sophisticated downstream ML tasks. In such cases, today's standard task-agnostic LDP approaches may not be ideal. As depicted in Fig. \ref{fig:architecture}, consider complex user data $x$ that must be anonymized before passing it into a task function $y = f(x)$. A standard approach would be to simply transform $x$ into $\hat{x} = x + w$ by adding artificial noise $w$, whose scale depends on the sensitivity of user data (i.e. worst-case variation among a user population) and a given privacy budget, \textit{regardless} of what task $f$ the anonymized data $\hat{x}$ will be used for. However, as the dimension and variability of user data grows, today's methods would generally have to increase the scale of noise to provide the same LDP guarantee, even though many data attributes might be highly \textit{variable}, but minimally relevant for a task. As a consequence, one often adds excessive noise to all data attributes, which can severely degrade an ultimate task's performance. 
%or will require an excessive amount of data samples to achieve the same task performance. 

\input{figures_latex/fig_architecture.tex}

To address these challenges, this paper introduces a fundamentally different \textit{task-aware} LDP approach that improves the performance of ML tasks while still guaranteeing the same levels of privacy for multi-dimensional user data. 
Our key technical insight is to characterize the dependence of task performance on various user data attributes, which guides how we \textit{learn} a concise, task-relevant encoding (i.e. latent representation) $\phi$ of user data. Then, for the same privacy budget, we can directly expose and perturb only the task-relevant encoding $\phi$ rather than raw user data $x$, which often allows us to add less noise and thereby improve task accuracy (see Section 2 for a concrete example).
%For the same privacy budget, rather than directly expose and perturb raw data $x$, we can instead only expose a task-relevant encoding $\phi$, which often allows us to add less noise and thereby improve task accuracy.   
%By only exposing high-valued data attributes that are essential for a task (i.e. encoding $\phi$), we can often add less noise $w'$, thereby potentially improving task performance for the same privacy budget. 
%By only exposing a task-relevant encoding $\phi$ of user data as opposed to raw data $x$, we often need to add less noise while guaranteeing the same privacy budget, which allows us to improve task performance. 
Crucially, user privacy is guaranteed under the same privacy budget according to the post-processing immunity of DP \cite{dwork2014algorithmic} (i.e., one cannot make the output of a privacy algorithm less differentially private without additional knowledge). As such, an adversary cannot decode the anonymized latent representation $\phi$ to reduce the level of privacy.
%As we formalize in Section \ref{sec:problem_formulation}, our method allows us to learn and expose only high-valued data attributes that are essential to improving task performance, which allows us to add smaller levels of noise to guarantee the same level of privacy.
% continue here ...
Our method allows us to learn and expose only high-valued data attributes and flexibly adjust their signal-to-noise ratio based on their importance to a task. 
%that are essential to improving task performance. 
%Moreover, even for high-valued data attributes, we can adjust the signal-to-noise ratio in a task-driven manner based on their importance.
Moreover, when different data attributes are dependent on each other, task-aware LDP preservation is even more promising in that we can consider the utilities of the underlying orthogonal bases through principal component analysis (PCA) \cite{dunteman1989principal}, instead of the raw data attributes.

\phead{Contributions.} In light of prior work, our contributions are three-fold. First, we propose a task-aware privacy preservation problem based on an encoder-decoder framework, which aims at minimizing the overall task loss under a given LDP budget $\epsilon$ (Section \ref{sec:problem_formulation}). Second, in terms of task-aware privacy preservation, we give an analytical near-optimal solution for a linear setting and MSE task loss, and provide a heuristic learning algorithm for more general settings (Section \ref{sec:analysis}). Third, we validate the effectiveness of our task-aware approach through three real-world experiments, which show our task-aware approach outperforms the benchmark approach on overall task loss under various LDP budgets by as much as $62.5\%$ (Section \ref{sec:evaluation}). All the proofs are given in the Appendix. 

\phead{Related Work.} 
1) \underline{Utility maximization in DP/LDP}. Most theoretical DP/LDP research either provides a utility upper bound for a given privacy budget under some weak assumptions \cite{alvim2011differential,duchi2013local,makhdoumi2013privacy,hardt2010geometry,wang2019subsampled}, or design optimal privacy preservation mechanisms in some specific use cases \cite{mcsherry2007mechanism,wasserman2010statistical,friedman2010data,xiao2010differential,kairouz2014extremal,geng2015optimal,liu2016dependence,yiwen2018utility}. To the best of our knowledge, with respect to \textit{multi-dimensional user data}, \cite{murakami2019utility} and \cite{wang2019collecting} are the only two similar works to ours.
% old 
\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be \SC{privacy-sensitive}, and hence the utility improvement is mainly achieved by providing privacy guarantees \SC{for only a subset of attributes}. 
\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally \SC{improves} utility. 
The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
% old 
%\cite{murakami2019utility} develops a utility-maximizing LDP framework under the assumption that some data attributes may not be sensitive, and hence the utility improvement is mainly achieved by providing different privacy guarantees. 
%\cite{wang2019collecting} mainly focuses on developing novel LDP mechanisms for multi-dimensional data with an objective of minimizing the worst-case noise variance, which naturally leads to a better utility. 
%The key difference of our work is we don't make additional assumptions on the sensitivity of user data and our task-aware approach achieves a better task performance \SC{than standard LDP benchmarks} by directly studying the \textit{dependencies} between the task objective and different attributes of user data.
2) \underline{End-to-end (E2E) learning}. There has been a wide variety of works training a cascade of complex deep neural networks (DNNs) through E2E learning, where a task-specific output is directly predicted from the raw inputs \cite{muller2006off,wang2012end,donti2017task,zhou2018voxelnet,amos2018differentiable}. Our work also follows such a practice, but introduces an LDP guarantee while improving the task performance.
3) \underline{DP/LDP in deep learning}. The popularity of deep learning also draws great attention to DP or LDP preservation therein \cite{song2013stochastic,shokri2015privacy,abadi2016deep,phan2016differential,papernot2016semi,mcmahan2018general,arachchige2019local,bu2020deep}. Our work is fundamentally different. Instead of preserving LDP \textit{during the learning process}, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with privacy preservation during the \textit{offline} training process, which requires some ground truth user data (\SC{e.g., from a small group of consenting volunteers)}. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.
 
%However, as the dimension and variability of user data $x$ grows, today's methods would generally have to increase the scale of the noise $w$ to provide the same LDP guarantee, even though many data could severely degrade ultimate task performance by adding significant levels of noise $w$ to mask highly-variable, but ultimately \textit{task-irrelevant}, user data attributes. Instead, 
%For such cases, a task-agnostic LDP preservation approach may not be ideal, since it simply perturbs all the data attributes by adding noise with a scale depending on the given privacy budget, regardless of what ultimate task the anonymized data will be used for. 
%And, in general, to provide the same LDP guarantee, the scale of the noise has to be increased when more data attributes are present, even though some of them may be redundant or minimally relevant to the ultimate task. 
%As a consequence, one often adds excessive noise that severely degrades an ultimate task's performance or will require an excessive amount of data samples to achieve the same task performance. 
%%The problem can become very severe for high dimensional data. 
%As a consequence, more data samples are required to achieve the same task performance.

% A few points to consider:

% 1. End-to-end model learning \cite{donti2017task}

% 2. LDP is widely used for preserving the privacy of individual users. Most of today's LDP preservations are task-agnostic, which perturbs the raw user data by adding noises with a scale depending on the given privacy budget, regardless for what task the user data is going to be used. Some existing researches, such as \cite{murakami2019utility,yiwen2018utility}, focus on developing a utility-maximized LDP framework. However, their major assumption is some users or some fields of the user data may have low or no privacy requirement, so the utility improvement is mainly achieved by providing different privacy guarantees.

% 3. In this paper, we focus on improving the task performance by choosing a salient latent representation of user data. Our key technical insight is, under a given privacy budget, when the raw user data consists of a non-trivial number of fields that are less or not relevant to the task, a task-agnostic LDP preservation approach has to adopt a large noise to mask a user's identity. Therefore, a salient task-aware LDP preservation approach should only expose high-valued data fields that are essential to improving the task performance, in which case only a smaller noise is needed to \textit{guarantee the same level of privacy}. For multi-dimensional \textit{continuous} data, task-agnostic LDP preservation is even more promising in that we can choose a low-dimensional representation consists of the high-valued principal components of raw user data, and adjust the signal-to-noise ratio saliently based on their importance.

% 4*. A natural concern of our proposed task-aware approach is whether the privacy of user is truly preserved, since we only preserve the privacy by adding noise to a salient representation, which is usually low-dimensional. We would like to point out that, the perturbed representation is computed solely at the user's end, and is the only information acquired by the downstream system. And differential privacy is immune to post processing \cite{dwork2014algorithmic}, i.e., without additional knowledge, one cannot make the output of a privacy algorithm less differentially private. So LDP is indeed preserved at the downstream side. 

% 5. Some existing researches focus on preserve LDP in deep learning. However, our paper is fundamentally different. Instead of preserving LDP \textit{during the learning process}, which is not our concern, we use learning as a tool to find the salient representation that improves the task performance under a given privacy budget. We don't specifically deal with the privacy preservation during the \textit{offline} training process, which requires some ground truth user data. However, LDP of user data is guaranteed after the \textit{online} deployment of the trained model.

% 6. Contributions:
% 1) Propose a task-aware privacy preservation problem based on encoder-decoder framework, which aims at minimize the overall task loss under a given LDP budget $\epsilon$;
% 2) Develop a co-design approach that gives solutions to the privacy preservation problem. An analytical near-optimal solution is given under linear model and MSE task loss, and for more general settings a heuristic learning algorithm is provided;
% 3) Demonstrate the effectiveness of our co-design approach through evaluation with three experiments, which show our co-design approach outperforms the benchmark approach on overall task loss under various LDP budgets, and the improvement can be as high as $39.6\%$.  


==> sections/old/analysis.tex <==
\subsection{Linear Case}

In this subsection, we consider linear encoder and decoder framework i.e., $g_e, g_{d,\target}, g_{d, \privacy}$ are linear functions in their corresponding inputs; and quadratic loss functions, i.e., $l_k = \|K_k(\hat{x}_k - x)\|^2_2$ where $K_k \in \reals^{m_k \times n}$ is the task matrix, $\forall k \in \{\target, \privacy\}$.  

Moreover, without loss of generality, we assume $\mu_x = \bm{0}$ and $\Sigma_{xx} = I$, where $\mu_x$ and $\Sigma_{xx}$ are the mean vector and the covariance matrix of $x$, respectively (the original data samples, if not satisfy this assumption, can always be linear transformed to a representation like this, and $K_i$ can absorb the reverse linear transformation). Centering $x$ also saves us from considering the constant terms in the linear encoder and decoder functions.

Hence, for $i \in \{1, 2, \cdots, Z\}$ we can express $\phi_i$ as $b_i^\top x$, with $b_i \in \reals^n$. Without loss of generality, we assume encoder output $\phi$ doesn't contain redundant information, and $b_i$'s are $Z$ unit orthogonal vectors in $\reals^n$. For the convenience of further analysis, we extend $\{b_1, b_2, \cdots, b_Z\}$ to a unit orthogonal basis $\{b_1, b_2, \cdots, b_n\}$ of $\reals^n$ and define $\phi_i = b_i^\top x, \forall i \in \{Z+1, Z+2, \cdots, n\}$ (which are not included in $Z$-dimensional vector $\phi$, however). Therefore, we have $\E[\phi_i^2] = \E [b_i^\top x x^\top b_i] = b_i^\top b_i = 1, \forall i$ and $\E[\phi_i \phi_j] = \E [b_i^\top x x^\top b_j] = b_i^\top b_j = 0, \forall i \neq j$. And $x$ can also be expressed as $\sum_{i=1}^n \phi_i b_i$. 

We claim that, for any given $\{b_1, b_2, \cdots, b_Z\}$, when $\phi$ is available $\hat{x}_k^* = \sum_{i=1}^Z \phi_i b_i$ is one of the optimal decoding and $\loss_k^* = \sum_{i=Z+1}^n \|K_k b_i\|^2$ for task $k$, $\forall k \in \{\target, \privacy\}$. To prove this, we start from the general linear transformation $\hat{x}_k = \sum_{i=1}^n  (\sum_{j=1}^Z \gamma_{i,j} \phi_j) \cdot b_i$ where $\{\gamma_{i,j} \in \reals|\forall i, \forall j \leq Z\}$ are parameters to be determined. Then we have $\forall k \in \{\target, \privacy\}$:
\begin{align}
\loss_k 
& = \E[\|K_k \sum_{i=1}^n (\sum_{j=1}^Z \gamma_{i,j} \phi_j - \phi_i) \cdot b_i\|^2] = \E[\|\sum_{i=1}^n (\sum_{j=1}^Z \gamma_{i,j} \phi_j - \phi_i) \cdot K_k b_i\|^2]
\end{align}
is a quadratic function of $\{\gamma_{i,j} |\forall i, \forall j \leq Z\}$. The coefficient associated with $\gamma_{i,j}^2$ in $\loss_k$ is $\E[\phi^2_j] \| K_k b_i\|^2 = \| K_k b_i\|^2 \geq 0$, $\forall i, \forall j \leq Z$, meaning $\loss_k$ is convex in $\{\gamma_{i,j} |\forall i, \forall j \leq Z\}$. Moreover, we can verify that $\gamma_{i,i} = 1, \forall i \leq Z$ and $\gamma_{i,j} = 0, \forall i \neq j, j\leq Z$ satisfy:
\begin{align}
\frac{\nabla \loss_k}{\nabla \gamma_{i,j}} = 2(\gamma_{j,j}-1) b_i^\top K_k^\top K_k b_j + 2\sum_{p \neq j} \gamma_{p,j} b_i^\top K_k^\top K_k b_p = 0, \quad \forall i, \forall j\leq Z
\end{align}
where we applied $\E[\phi_i^2] = 1, \forall i$ and $\E[\phi_i \phi_j] = 0, \forall i \neq j$. This proves that $\hat{x}_k^* = \sum_{i=1}^Z \phi_i b_i$ is one of the optimal decoding, and corresponding $\loss_k^* = \E[\|\sum_{i=Z+1}^n \phi_i \cdot K_k b_i\|^2] = \sum_{i=Z+1}^n \sum_{j=Z+1}^n \E[\phi_i \phi_j] b_i^\top P_1^\top P_1 b_j= \sum_{i=Z+1}^n \|K_k b_i\|^2$.

The further analyses of LDP and task-based privacy diverge from here and we continue the analysis separately.

\subsubsection{Local Differential Privacy}

\paragraph{Separate Design.}
The encoder aims to choose the optimal $\{b_1, b_2, \cdots, b_Z\}$ that $\loss_\target = \sum_{i=Z+1}^n \|K_\target b_i\|^2$ is minimized. This is exactly a principal component analysis (PCA) problem, which tells us that if the eigen-values of the semi-positive definite matrix $K_\target^\top K_\target$ are $\mu_1, \mu_2, \cdots, \mu_n$ with $\mu_1 \geq \mu_2 \geq \cdots \geq \mu_n \geq 0$, the optimal $\{b_1, b_2, \cdots, b_Z\}$ should be the eigen-vectors corresponding to the top-$Z$ eigen-values $\{\mu_1, \mu_2, \cdots, \mu_Z\}$.

However, the decoder of task $k$, $\forall k \in \{\target, \privacy\}$, only sees noise-disturbed representation $\phi'$. We use $\sigma_w^2$ to denote the variance of each element in the noise vector $w$, which grows when we require a more conservative privacy (as we can see in Eq.\ref{eq:lap}-\ref{eq:gauss}). We claim that, when $\phi'$ is available $\hat{x}_k^* = \sum_{i=1}^Z \frac{1}{1 + \sigma_w^2} \phi'_i b_i$ is one of the optimal decoding and $\loss_k^* = \sum_{i=1}^Z \frac{\sigma_w^2}{1 + \sigma_w^2} \|K_k b_i\|^2 + \sum_{i=Z+1}^n \|K_k b_i\|^2$ for task $k$, $\forall k \in \{\target, \privacy\}$. The proof is similar to the noise-free case, and we put it in the appendix due to the limitation of space.

\paragraph{Co-Design.}

In the co-design case, since we need to consider the effect of noise vector $w$, to minimize task loss $\loss_\privacy$, the scale of each $\phi_i$ should be different in general. To be more specific, we want to assign a larger scale to $\phi_i$'s with more importance, and hence it will achieve a higher signal-to-noise ratio.

Therefore, we express $\phi_i$ as $a_i \cdot b_i^\top x$, where $b_i \in \reals^n$ is a unit vector and $a_i \in \reals$ is the scaling coefficient, $\forall i \in \{1, 2, \cdots, Z\}$. Moreover, we claim that $b_i$'s should be orthogonal for optimal encoding. This is because, suppose $b_1$ and $b_2$, then we either have: 1) $|b_1^\top b_2| = 1$, which means $b_1 = \pm b_2$ and we are wasting one dimension of $\phi$ to send redundant information; 2) $|b_1^\top b_2| \in (0, 1)$, then we can replace $a_1$ and
$b_1$ by $a_1' = \sqrt{1 - (b_1^\top b_2)^2} a_1$ and $b_1' = (b_1 - (b_1^\top b_2) \cdot b_2) / \sqrt{1 - (b_1^\top b_2)^2}$, respectively. This gives us $b_1' \bot b_2$, and reduces (or maintains) the sensitivity of function $g_e$, since for any $x_1$ and $x_2$:
\begin{align}
| a_1 b_1^\top (x_1 - x_2) | & = |(a_1' b_1' + a_1(b_1^\top b_2)\cdot b_2)^\top (x_1 - x_2) | \\
& = |a_1' b_1'^\top (x_1 - x_2) | + |a_1(b_1^\top b_2)\cdot b_2^\top (x_1 - x_2) | \geq |a_1' b_1'^\top (x_1 - x_2) |
\end{align}
which means the distance between $g_e(x_1)$ and $g_e(x_2)$ in the first dimension is reduced (or maintained). And the distances in the other dimensions remain the same, so we have $\Delta_k g_e$ is reduced (or maintained), $\forall k \in \{1, 2\}$. This further reduces (or maintains) the variance of the nosies we will add on $\phi$.

Therefore, we only consider orthogonal $b_i$'s. We claim that, when $\phi'$ is available $\hat{x}_k^* = \sum_{i=1}^Z \frac{a_i}{a_i^2 + \sigma_w^2} \phi'_i b_i$ is one of the optimal decoding and $\loss_k^* = \sum_{i=1}^Z \frac{\sigma_w^2}{a_i^2 + \sigma_w^2} \|K_k b_i\|^2 + \sum_{i=Z+1}^n \|K_k b_i\|^2$ for task $k$, $\forall k \in \{\target, \privacy\}$. The proof is similar to the case when $a_i = 1$.

Without loss of generality, we add constraint $\sum_{i=1}^Z a_i^2 = Z$, where $\sum_{i=1}^Z a_i^2$ is the $\ell_2$ norm of the vector $a = [a_1, a_2, \cdots, a_z]$. This is because, if we increase $a_1, a_2, \cdots, a_Z$ proportionally, the sensitivity of $g_e$ and further $\sigma_w$ will also increase proportionally. Note that we can also constrain the $\ell_p$ norm of $a$ for other $p$'s, but the readers will see consider $\ell_2$ norm here is more suitable for this problem.

The encoder hence needs to choose the optimal $\{a_1, a_2, \cdots, a_Z\}$ and $\{b_1, b_2, \cdots, b_Z\}$ such that $\loss_\target^*$ given above is minimized. This is a hard problem, in the sense that $\sigma_w^2$ depends jointly on our choice and the distribution of data sample $\dist$. 

We then consider a sub-problem here instead: for fixed $\sigma_w^2$, what's the optimal choice of $\{a_1, a_2, \cdots, a_Z\}$ and $\{b_1, b_2, \cdots, b_Z\}$ that minimizes $\loss_\target^*$, given $\sum_{i=1}^Z a_i^2 = Z$? We first notice that $\{b_1, b_2, \cdots, b_Z\}$ should be the eigen-vectors corresponding to the top-$Z$ eigen-values $\{\mu_1, \mu_2, \cdots, \mu_Z\}$. This gives us $\loss_\target^* = \sum_{i=1}^Z \frac{\sigma_w^2}{a_i^2 + \sigma_w^2} \mu_i + \sum_{i=Z+1}^n \mu_i$. Thus we only need to consider how to choose $\{a_1, a_2, \cdots, a_Z\}$. This can be solved by Karush–Kuhn–Tucker (KKT) approach, with the following Lagrangian function:
\begin{align}
L(a_1^2, \cdots, a_Z^2, \alpha_1, \cdots, \alpha_Z, \beta) = \loss_\target^*(a_1^2, \cdots, a_Z^2) + \sum_{i=1}^Z \alpha_i(-a_i^2) + \beta(\sum_{i=1}^Z a_i^2 - Z) 
\end{align}
where we treat $a_i^2$ instead of $a_i$ as the variable to avoid solving higher-degree equations. The solution is:
\begin{align}
a_i^2 = 
\begin{cases}
\frac{\sqrt{\mu_i}}{\sum_{i=1}^T \sqrt{\mu_i}}(Z+T\sigma_w^2) - \sigma_w^2, & \forall i \in \{1, 2, \cdots, T\}\\
0, & \forall i \in \{T+1, T+2, \cdots, Z\}
\end{cases}
\end{align}
where $T \leq Z$ is the biggest number such that:
\begin{align}
\frac{\sqrt{\mu_i}}{\sum_{i=1}^T \sqrt{\mu_i}}(Z+T\sigma_w^2) - \sigma_w^2 > 0
\end{align}
and the optimal $\loss_\target^*$ is:
\begin{align} 
\loss_\target^* = \frac{\sigma_w^2}{Z + T\sigma_w^2} (\sum_{i=1}^T  \sqrt{\mu_i})^2 + \sum_{i=T+1}^n \mu_i
\end{align}

Hence we can update the encoder parameter $\theta_e$ (which corresponds to $\{a_1, a_2, \cdots, a_Z\}$ and $\{b_1, b_2, \cdots, b_Z\}$) and the noise variance $\sigma^2$ alternatively until convergence.

\paragraph{Benchmark.} The benchmark policy adds noise directly to the original data sample vector $x$. Without loss of generality, let $\mu_x = 0$ and we consider non-trivial $\Sigma_{xx}$. Moreover, we have $\Sigma_{ww} = \sigma^2_w I$.

Since $\hat{x}_\target$ is a linear transformation of $x$, we let $\hat{x}_\target = G (x + w)$, where $G \in \reals^{n \times n}$. Then we have
\begin{align}
\loss_\target 
& = \E[\|K_\target(\hat{x}_\target - x)\|^2] 
= \E[\|K_\target((G-I)x + Gw)\|^2]\\
& = \E[\tr(K_\target(G-I)xx^\top (G-I)^\top K_\target^\top) + \tr(K_\target G ww^\top G^\top K_\target^\top)]\\
& = \tr(K_\target(G-I) \Sigma_{xx} (G-I)^\top K_\target^\top) + \tr(K_\target G \Sigma_{ww} G^\top K_\target^\top)
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. Therefore, by letting
\begin{align}
\frac{\nabla \loss_\target}{\nabla G} = K_\target^\top K_\target ((G-I) \Sigma_{xx} + G \Sigma_{ww}) = 0
\end{align}
we get $G^* = \Sigma_{xx} (\Sigma_{xx} + \Sigma_{ww})^{-1}$, and the corresponding $\loss_\target^* = \tr(K_\target^\top K_\target \Sigma_{xx} (\Sigma_{xx} + \Sigma_{ww})^{-1} \Sigma_{ww})$.

\subsubsection{Task-based Privacy}

The encoder aims to choose the optimal $\{b_1, b_2, \cdots, b_Z\}$ that $\loss_\total = \sum_{i=Z+1}^n (\|K_\target b_i\|^2 - \lambda \|K_\privacy b_i\|^2)$ is minimized. This is a contrastive PCA problem \cite{abid2017contrastive}, which tells us that if the eigen-values of the symmetric matrix $K_\target^\top K_\target - \lambda K_\privacy^\top K_\privacy$ are $\mu_1, \mu_2, \cdots, \mu_n$ with $\mu_1 \geq \mu_2 \geq \cdots \geq \mu_n$, the optimal $\{b_1, b_2, \cdots, b_Z\}$ should be the eigen-vectors corresponding to the top-$Z$ eigen-values $\{\mu_1, \mu_2, \cdots, \mu_Z\}$. And we further have $\loss_\total^* = \sum_{i=Z+1}^n \mu_i$, and $\loss_k^* = \sum_{i=Z+1}^n \|K_k b_i\|^2$ for task $k$, $\forall k \in \{\target, \privacy\}$. Note that if $\exists i \leq Z$ s.t. $\mu_i < 0$, we can exclude $\phi_i$ from the latent representation $\phi$ to get a better $\loss_\total^*$.  


\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}

\subsection{General Case}

For more complex scenarios, it is challenging to provide analytical forms of the optimal encoder and decoders. Thus, we present heuristic algorithms for LDP and task-based privacy preservation, as shown in Algorithm \ref{alg:ldp} and \ref{alg:task_based_privacy}, respectively.

\paragraph{Co-design (Sketch).} May need to penalize $\loss_\target - \eta \|\theta_e\|^2$. If we don't penalize the norm of $\theta_e$, for any given $\sigma_w^2$ there won't be a stationary $\theta_e^*$ such that $-\nabla_{\theta_e^*} \loss_\target = 0$. This is because, by increasing the scale of $g_e$'s output proportionally, we can always drive the signal-to-noise ratio to any positive small number. Hence we propose Algorithm \ref{alg:ldp_codesign}.  

\begin{algorithm}[tb]
   \caption{LDP Preservation Training (Separate Design)}
   \label{alg:ldp}
   \begin{algorithmic}[1]
        \Statex \algbackskip \textbf{Step I:} Encoder Training
        \State Initialize $\theta_e, \theta_{d,\target}$; set $\hat{x}_\target = g_{d,\target}(g_e(x; \theta_e); \theta_{d,\target})$ 
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_{d,\target}$ with $- \nabla_{\theta_e} \loss_\target$ and $- \nabla_{\theta_{d,\target}} \loss_\target$, respectively
        \EndFor
        \State $\theta_e^* = \theta_e$
        \Statex
        \Statex \algbackskip \textbf{Step II:} Decoder Training for task $k$, $\forall k \in \{\target, \privacy\}$ 

        \State Initialize $\theta_{d,k}$; generate a noise sample $w$ for each data sample $x$, and set $\hat{x}_k = g_{d,k}(g_e(x; \theta_e^*) + w; \theta_{d,k})$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_{d,k}$ with $- \nabla_{\theta_{d,k}} \loss_k$
        \EndFor
        \State $\theta_{d,k}^* = \theta_{d,k}$
        \Statex
        \State Return $\theta_e^*, \theta_{d,\target}^*, \theta_{d,\privacy}^*$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{LDP Preservation Training (Co-Design)}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \State Initialize $\theta_e, \theta_{d,\target}$; set $\hat{x}_\target = g_{d,\target}(g_e(x; \theta_e)+w; \theta_{d,\target})$ 
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_{d,\target}$ with $- \nabla_{\theta_e} \loss_\target + 2 \eta \theta_e$ and $- \nabla_{\theta_{d,\target}} \loss_\target$, respectively, by one or multiple steps
             \State Update $\sigma_w^2$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
        \EndFor
        \State Return $\theta_e, \theta_{d,\target}$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Task-based Privacy Preservation Training}
   \label{alg:task_based_privacy}
   \begin{algorithmic}[1]
        \State Initialize $\theta_e, \theta_{d,\target}, \theta_{d,\privacy}$; set $\phi = g_e(x; \theta_e)$ and $\hat{x}_k = g_{d,k}(\phi; \theta_{d,k}), \forall k \in \{ \target, \privacy\}$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
            \State Update $\theta_{d,\target}$ with $-\nabla_{\theta_{d,\target}} \loss_\target$  by one or multiple steps
            \State Update $\theta_{d,\privacy}$ with $-\nabla_{\theta_{d,\privacy}} \loss_\privacy$ by one or multiple steps
            \State Update $\theta_{e}$ with $-\nabla_{\theta_{e}} \loss_\total$ by one or multiple steps
        \EndFor
        \State Return $\theta_e, \theta_{d,1}, \theta_{d,2}$
    \end{algorithmic}
\end{algorithm}


==> sections/old/analysis_2.tex <==
\subsection{Linear Encoder and Decoder with $\ell_2$ Task Loss}

In this subsection, we consider a linear encoder and decoder framework with $\ell_2$ task loss. That is, $g_e$ and $g_d$ are linear functions in their corresponding inputs, and the loss function $l = \|K(\hat{x} - x)\|^2_2$ where $K \in \reals^{m \times n}$ is the task matrix.

\paragraph{Practicality of the setting.} Linear transformation is the most basic encoding and decoding approach for many dimensionality-reduction techniques, such as principal component analysis (PCA). And $\ell_2$ task loss is quite common in many application scenarios. For example, belows are two types of applications with $\ell_2$ task loss:
\begin{itemize}
\item \textbf{Estimate the mean.} Given $N$ samples of $x$, we want to estimate the mean of these samples in a few directions. These directions are denoted by $K' \in \reals^{m \times n}$. Then the sum of the variance of these estimations by using $\hat{x}$ instead of $x$ will be $\loss = \frac{1}{N}\E_{x \sim \dist}[\|K'(\hat{x} - x)\|^2_2] = \E_{x \sim \dist}[\|\frac{1}{\sqrt{N}} \cdot K'(\hat{x} - x)\|^2_2] $, which is a natural objective function.
\item \textbf{Linear-quadratic regulator (LQR).} In LQR problem, The control decision $u$ that minimizes the control cost is given by $u = -Kx$, where $K$ is a matrix determined by the matrices associated with the linear dynamics and the quadratic cost. $l = \|K(\hat{x} - x)\|^2_2$ captures the total mean-squared error of control when using $\hat{x}$ instead of $x$ as our current state observation.
\end{itemize}

Without loss of generality, we can also assume $\mu_x = \bm{0}$ and $\Sigma_{xx}$ is positive definite, where $\mu_x$ and $\Sigma_{xx}$ are the mean vector and the covariance matrix of $x$, respectively. Zero-centered $x$ saves us from considering the constant terms in the linear encoder and decoder functions, and positive definite $\Sigma_{xx}$ guarantees $x$ cannot be linear transformed to a low-dimensional representation without losing information.

We then factorize $\Sigma_{xx}$ into $Q \Lambda Q^\top$, where $Q$ is an orthogonal matrix composed of $\Sigma_{xx}$'s eigen vectors and $\Lambda$ is a diagonal matrix composed of $\Sigma_{xx}$'s eigen values. For the convenience of our further analysis, we let $h = \Omega^{-1}x$ where $\Omega = Q \sqrt{\Lambda}$. Here $h$ can be viewed as another representation of $x$, with covariance matrix $\Sigma_{hh} = I$. Since $K x = P h$, where $P = K \Omega$, it is equivalent to considering data representation $h$ with task matrix $P$.

We use $C \in \reals^{Z \times n}$ and $G \in \reals^{n \times Z}$ to denote the encoder and decoder matrix associated with $h$, i.e., $\phi = C h$ and $\hat{h} = G(Ch+w)$. Equivalently, based on the relationship between $x$ and $h$ we have $\phi = C \Omega^{-1} x$ and $\hat{x} = \Omega G(C\Omega^{-1}x+w)$. We also use $\Sigma_{ww}$ to denote the covariance matrix of $w$, and it can be expressed as $\Sigma_{ww} = \sigma_w^2 I$, where $\sigma_w^2$ is the variance of the noise we will add to each dimension of $\phi$.

Let's first determine the optimal decoder $G$ that minimizes $\loss$ for a given encoder $C$, which is given by the following proposition.

\begin{prop}[Optimal Decoder $G$ that Minimizes $\loss$]
An optimal decoder $G$ that minimizes $\loss$ for a given encoder $C$ can be expressed as $G = C^\top (C C^\top + \Sigma_{ww})^{-1}$, and corresponding $\loss$ is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  C^\top (CC^\top + \Sigma_{ww})^{-1} C) \label{eq:loss_C}
\end{align} 
\end{prop}
\begin{proof}
We have
\begin{align}
\loss 
& = \E[\|K(\hat{x} - x)\|^2_2] = \E[\|P(\hat{h} - h)\|^2_2] 
= \E[\|P((GC-I)h + Gw)\|^2_2]\\
& = \E[\tr(P(GC-I)hh^\top (GC-I)^\top P^\top) + \tr(P G ww^\top G^\top P^\top)]\\
& = \tr(P(GC-I) (GC-I)^\top P^\top) + \tr(P G \Sigma_{ww} G^\top P^\top) \label{eq:loss_CG}
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. And we can verify that $G = C^\top (C C^\top + \Sigma_{ww})^{-1}$ is a zero point of
\begin{align}
\frac{\nabla \loss}{\nabla G} = 2 P^\top P ((GC-I) C^\top + G \Sigma_{ww})
\end{align}
Then we plug the expression of $G$ into Eq.\ref{eq:loss_CG} and get Eq.\ref{eq:loss_C}.
\end{proof}

We can also get the resulted $\loss$ for our benchmark apporach by letting $C = \Omega$ and plug it into Eq.\ref{eq:loss_C}.
\begin{cor}[Optimal $\loss$ for the benchmark approach]
The optimal $\loss$ for the benchmark approach is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  \Omega^\top (\Omega\Omega^\top + \Sigma_{ww})^{-1} \Omega)
\end{align}
\end{cor}

Our next step is to design an encoder $C$ that minimizes Eq.\ref{eq:loss_C}. Without loss of generality, we let $Z \geq n$ and allow some columns of $C$ be zero. Suppose the singular value decomposition of $C$ is $U \Sigma V^\top$, where $U \in \reals^{Z \times Z}$ and $V \in \reals^{n \times n}$ are orthogonal matrices and $\Sigma \in \reals^{Z \times n}$ is a rectangular diagonal matrix. And the singular values are denoted by $\sigma_1, \cdots, \sigma_n$ with $|\sigma_1| \geq \cdots \geq |\sigma_n|$. Then designing $C$ is equivalent to designing matrix $U$, $V$ and $\Sigma$.

The geometric interpretation of applying transform $C = U \Sigma V^\top$ to vector $h$ contains three sub-transforms: 1) rotate $h$ by applying rotation matrix $V^\top$; 2) scale $V^\top h$ by applying scaling matrix $\Sigma$; 3) rotate $\Sigma V^\top h$ by applying rotation matrix $U$. Any arbitrary rotate transformation $R \in \reals^{n \times n}$ doesn't change the $\ell_2$ norm of any vector $v \in \reals^n$, because $\|R v\|^2_2 = \tr(v^\top R^\top R v) = \tr(v^\top v) = \|v\|^2_2$. But for $\ell_1$ norm it is usually not true. And scaling transformation doesn't maintain either $\ell_1$ or $\ell_2$ norm in general. Therefore, in general, for $\ell_1$ norm, the choice of any of $U$, $\Sigma$ and $V$ will affect $\Delta_1 g_e$ and $\sigma_w^2$; and for $\ell_2$ norm, only the choice of $\Sigma$ and $V$ will affect $\Delta_2 g_e$ and $\sigma_w^2$ (transformation $V^\top$ doesn't change $\ell_2$ norm itself, but since it specifies the directions that $\Sigma$ should be applied it will eventually affect the $\Delta_2 g_e$ and $\sigma_w^2$).

In the following analysis, we assume the boundary of the region of $h$ is a hypersphere of radius $r \geq 1$: $\{ h \in \reals^n: \|h\|_2^2 = r^2\}$. This is a non-trivial assumption, but we are essentially assuming the maximum value of $\|d^\top h\|_2^2$ in any direction $d \in \reals^n$ s.t. $\|d\|^2_2 = 1$ is proportional to the variance of $d^\top h$, which is always 1 (since we have $\Sigma_{hh} = I$ already). And from $\text{Var}(d^\top h) \leq \E[(d^\top h)^2] \leq r^2$ we get $r \geq 1$. Since the equation of a hypersphere after applying any rotate transformation remains unchanged, this assumption gives us a nice property: the choice of $V$ doesn't change the location of the boundary and hence doesn't affect $\Delta g_e$ and $\sigma_w^2$.

Based on the above assumption, we can safely consider the optimal design of $V$ that minimizes $\loss$ when $\Sigma$ and $\sigma_w^2$ are given, which leads to the following proposition.

\begin{prop}[Optimal $V$ that Minimize $\loss$]
Suppose the eigen decomposition of the Gram matrix $P^\top P$ is expressed as $P^\top P Q = Q \Lambda$, where $\Lambda = \text{diag}(\lambda_1, \cdots, \lambda_n)\in \reals^{n\times n}$ is a diagonal matrix whose diagonal elements are eigen values with $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$, and $Q \in \reals^{n \times n}$ is an orthogonal matrix whose columns are corresponding normalized eigen vectors. Then $\loss$ is minimized for $V = Q$, under given $\Sigma$ and $\sigma_w^2$. And the corresponding $\loss$ can be expressed as
\begin{align}
\loss = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2} \label{eq:loss_Sigma}
\end{align}
\end{prop}

\begin{proof}
We have $\tr(P^\top P) = \sum_{i=1}^n \lambda_i$, which is a fixed number. Therefore we focus on maximizing the second trace term in Eq.\ref{eq:loss_C}. We first notice that
\begin{align}
C\Sigma_{xx}C^\top + \Sigma_{ww} = U \Sigma \Sigma^\top  U^\top + \sigma_w^2 I = U \text{diag}(\sigma_1^2+\sigma_w^2, \cdots, \sigma_n^2 + \sigma_w^2, \underbrace{\sigma_w^2, \cdots, \sigma_w^2}_{Z-n\text{ in total}}) U^\top
\end{align}
Then we have
\begin{align}
& C^\top (CC^\top + \Sigma_{ww})^{-1} C\\ 
= & V \Sigma^\top U^\top \cdot U \text{diag}(\frac{1}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{1}{\sigma_n^2+\sigma_w^2}, \frac{1}{\sigma_w^2}, \cdots, \frac{1}{\sigma_w^2}) U^\top \cdot U \Sigma V^\top\\
= & V \Sigma^\top \text{diag}(\frac{1}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{1}{\sigma_n^2+\sigma_w^2}, \frac{1}{\sigma_w^2}, \cdots, \frac{1}{\sigma_w^2}) \Sigma V^\top\\
= & V \text{diag}(\frac{\sigma_1^2}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{\sigma_n^2}{\sigma_n^2+\sigma_w^2}) V^\top
\end{align}
so $C^\top (CC^\top + \Sigma_{ww})^{-1} C$ is a positive semi-definite matrix with eigen-values $\frac{\sigma_1^2}{\sigma_1^2+\sigma_w^2} \geq \cdots \geq \frac{\sigma_n^2}{\sigma_n^2+\sigma_w^2} \geq 0$. Then by Ruhe's trace inequality \cite{ruhe1970perturbation} (a corollary of Von Neumann’s trace inequality \cite{von1937some}), we have
\begin{align}
\tr(P^\top P  C^\top (CC^\top + \Sigma_{ww})^{-1} C) \leq \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2}
\end{align}
and when $V = Q$ the equality holds. So we have Eq.\ref{eq:loss_Sigma} for $V = Q$.
\end{proof}
 
In the above proposition, we see choosing a $Z > n$ brings no additional benefit, so for simplicity we only consider $Z = n$. 

% And when $\sigma_w^2$ is fixed, the choice of $U$ doesn't affect loss $\loss$. This is immediately true when we use $\sigma_w^2$ is based on $\Delta_2 g_e$ (as we discussed earlier). However, we still need to carefully design $U$ when $\sigma_w^2$ is based on $\Delta_1 g_e$.

We notice that, after the first two transforms $\Sigma$ and $V^\top$, the boundary $\{ h \in \reals^n: \|h\|_2^2 = r^2\}$ becomes $\{ v \in \reals^n: \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$, which is a hyperellipsoid. We therefore have the following proposition that gives the optimal $U$ which minimizes $\Delta_1 g_e$ and $\Delta_2 g_e$. 

\begin{prop}[Optimal $U$ that Minimizes $\Delta_1 g_e$]
For given $\Sigma$, $U = I$ minimizes $\Delta_1 g_e$, whose minimum value is
\begin{align}
\Delta_1 g_e = 2 \sqrt{\sum_{i=1}^n \frac{\sigma_i^2}{r^2}}
\end{align}
\end{prop}

\begin{proof}
It is proved by using some geometric properties of the hyperellipsoid. Due to space limit, please see appendix.
\end{proof}

\begin{prop}[Optimal $U$ that Minimize $\Delta_2 g_e$] \label{prop:U_l2norm}
For given $\Sigma$, we can choose any orthogonal $U$, and they all give the same value of $\Delta_2 g_e = 2 \frac{\sigma_1}{r}$.
\end{prop}

\begin{proof}
When $U = I$, the maximum $\ell_2$ distance between any two points on $\{ v \in \reals^n: \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$ is $2 \frac{\sigma_1}{r}$, corresponding to points $(\pm \frac{\sigma_1}{r}, 0, \cdots, 0)$. And rotate transformation $U$ doesn't affect $\Delta_2 g_e$. So we have $\Delta_2 g_e = 2 \frac{\sigma_1}{r}$ for any orthogonal $U$.
\end{proof}


TODO

---------



since any orthogonal $U$ is optimal, for simplicity we just let $U = I$. Therefore, for optimal encoder design we only consider $C = \Sigma Q^\top$.  

Next we need to consider how to select $\sigma_1^2, \cdots, \sigma_n^2$ to minimize Eq.\ref{eq:loss_Sigma}. Clearly, for any given $\sigma_1^2, \cdots, \sigma_n^2$ if we increase them proportionally, $\sigma_w^2$ also need to be increased proportionally to preserve the same $(\epsilon, \delta)$-LDP. So without loss of generality, we impose an additional constraint $\sum_{i=1}^n \sigma_i^2 = M$, where $M$ is a positive constant.

Constraint $\sum_{i=1}^n \sigma_i^2 = M$ guarantees the sum of variance of $g_e$ remains the same, but it doesn't guarantee $\sigma_w^2$ remains unchanged, because $\sigma_w^2$ is based on the sensitivity of function $g_e$, which further depends on the maximum difference under $\ell_1$ or $\ell_2$ norm, but not the variance. Due to the difficulty of directly coordinating these two parts, we here consider a sub-problem first: for fixed $\sigma_w^2$, what is the optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ such that $\loss$ in Eq.\ref{eq:loss_Sigma} is minimized, given $\sum_{i=1}^Z \sigma_i^2 = M$? The solution is given by the following proposition.

\begin{prop}[Optimal $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ under given $\sigma_w^2$]
When $\sigma_w^2$ is fixed and under given constraint $\sum_{i=1}^n \sigma_i^2 = M$, the optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ is given by
\begin{align}
\sigma_i^2 = 
\begin{cases}
\frac{\sqrt{\lambda_i}}{\sum_{i=1}^T \sqrt{\lambda_i}}(M+T\sigma_w^2) - \sigma_w^2, & \forall i \in \{1, 2, \cdots, T\}\\
0, & \forall i \in \{T+1, T+2, \cdots, n\}
\end{cases} \label{eq:opt_sigma}
\end{align}
where $T \leq n$ is the biggest number such that:
\begin{align}
\frac{\sqrt{\lambda_T}}{\sum_{i=1}^T \sqrt{\lambda_i}}(M+T\sigma_w^2) - \sigma_w^2 > 0 \label{eq:opt_T}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{\sigma_w^2}{M + T\sigma_w^2} (\sum_{i=1}^T  \sqrt{\lambda_i})^2 + \sum_{i=T+1}^n \lambda_i \label{eq:loss_w}
\end{align}
\end{prop}

\begin{proof}
The considered optimization problem is to minimize $\loss$ in Eq.\ref{eq:loss_Sigma} under constraint $\sum_{i=1}^n \sigma_i^2 = M$ and $\sum_{i=1}^Z \sigma_i^2 \geq 0$ (here we view $\sigma_i^2$ instead of $\sigma_i$ as the decision variable). Note that though in Eq.\ref{eq:loss_Sigma} we also have $\sigma_1^2 \geq \sigma_n^2$, we don't need to explicitly consider this constraint, because minimizing $\loss$ will implicitly guarantee that, according to the rearrangement inequality. 

This problem can be solved by Karush–Kuhn–Tucker (KKT) approach, with the following Lagrangian function:
\begin{align}
L(\sigma_1^2, \cdots, \sigma_n^2, \alpha_1, \cdots, \alpha_n, \beta) = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2} + \sum_{i=1}^n \alpha_i(-\sigma_i^2) + \beta(\sum_{i=1}^n \sigma_i^2 - M) 
\end{align}
where $\alpha_1, \cdots, \alpha_n$ and $\beta$ are Lagrangian multipliers. We know that the solution will automatically guarantee $\sigma_1^2 \geq \cdots \geq \sigma_n^2$, so we can safely assume there exists $T \leq Z$ such that $\alpha_i = 0$ for $i \leq T$, and $\alpha_i > 0$ for $i > T$. Then for $i > T$ we have $\sigma_i^2 = 0$, and for $i \leq T$ we have
\begin{align}
\frac{\nabla L}{\nabla \sigma_i^2} = -\frac{\sigma_w^2}{(\sigma_i^2 + \sigma_w^2)^2} \lambda_i = \beta
\end{align}
combining with $\sum_{i=1}^T \sigma_i^2 = M$ we eventually get Eq.\ref{eq:opt_sigma}. Enforcing $\sigma_T^2 > 0$ we get Eq.\ref{eq:opt_T}. And plug Eq.\ref{eq:opt_sigma} into Eq.\ref{eq:loss_Sigma} we get Eq.\ref{eq:loss_w}.   
\end{proof}

The above proposition doesn't tell us the optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ directly, because we assume $\sigma_w^2$ remains unchanged. However, we can design a numerical algorithm to find an approximated answer by using alternating iteration, as shown in Algorithm \ref{alg:ldp_codesign_linear}.

\begin{algorithm}[tb]
   \caption{$(\epsilon, \delta)$-LDP Preservation for Linear Encoder and Decoder with $\ell_2$ Task Loss (Co-Design)}
   \label{alg:ldp_codesign_linear}
   \begin{algorithmic}[1]
        \Require $\epsilon$, $\delta$
        \State Initialize $\sigma_w^2$ 
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\sigma_1^2, \cdots, \sigma_n^2$ based on Eq.\ref{eq:opt_sigma}
             \State Update $\sigma_w^2$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
        \EndFor
        \State Return $\sigma_1^2, \cdots, \sigma_n^2$ and $\sigma_w^2$
    \end{algorithmic}
\end{algorithm}  


\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}

\subsection{General Case}

For more complex scenarios, it is challenging to provide analytical forms of the optimal encoder and decoders. Thus, we present heuristic algorithms for both co-design approach and the benchmark approach.


\paragraph{Co-design.} Our proposed co-design algorithm in the general case is Algorithm \ref{alg:ldp_codesign}. It adopts a similar alternating iteration approach as Algorithm \ref{alg:ldp_codesign_linear}. However, for encoder parameter $\theta_e$, instead of directly penalizing $\loss$, we add an $\ell_2$ regularization term $\eta \|\theta_e\|^2$ where $\eta$ is a positive constant. Therefore, we update $\theta_e$ with the negative gradient $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$. Without regularization, the $\|\theta_e\|^2$ will grow arbitrarily since we can always achieve a lower $\loss$ by increasing $\phi$ proportionally. But it is not a direction we are looking for since $\sigma_w^2$ will also increase proportionally to guarantee $(\epsilon, \delta)$-LDP.  

\paragraph{Benchmark.} For the benchmark approach, our proposed algorithm only differs from Algorithm \ref{alg:ldp_codesign} in line 3 by just updating $\theta_d$ with $- \nabla_{\theta_d} \loss$ by one or multiple steps. In line 4, though $\Delta g_e$ remains unchanged, we still update $w$ to avoid overfitting. 

\begin{algorithm}[tb]
   \caption{$(\epsilon, \delta)$-LDP Preservation in the General Case (Co-Design)}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \Require $\epsilon$, $\delta$
        \State Initialize $\theta_e, \theta_d$ and $\sigma_w^2$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
             \State Update $w$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
        \EndFor
        \State Return $\theta_e, \theta_d$ and $\sigma_w^2$
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
%    \caption{$(\epsilon, \delta)$-LDP Preservation in the General Case (Benchmark)}
%    \label{alg:ldp_benchmark}
%    \begin{algorithmic}[1]
%         \Require $\epsilon$, $\delta$
%         \State Initialize $\theta_d$; set $g_e(x) = x$
%         \State Compute $\sigma_w^2$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
%         \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
%              \State Update $\theta_d$ with $- \nabla_{\theta_d} \loss$
%         \EndFor
%         \State Return $\theta_d$ and $\sigma_w^2$
%     \end{algorithmic}
% \end{algorithm}


==> sections/old/analysis_3.tex <==
\subsection{Linear Encoder and Decoder with $\ell_2$ Task Loss}

In this subsection, we consider a linear encoder and decoder framework with $\ell_2$ task loss. That is, $g_e$ and $g_d$ are linear functions in their corresponding inputs, and the loss function $l = \|K(\hat{x} - x)\|^2_2$ where $K \in \reals^{m \times n}$ is the task matrix.

\paragraph{Practicality of the setting.} Linear transformation is the most basic encoding and decoding approach for many dimensionality-reduction techniques, such as principal component analysis (PCA). And $\ell_2$ task loss is quite common in many application scenarios. For example, belows are two types of applications with $\ell_2$ task loss:
\begin{itemize}
\item \textbf{Estimate the mean.} Given $N$ samples of $x$, we want to estimate the mean of these samples in a few directions. These directions are denoted by $K' \in \reals^{m \times n}$. Then the sum of the variance of these estimations by using $\hat{x}$ instead of $x$ will be $\loss = \frac{1}{N}\E_{x \sim \dist}[\|K'(\hat{x} - x)\|^2_2] = \E_{x \sim \dist}[\|\frac{1}{\sqrt{N}} \cdot K'(\hat{x} - x)\|^2_2] $, which is a natural objective function.
\item \textbf{Linear-quadratic regulator (LQR).} In LQR problem, The control decision $u$ that minimizes the control cost is given by $u = -Kx$, where $K$ is a matrix determined by the matrices associated with the linear dynamics and the quadratic cost. $l = \|K(\hat{x} - x)\|^2_2$ captures the total mean-squared error of control when using $\hat{x}$ instead of $x$ as our current state observation.
\end{itemize}

Without loss of generality, we can also assume $\mu_x = \bm{0}$ and $\Sigma_{xx}$ is positive definite, where $\mu_x$ and $\Sigma_{xx}$ are the mean vector and the covariance matrix of $x$, respectively. Zero-centered $x$ saves us from considering the constant terms in the linear encoder and decoder functions, and positive definite $\Sigma_{xx}$ guarantees $x$ cannot be linear transformed to a low-dimensional representation without losing information.

We then factorize $\Sigma_{xx}$ into $Q \Lambda Q^\top$, where $Q$ is an orthogonal matrix composed of $\Sigma_{xx}$'s eigen vectors and $\Lambda$ is a diagonal matrix composed of $\Sigma_{xx}$'s eigen values. For the convenience of our further analysis, we let $h = \Omega^{-1}x$ where $\Omega = Q \sqrt{\Lambda}$. Here $h$ can be viewed as another representation of $x$, with covariance matrix $\Sigma_{hh} = I$. Since $K x = P h$, where $P = K \Omega$, it is equivalent to considering data representation $h$ with task matrix $P$.

We use $C \in \reals^{Z \times n}$ and $G \in \reals^{n \times Z}$ to denote the encoder and decoder matrix associated with $h$, i.e., $\phi = C h$ and $\hat{h} = G(Ch+w)$. Equivalently, based on the relationship between $x$ and $h$ we have $\phi = C \Omega^{-1} x$ and $\hat{x} = \Omega G(C\Omega^{-1}x+w)$. We also use $\Sigma_{ww}$ to denote the covariance matrix of $w$, and it can be expressed as $\Sigma_{ww} = \sigma_w^2 I$, where $\sigma_w^2$ is the variance of the noise we will add to each dimension of $\phi$.

Let's first determine the optimal decoder $G$ that minimizes $\loss$ for a given encoder $C$, which is given by the following proposition.

\begin{prop}[Optimal decoder $G$ that minimizes $\loss$]\label{prop:opt_decoder}
An optimal decoder $G$ that minimizes $\loss$ for a given encoder $C$ can be expressed as $G = C^\top (C C^\top + \Sigma_{ww})^{-1}$, and corresponding $\loss$ is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  C^\top (CC^\top + \Sigma_{ww})^{-1} C) \label{eq:loss_C}
\end{align} 
\end{prop}
\begin{proof}
We have
\begin{align}
\loss 
& = \E[\|K(\hat{x} - x)\|^2_2] = \E[\|P(\hat{h} - h)\|^2_2] 
= \E[\|P((GC-I)h + Gw)\|^2_2]\\
& = \E[\tr(P(GC-I)hh^\top (GC-I)^\top P^\top) + \tr(P G ww^\top G^\top P^\top)]\\
& = \tr(P(GC-I) (GC-I)^\top P^\top) + \tr(P G \Sigma_{ww} G^\top P^\top) \label{eq:loss_CG}
\end{align}
where $\tr(\cdot)$ denotes the trace of a matrix. And we can verify that $G = C^\top (C C^\top + \Sigma_{ww})^{-1}$ is a zero point of
\begin{align}
\frac{\nabla \loss}{\nabla G} = 2 P^\top P ((GC-I) C^\top + G \Sigma_{ww})
\end{align}
Then we plug the expression of $G$ into Eq.\ref{eq:loss_CG} and get Eq.\ref{eq:loss_C}.
\end{proof}

We can also get the resulted $\loss$ for our benchmark apporach by letting $C = \Omega$ and plug it into Eq.\ref{eq:loss_C}.
\begin{cor}[Optimal $\loss$ for the benchmark approach]
The optimal $\loss$ for the benchmark approach is
\begin{align}
\loss = \tr(P^\top P) - \tr(P^\top P  \Omega^\top (\Omega\Omega^\top + \Sigma_{ww})^{-1} \Omega)
\end{align}
\end{cor}

Our next step is to design an encoder $C$ that minimizes Eq.\ref{eq:loss_C}. Without loss of generality, we let $Z \geq n$ and allow some columns of $C$ be zero. Suppose the singular value decomposition of $C$ is $U \Sigma V^\top$, where $U \in \reals^{Z \times Z}$ and $V \in \reals^{n \times n}$ are orthogonal matrices and $\Sigma \in \reals^{Z \times n}$ is a rectangular diagonal matrix. And the singular values are denoted by $\sigma_1, \cdots, \sigma_n$ with $|\sigma_1| \geq \cdots \geq |\sigma_n|$. Then designing $C$ is equivalent to designing matrix $U$, $V$ and $\Sigma$.

The geometric interpretation of applying transform $C = U \Sigma V^\top$ to vector $h$ contains three sub-transforms: 1) rotate $h$ by applying rotation matrix $V^\top$; 2) scale $V^\top h$ by applying scaling matrix $\Sigma$; 3) rotate $\Sigma V^\top h$ by applying rotation matrix $U$. Any arbitrary rotate transformation $R \in \reals^{n \times n}$ doesn't change the $\ell_2$ norm of any vector $v \in \reals^n$, because $\|R v\|^2_2 = \tr(v^\top R^\top R v) = \tr(v^\top v) = \|v\|^2_2$. But for $\ell_1$ norm it is usually not true. And scaling transformation doesn't maintain either $\ell_1$ or $\ell_2$ norm in general. Therefore, in general, for $\ell_1$ norm, the choice of any of $U$, $\Sigma$ and $V$ will affect $\Delta_1 g_e$ and $\sigma_w^2$; and for $\ell_2$ norm, only the choice of $\Sigma$ and $V$ will affect $\Delta_2 g_e$ and $\sigma_w^2$ (transformation $V^\top$ doesn't change $\ell_2$ norm itself, but since it specifies the directions that $\Sigma$ should be applied it will eventually affect the $\Delta_2 g_e$ and $\sigma_w^2$).

In the following analysis, we make the following assumption in terms of the boundary of the region of $h$.

\begin{assumption} [Boundary is a hypersphere] \label{assumption:boundary_h}
The boundary of the region of $h$ is a hypersphere of radius $r \geq 1$, which is expressed as $\{ h \in \reals^n: \|h\|_2^2 = r^2\}$.
\end{assumption} 

 This is a non-trivial assumption, but we are essentially assuming the maximum value of $\|d^\top h\|_2^2$ in any direction $d \in \reals^n$ s.t. $\|d\|^2_2 = 1$ is proportional to the variance of $d^\top h$, which is always 1 (since we have $\Sigma_{hh} = I$ already). And from $\text{Var}(d^\top h) \leq \E[(d^\top h)^2] \leq r^2$ we get $r \geq 1$. Since the equation of a centered hypersphere after rotation remains unchanged, this assumption gives us a nice property: the choice of $V$ doesn't change the equation of the boundary and hence doesn't affect $\Delta g_e$ and $\sigma_w^2$.

Based on the above assumption, we can safely consider the optimal design of $V$ that minimizes $\loss$ when $\Sigma$ and $\sigma_w^2$ are given, which leads to the following proposition.

\begin{prop}[Optimal $V$ that minimizes $\loss$ under Assumption \ref{assumption:boundary_h}]
Suppose the eigen decomposition of the Gram matrix $P^\top P$ is expressed as $P^\top P Q = Q \Lambda$, where $\Lambda = \text{diag}(\lambda_1, \cdots, \lambda_n)\in \reals^{n\times n}$ is a diagonal matrix whose diagonal elements are eigen values with $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$, and $Q \in \reals^{n \times n}$ is an orthogonal matrix whose columns are corresponding normalized eigen vectors. Then $\loss$ is minimized for $V = Q$, under given $\Sigma$ and $\sigma_w^2$. And the corresponding $\loss$ can be expressed as
\begin{align}
\loss = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2} \label{eq:loss_Sigma}
\end{align}
\end{prop}

\begin{proof}
We have $\tr(P^\top P) = \sum_{i=1}^n \lambda_i$, which is a fixed number. Therefore we focus on maximizing the second trace term in Eq.\ref{eq:loss_C}. We first notice that
\begin{align}
C\Sigma_{xx}C^\top + \Sigma_{ww} = U \Sigma \Sigma^\top  U^\top + \sigma_w^2 I = U \text{diag}(\sigma_1^2+\sigma_w^2, \cdots, \sigma_n^2 + \sigma_w^2, \underbrace{\sigma_w^2, \cdots, \sigma_w^2}_{Z-n\text{ in total}}) U^\top
\end{align}
Then we have
\begin{align}
& C^\top (CC^\top + \Sigma_{ww})^{-1} C\\ 
= & V \Sigma^\top U^\top \cdot U \text{diag}(\frac{1}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{1}{\sigma_n^2+\sigma_w^2}, \frac{1}{\sigma_w^2}, \cdots, \frac{1}{\sigma_w^2}) U^\top \cdot U \Sigma V^\top\\
= & V \Sigma^\top \text{diag}(\frac{1}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{1}{\sigma_n^2+\sigma_w^2}, \frac{1}{\sigma_w^2}, \cdots, \frac{1}{\sigma_w^2}) \Sigma V^\top\\
= & V \text{diag}(\frac{\sigma_1^2}{\sigma_1^2+\sigma_w^2}, \cdots, \frac{\sigma_n^2}{\sigma_n^2+\sigma_w^2}) V^\top
\end{align}
so $C^\top (CC^\top + \Sigma_{ww})^{-1} C$ is a positive semi-definite matrix with eigen-values $\frac{\sigma_1^2}{\sigma_1^2+\sigma_w^2} \geq \cdots \geq \frac{\sigma_n^2}{\sigma_n^2+\sigma_w^2} \geq 0$. Then by Ruhe's trace inequality \cite{ruhe1970perturbation} (a corollary of Von Neumann’s trace inequality \cite{von1937some}), we have
\begin{align}
\tr(P^\top P  C^\top (CC^\top + \Sigma_{ww})^{-1} C) \leq \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2}
\end{align}
and when $V = Q$ the equality holds. So we have Eq.\ref{eq:loss_Sigma} for $V = Q$.
\end{proof}
 
In the above proposition, we see choosing a $Z > n$ brings no additional benefit, so for simplicity we only consider $Z = n$. 

% And when $\sigma_w^2$ is fixed, the choice of $U$ doesn't affect loss $\loss$. This is immediately true when we use $\sigma_w^2$ is based on $\Delta_2 g_e$ (as we discussed earlier). However, we still need to carefully design $U$ when $\sigma_w^2$ is based on $\Delta_1 g_e$.

We notice that, after the first two transforms $\Sigma$ and $V^\top$, the boundary $\{ h \in \reals^n: \|h\|_2^2 = r^2\}$ becomes $\{ v \in \reals^n: \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$, which is a hyperellipsoid. We therefore have the following proposition that gives the optimal $U$ which minimizes $\Delta_1 g_e$ and $\Delta_2 g_e$. 

\begin{prop}[Optimal $U$ that minimizes $\Delta_1 g_e$ under Assumption \ref{assumption:boundary_h}]
For given $\Sigma$, $U = I$ minimizes $\Delta_1 g_e$, whose minimum value is
\begin{align}
\Delta_1 g_e = 2r \sqrt{\sum_{i=1}^n \sigma_i^2}
\end{align}
\end{prop}

\begin{proof}
It is proved by using some geometric properties of the hyperellipsoid. We put the detailed proof in the appendix due to space limit.
\end{proof}

\begin{prop}[Optimal $U$ that minimizes $\Delta_2 g_e$ under Assumption \ref{assumption:boundary_h}] \label{prop:U_l2norm}
For given $\Sigma$, any orthogonal $U$ gives the same value of $\Delta_2 g_e$: 
\begin{align}
\Delta_2 g_e = 2r |\sigma_1|
\end{align}
\end{prop}

\begin{proof}
When $U = I$, the maximum $\ell_2$ distance between any two points on $\{ v \in \reals^n: \sum_{i=1}^n v_i^2 / \sigma_i^2 = r^2\}$ is $2r \cdot |\sigma_1|$, corresponding to points $(\pm 2r |\sigma_1|, 0, \cdots, 0)$. And rotate transformation $U$ doesn't affect $\Delta_2 g_e$. So we have $\Delta_2 g_e = 2r |\sigma_1|$ for any orthogonal $U$.
\end{proof}

Therefore, we can just choose $U = I$ to minimize either $\Delta_1 g_e$ and $\Delta_2 g_e$. 

% Therefore, for optimal encoder design we only consider $C = \Sigma Q^\top$.

Next we need to consider how to select $\sigma_1^2, \cdots, \sigma_n^2$ to minimize Eq.\ref{eq:loss_Sigma}, which is the only remaining piece. Clearly, for any given $\sigma_1^2, \cdots, \sigma_n^2$ if we increase them proportionally, $\sigma_w^2$ also need to be increased proportionally to preserve the same $(\epsilon, \delta)$-LDP. So without loss of generality, we impose an additional constraint $\sum_{i=1}^n \sigma_i^2 = M$, where $M$ is a positive constant. 

The following two propositions give the optimal choice for Laplace mechanism and Gaussian mechanism, respectively.

% Constraint $\sum_{i=1}^n \sigma_i^2 = M$ guarantees the sum of variance of $g_e$ remains the same, but it doesn't guarantee $\sigma_w^2$ remains unchanged, because $\sigma_w^2$ is based on the sensitivity of function $g_e$, which further depends on the maximum difference under $\ell_1$ or $\ell_2$ norm, but not the variance. Due to the difficulty of directly coordinating these two parts, we here consider a sub-problem first: for fixed $\sigma_w^2$, what is the optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ such that $\loss$ in Eq.\ref{eq:loss_Sigma} is minimized, given $\sum_{i=1}^Z \sigma_i^2 = M$? The solution is given by the following proposition.

\begin{prop}[Optimal $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $(\epsilon, 0)$-LDP with Laplace mechanism under  Assumption \ref{assumption:boundary_h}]
The optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $(\epsilon, 0)$-LDP with Laplace mechanism under constraint $\sum_{i=1}^n \sigma_i^2 = M$ is given by
\begin{align}
\sigma_i^2 = 
\begin{dcases*}
M \cdot (\frac{\sqrt{\lambda_i}}{\sum_{i=1}^T \sqrt{\lambda_i}}(1+T\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2}), & $\forall i \in \{1, 2, \cdots, T\}$\\
0, & $\forall i \in \{T+1, T+2, \cdots, n\}$
\end{dcases*} \label{eq:opt_sigma_laplace}
\end{align}
where $T \leq n$ is the biggest number such that:
\begin{align}
\frac{\sqrt{\lambda_T}}{\sum_{i=1}^T \sqrt{\lambda_i}}(1+T\cdot \frac{8r^2}{\epsilon^2}) - \frac{8r^2}{\epsilon^2} > 0 \label{eq:opt_T_laplace}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{8r^2/\epsilon^2}{1 + T\cdot8r^2/\epsilon^2} (\sum_{i=1}^T  \sqrt{\lambda_i})^2 + \sum_{i=T+1}^n \lambda_i \label{eq:loss_laplace}
\end{align}
\end{prop}

\begin{proof}
First, to preserve $(\epsilon, 0)$-LDP for Laplace mechanism, we have 
\begin{align}
\sigma_w^2 = 2 \cdot \frac{(\Delta_1 g_e)^2}{\epsilon^2} = 2 \cdot \frac{4r^2 \cdot \sum_{i=1}^n \sigma_i^2}{\epsilon^2} = \frac{8r^2M}{\epsilon^2} \label{eq:w_laplace}
\end{align}
under constraint $\sum_{i=1}^n \sigma_i^2 = M$. 

Next we need to determine $\sigma_1^2, \cdots, \sigma_n^2$. The considered problem is an optimization problem which aims at minimizing $\loss$ in Eq.\ref{eq:loss_Sigma} under constraint $\sum_{i=1}^n \sigma_i^2 = M$ and $\sum_{i=1}^Z \sigma_i^2 \geq 0$ (here we view $\sigma_i^2$ instead of $\sigma_i$ as the decision variable). Note that though in Eq.\ref{eq:loss_Sigma} we also have $\sigma_1^2 \geq \sigma_n^2$, we don't need to explicitly consider this constraint, because minimizing $\loss$ will implicitly guarantee that, according to the rearrangement inequality. 

This problem can be solved by Karush–Kuhn–Tucker (KKT) approach, with the following Lagrangian function:
\begin{align}
L(\sigma_1^2, \cdots, \sigma_n^2, \alpha_1, \cdots, \alpha_n, \beta) = \sum_{i=1}^n \lambda_i - \sum_{i=1}^n \lambda_i \frac{\sigma_i^2}{\sigma_i^2+\sigma_w^2} + \sum_{i=1}^n \alpha_i(-\sigma_i^2) + \beta(\sum_{i=1}^n \sigma_i^2 - M) 
\end{align}
where $\alpha_1, \cdots, \alpha_n$ and $\beta$ are Lagrangian multipliers. We know that the solution will automatically guarantee $\sigma_1^2 \geq \cdots \geq \sigma_n^2$, so we can safely assume there exists $T \leq Z$ such that $\alpha_i = 0$ for $i \leq T$, and $\alpha_i > 0$ for $i > T$. Then for $i > T$ we have $\sigma_i^2 = 0$, and for $i \leq T$ we have
\begin{align}
\frac{\nabla L}{\nabla \sigma_i^2} = -\frac{\sigma_w^2}{(\sigma_i^2 + \sigma_w^2)^2} \lambda_i = \beta
\end{align}
combining with $\sum_{i=1}^T \sigma_i^2 = M$ and Eq.\ref{eq:w_laplace} we eventually get Eq.\ref{eq:opt_sigma_laplace}. Enforcing $\sigma_T^2 > 0$ we get Eq.\ref{eq:opt_T_laplace}. And plug Eq.\ref{eq:opt_sigma_laplace} into Eq.\ref{eq:loss_Sigma} we get Eq.\ref{eq:loss_laplace}.   
\end{proof}

\begin{prop}[Optimal $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $(\epsilon, \delta)$-LDP with Gaussian mechanism under Assumption \ref{assumption:boundary_h}] \label{prop: opt_sigma_gaussian}
The optimal choice of $\sigma_1^2, \cdots, \sigma_n^2$ that minimize $\loss$ and preserve $(\epsilon, \delta)$-LDP with Gaussian mechanism under constraint $\sum_{i=1}^n \sigma_i^2 = M$ is given by
\begin{align}
\sigma_i^2 = \frac{M}{n} \quad \forall i \in \{1, 2, \cdots, n\} \label{eq:opt_sigma_gaussian}
\end{align}
and the corresponding $\loss$ is
\begin{align} 
\loss = \frac{8r^2 \log (1.25/\delta)/\epsilon^2}{1+ 8r^2 \log (1.25/\delta)/\epsilon^2} \sum_{i=1}^n \lambda_i \label{eq:loss_gaussian}
\end{align}
\end{prop}

\begin{proof}
We first drop the constraint $\sum_{i=1}^n \sigma_i^2 = M$, and enforce it in the end.

To preserve $(\epsilon, \delta)$-LDP with Laplace mechanism, we have 
\begin{align}
\sigma_w^2 = \frac{2 \log (1.25/\delta) \cdot (\Delta_2 g_e)^2}{\epsilon^2} = \frac{2 \log (1.25/\delta) \cdot 4r^2 \sigma_1^2}{\epsilon^2} = \frac{8r^2 \log (1.25/\delta)}{\epsilon^2} \cdot\sigma_1^2 \label{eq:w_laplace}
\end{align}
which means we have fixed $\sigma_w^2$ for fixed $\sigma_1^2$. Therefore, $\sigma_2^2, \sigma_3^2, \cdots, \sigma_n^2$ should be as large as possible to minimize $\loss$ in Eq.\ref{eq:loss_Sigma}, since $\sigma_w^2$ doesn't depend on them. Thus we should make $\sigma_1^2 = \sigma_2^2 = \cdots = \sigma_2^2$. Plug it and Eq.\ref{eq:w_laplace} into Eq.\ref{eq:loss_Sigma} we get Eq.\ref{eq:loss_gaussian}.

And enforcing constraint $\sum_{i=1}^n \sigma_i^2 = M$ we get Eq.\ref{eq:opt_sigma_gaussian}. 
\end{proof}

\paragraph{Summary.} Proposition \ref{prop:opt_decoder}-\ref{prop: opt_sigma_gaussian} give the optimal encoder and decoder design with Laplace and Gaussian mechanism, under the Assumption \ref{assumption:boundary_h}. In the general case, if the boundary of the region of $h$ is not a hypersphere, we can use the smallest hypersphere to bound the region of $h$, and get a sub-optimal design of the encoder and decoder with Laplace and Gaussian mechanism. And this yields a near-optimal solution if the boundary of the region of $h$ is "nearly" a hypersphere.

\subsection{General Case}

For more complex scenarios, it is challenging to provide analytical forms of the optimal encoder and decoders. Thus, we present heuristic algorithms for both co-design approach and the benchmark approach.


\paragraph{Co-design.} Our proposed co-design algorithm in the general case is Algorithm \ref{alg:ldp_codesign}. It adopts a similar alternating iteration approach. However, for encoder parameter $\theta_e$, instead of directly penalizing $\loss$, we add an $\ell_2$ regularization term $\eta \|\theta_e\|^2$ where $\eta$ is a positive constant. Therefore, we update $\theta_e$ with the negative gradient $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$. Without regularization, the $\|\theta_e\|^2$ will grow arbitrarily since we can always achieve a lower $\loss$ by increasing $\phi$ proportionally. But it is not a direction we are looking for since $\sigma_w^2$ will also increase proportionally to guarantee $(\epsilon, \delta)$-LDP.  

\paragraph{Benchmark.} For the benchmark approach, our proposed algorithm only differs from Algorithm \ref{alg:ldp_codesign} in line 3 by just updating $\theta_d$ with $- \nabla_{\theta_d} \loss$ by one or multiple steps. In line 4, though $\Delta g_e$ remains unchanged, we still update $w$ to avoid overfitting. 

\begin{algorithm}[tb]
   \caption{$(\epsilon, \delta)$-LDP Preservation in the General Case (Co-Design)}
   \label{alg:ldp_codesign}
   \begin{algorithmic}[1]
        \Require $\epsilon$, $\delta$
        \State Initialize $\theta_e, \theta_d$ and $\sigma_w^2$
        \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
             \State Update $\theta_e$ and $\theta_d$ with $- (\nabla_{\theta_e} \loss + 2 \eta \theta_e)$ and $- \nabla_{\theta_d} \loss$, respectively, by one or multiple steps
             \State Update $w$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
        \EndFor
        \State Return $\theta_e, \theta_d$ and $\sigma_w^2$
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
%    \caption{$(\epsilon, \delta)$-LDP Preservation in the General Case (Benchmark)}
%    \label{alg:ldp_benchmark}
%    \begin{algorithmic}[1]
%         \Require $\epsilon$, $\delta$
%         \State Initialize $\theta_d$; set $g_e(x) = x$
%         \State Compute $\sigma_w^2$ based on $\Delta g_e$ and LDP requirement $(\epsilon, \delta)$
%         \For{$\tau \in \{0, 1, \cdots, N_\text{epochs}-1\}$}
%              \State Update $\theta_d$ with $- \nabla_{\theta_d} \loss$
%         \EndFor
%         \State Return $\theta_d$ and $\sigma_w^2$
%     \end{algorithmic}
% \end{algorithm}


==> sections/old/problem_formulation.tex <==
We now formally define the privacy preservation problem in end-to-end model learning. Let $\target$ and $\privacy$ denote the target task that the user wants to accomplish and the adversarial task that the user wants to preserve privacy from, respectively. And let $x \in \reals^n$ be an original data sample which is drawn from distribution $\dist$. 

To preserve the privacy of $x$, we consider a general encoder-decoder model. The encoder maps $x$ to a latent representation $\phi \in \reals^Z$ with $Z \leq n$, using model parameter $\theta_e$:
\begin{align}
\phi = g_e(x; \theta_e)
\end{align}
And the decoder associated with task $k$, $\forall k \in \{ \target, \privacy\}$, reconstructs an estimate of $x$, denoted by $\hat{x}_k$, using model parameter $\theta_{d, k}$:
\begin{align}
\hat{x}_k = g_{d,k}(\phi; \theta_{d,k}) \label{eq:decoder}
\end{align}

For task $k \in \{1,2\}$, define task loss $\loss_k = \E_{x \sim \dist}[l_k(\hat{x}_k, x)]$, where $l_k$ represents the loss of using the reconstructed data $\hat{x}_k$ instead of original data $x$. Our target is to minimize $\loss_\target$ as much as possible while maximize $\loss_\privacy$ as much as possible. Note that the decoder parameter $\theta_\privacy$ associated with task $\privacy$ is determined by the opponent, hence we cannot manipulate it in reality and need to assume it is always optimal, i.e., minimizes $\loss_\privacy$, under any given encoder parameter $\theta_e$.  

\subsection{Preserve LDP for encoder output}

In our problem, to preserve $(\epsilon, \delta)$-LDP we treat encoder function $g_e$ as the sensitive function $f$, and use $w \in \reals^Z$ to denote the $Z$-dimensional Laplace or Gaussian vector added to the the latent representation $\phi$. For convenience we let $\phi' = \phi + w$ represent the noisy latent representation.

\paragraph{Encoder and Decoder Separate Design.} In the separate design case, the encoder parameter $\theta_e$ is first determined \textit{without considering privacy preservation}:
\begin{align}
\min_{\theta_e} \min_{\theta_{d,\target}} \quad & \loss_\target = \E_{x \sim \dist}[l_\target(\hat{x}_\target, x)]\\
\text{s.t.} \quad & \hat{x}_\target = g_{d,\target}(g_e(x; \theta_e); \theta_{d,\target})
\end{align}

We can then determine the scale or the variation of each element in the noise vector $w$, based on the sensitivity of function $g_e$ under parameter $\theta_e^*$ and input $x \sim D$. In the end, the target task and the adversarial task will then determine the optimal decoder parameters for input $\phi'$, i.e., $\forall k \in \{\target, \privacy\}$:
\begin{align}
\min_{\theta_{d,k}} \quad & \loss_k = \E_{x \sim \dist}[l_k(\hat{x}_i, x)] \label{eq:ldp_decoder_1}\\
\text{s.t.} \quad & \hat{x}_k = g_{d,k}(g_e(x; \theta_e^*) + w; \theta_{d,k}) \label{eq:ldp_decoder_2}
\end{align}

\paragraph{Encoder and Decoder Co-design.} In the co-design case, we determine the optimal $\theta_e$ and $\theta_{d,\target}$ such that $\loss_\target$ is minimized and \textit{$(\epsilon, \delta)$-LDP is preserved}:
\begin{align}
\min_{\theta_e, \theta_{d,\target}} \quad & \loss_\target = \E_{x \sim \dist}[l_\target(\hat{x}_\target, x)]\\
\text{s.t.} \quad & \hat{x}_\target = g_{d,\target}(g_e(x; \theta_e)+w; \theta_{d,\target})\\
& w \sim \text{Lap}^Z(0, \frac{\Delta_1 g_e}{\epsilon}) \text{ or } \mathcal{N}^Z(0, \frac{2 \log (1.25/\delta) \cdot (\Delta_2 g_e)^2}{\epsilon^2}) 
\end{align}
and the adversarial task can determine its encoder in the end using the same method as Eq.\ref{eq:ldp_decoder_1}-\ref{eq:ldp_decoder_2}.

\paragraph{Benchmark.} The benchmark policy preserves $(\epsilon, \delta)$-LDP by adding noise vector directly to the original data $x$, i.e., $g_e(x) = x$ and $w \in \reals^{n}$.

\subsection{Task-based Privacy}

The task-based privacy preservation scheme jointly considers the $\loss_\target$ and $\loss_\privacy$ when determining the optimal $\theta_e$ and $\theta_{d,\target}$:
\begin{align}
\min_{\theta_e, \theta_{d,\target}} \max_{\theta_{d,\privacy}} \quad & \loss_\total = \loss_\target - \lambda \loss_\privacy = \E_{x \sim \dist}[l_\target(\hat{x}_\target, x) - \lambda l_\privacy(\hat{x}_\privacy, x)]\\
\text{s.t.} \quad & \phi = g_e(x; \theta_e)\\
& \hat{x}_k = g_{d,k}(\phi; \theta_{d,k}), \quad \forall k \in \{ \target, \privacy\}
\end{align}
where $\lambda$ is a privacy-preservation weight specified by the user.

